POLYFLOW: A Neuro-Symbolic Framework for Static Cross-Language Information Flow Analysis

Modern software systems are commonly constructed in multiple, interacting programming languages. This construction leads to additional, often stealthy vulnerabilities buried in complex information flow due to language interactions. Existing static analyzers are impeded by the heterogeneous semantics of different languages, whereas dynamic approaches suffer from the limited coverage of (available and/or generated) test inputs. In this paper, we develop PolyFlow, a neural-symbolic framework for statically reasoning about information flow across language boundaries, combining large language models (LLMs) and static analysis synergistically. Governed by the control-flow representation of a given multi-language system, PolyFlow leverages LLMs to identify implicit flow facts due to challenging language features, hence augmenting the base representation and then propagating data flow through the system. It tackles inherent barriers (e.g., token limit and hallucination) of LLMs by putting them under careful guidance (e.g., static-analysis-guided scoping, context management, and fact checking), along with a multi-LLM expert panel for negotiated validation. Our experiments on real-world Python-C and Java-C systems show that PolyFlow is cost-effective and superior to various kinds of state-of-the-art baselines, revealing previously unknown cross-language vulnerabilities that are missed by all the baselines.

==> Sections/00_abstract-cai.tex <==

\begin{abstract}
% Modern software systems are commonly constructed in multiple, interacting programming languages, especially in the era of machine learning (ML). While well justifiable, the multi-language construction leads to additional, often stealthy vulnerabilities induced by the information flow due to the language interactions. Analyzing the cross-language information flow is challenging due to the heterogeneous semantics of the languages. Existing relevant works are mostly resort to dynamic analysis, which are subject to the limited coverage of test inputs, either available or generated. In this paper, we develop {\tech}, a purely static information flow analysis framework that leverages foundation large language models (LLMs) anAd traditional static analysis working synergistically as an LLM-based agent. {\tech} particularly deals with implicit flows that conventional static analysis often stumbles to resolve due to dynamic language features, through a fixed-point iterative feature handling process. We have implemented {\tech} for systems built in Python and C, and applied to 13 real-world Python-C projects of diverse scales and domains. Our results demonstrate the superiority of {\tech} in static cross-language information flow analysis over state-of-the-art (static, dynamic, and ML-based) baselines in terms of accuracy, while maintaining practical scalability to large-scale multi-language systems. 
% %It also enabled the discovery of a number of previously unknown cross-language vulnerabilities that the baselines failed to detect.

Modern software systems are commonly %and increasingly 
constructed in multiple, \textit{interacting} programming languages. %especially in the era of machine learning (ML). 
%While well justifiable, 
This %multilingual 
construction leads to additional, often stealthy vulnerabilities %induced by complex information flow resulting from language interactions. 
buried in complex information flow due to language interactions.
%Analyzing the cross-language information flow is challenging due to the heterogeneous semantics of the languages. 
%Existing relevant works often resort to dynamic analysis, hence subject to the limited coverage of (available or generated) test inputs. 
Existing static analyzers are impeded by the heterogeneous semantics of different languages, whereas %current 
dynamic approaches suffer from the limited coverage of (available and/or generated) test inputs. 
%, either available or generated. 
%In this paper, we develop {\tech}, an \textit{agentic} framework based on foundation large language models (LLMs) and traditional static analysis working synergistically for \textit{purely static cross-language information flow analysis}. 
In this paper, we develop {\tech}, an \textit{agentic} framework for statically reasoning about information flow across language boundaries via a neuro-symbolic approach, 
combining large language models (LLMs) and static analysis synergistically. 
Governed by the control-flow representation of a given multi-language system, the agent leverages LLMs to identify implicit flow facts due to challenging language features, hence augmenting the base representation and then propagating data flow through the system. 
%, both under careful guidance (e.g., scope reduction and context management/coordination) of the static analysis. 
%It explicitly identifies and reasons about control and data flow both within and across language boundaries, including those induced by challenging language features, while balancing analysis cost and effectiveness via a refinement-based strategy. 
%It also deals with inherent limitations of LLMs via static analysis for guidance and a multi-LLM expert panel for cross-validation. 
It addresses inherent barriers (e.g., token limit and hallucination) of LLMs by putting them under careful guidance (e.g., %scope reduction, context coordination, 
adaptive scoping, context management, and fact checking) of the static analysis, along with a multi-LLM expert panel for negotiated agreements. 
%We implemented {\tech} for systems built in Python and C, and applied it to ? real-world Python-C projects of diverse scales and domains.  
Our experiments show that {\tech} is cost-effective and superior to various kinds of state-of-the-art baselines, % for analyzing cross-language information flow, 
%enabling discovery of 
revealing previously unknown cross-language vulnerabilities in real-world systems that are missed by all the baselines. 
\end{abstract}


==> Sections/00_abstract.tex <==
\begin{abstract}

\end{abstract}

==> Sections/01_intro-cai.tex <==
%!TEX root = paper.tex
\vspace{-3pt}
\section{Introduction}\label{sec:intro}
\vspace{-2pt}
% the context of problem: prevalance of multilingual construction
Software systems today are mostly \textit{multilingual}~\cite{jones2010software,delorey2007programming,ray2014large,yang2024multi}, composed of code units %written 
in diverse programming languages that \textit{interact} to deliver seamless functionalities~\cite{tomassetti2014empirical,mayer2015empirical,valverde2015punctuated,li2024multilingual}. This heterogeneous composition is well justified by combining the unique advantages of individual languages\cite{bae2019towards,mayer2017multi}. 
For instance, highly impactful %and pervasive 
machine learning (ML) frameworks (e.g., TensorFlow and PyTorch) are typical examples of multi-language (Python-C) software, which leverage Python for its support of rapid prototyping and C for its great performance efficiency~\cite{hu2023empirical,li2023understandingb,li2025automated}. 

% the problem targeted: presence and prevalence and damage of cross-language vulnerabilities
However, %so much as it enhances productivity, 
the multilingual construction also results in greater complexity of multi-language systems, which leads to their statistical proneness~\cite{wen22fse,ray2014large,abidi2021multi,kochhar2016large,grichi2020impactjni} and practical exposure~\cite{dinh2021favocado,wen22usenixsecurity} to increased security threats.
In particular, the interaction between languages introduces \textit{{cross-language vulnerabilities}} as recently discovered~\cite{staicu2023bilingual,wen23usenixsecurity}: security flaws that arise from semantic mismatches, implicit assumptions and flows, or unsafe data exchange across language boundaries~\cite{hwang2021justgen,yang2024learning}. 
For example, in Python-C systems, improper marshaling of data types due to dynamic typing in Python caused unsafe memory allocation hence corruption in C through a native function call~\cite{wen22usenixsecurity}. 
%As another example, unchecked string formatting in C led to code injection vulnerabilities in Python via a foreign function return~\cite{wen22fse,haoran25fse}.  
These vulnerabilities are systemic yet stealthy, often escaping detection 
%due to the fragmented nature of existing analysis tools~\cite{horwitz10jan,yang2024learning}, which operate in language-specific silos. 
as existing analysis tools mostly operate in language-specific silos~\cite{horwitz10jan,yang2024learning}. 
Securing multi-language systems demands a %paradigm shift toward 
\textit{holistic}, cross-language analysis~\cite{wen22usenixsecurity,youn2023declarative,dinh2021favocado}, whose urgency is driven by the growing dominance of those systems~\cite{yang2024multi,meyerovich2013empirical,vasilescu2013babel,li2023understandinga,li2024exploratory}. 

%Despite widespread attention, cross-language vulnerabilities remain a critical, yet under-addressed, security challenge. Recent incident analyses have exposed how bugs spanning language boundaries (for example, type misinterpretation across C and Python or memory mismanagement between system-level and scripting languages) can lead to severe breaches. The discovery of such vulnerabilities in real-world systems illustrates a worrying gap in our current defenses, as attackers increasingly target the multilingual interfaces where traditional protection mechanisms falter.
%
%The significance and pervasiveness of cross-language vulnerabilities cannot be overstated, as they present a substantial threat to the overall security posture of multilingual software systems. Previously identified cross-language bugs serve as stark reminders of the potential dangers associated with these vulnerabilities. Consider, for instance, vulnerabilities that arise from improper handling of data types or memory management across language boundaries, which can lead to memory corruption, buffer overflows, and other critical security flaws. Detecting and addressing these vulnerabilities is essential to protect multilingual software systems from potential exploitation by malicious actors, thereby ensuring the continued reliability and trustworthiness of these systems.
%
%Cross-language vulnerabilities are both prevalent and perilous, as they exploit gaps in developers’ mental models of multilingual interactions. Such vulnerabilities persist because conventional static analyzers, fuzzers, and ML-based detectors focus on single-language contexts, failing to track tainted data flows across language boundaries. This limitation leaves critical attack surfaces unexamined, particularly in systems where high-level language abstractions (e.g., Python’s dynamic typing) interact unpredictably with low-level memory operations (e.g., C’s manual allocation).

% motivation: existing solutions and why they are not sufficient
In response, %the last few years have seen a number of 
relevant approaches exist. 
Yet many of them~\cite{fin2001amleto,fragoso2020gillian,groce2018extensible,liu2020fans,dinh2021favocado,moller2024cross} actually tackle single-language bugs, where the
“cross-language" terms, when present, refer to “supporting different languages", \textit{not} concerning scenarios where those languages \textit{co-exist and interact} in one project~\cite{li2023understandinga,li2023understandingb,li2024exploratory,ray2014large,berger2019impact,zhang2019study}. 
Among techniques that do address multilingual code, some only look at the design-level smells~\cite{abidi2021multi,li2025automated} or are limited to %cross-language 
API misuses~\cite{sultana2016understanding,hu2023empirical}. 
To really tackle cross-language bugs, a few \textit{dynamic} approaches emerged~\cite{bai2018bridgetaint,xue2018ndroid,wen22usenixsecurity}. However, they can only reveal bugs exercised by given test cases---which are particularly scarce in multi-language projects~\cite{wen23usenixsecurity}. 
While this may be mitigated by generating more tests, existing solutions either resort to much manual effort~\cite{hwang2021justgen} or fail due to the technique's randomness~\cite{wen23usenixsecurity}. 

Current \textit{static} approaches bypass the coverage limitation, but they rely on language-specific semantic rules~\cite{youn2023declarative} or abstract summaries~\cite{lee2020broadening,park2023static}/specification~\cite{kan2024cross} for native code and/or language interoperability, hence requiring labor-intensive per-language engineering. 
Recent advances %provide supporting capabilities for 
support static cross-language analysis~\cite{roth2024axa,zhang2025interactive}, whose potential for detecting cross-language bugs has yet to be demonstrated. More importantly, they require separate, mature analysis infrastructure for each language, which is not always available (e.g., for Python). 
%Moreover, as a common barrier to static analysis in general, these approaches suffer both imprecision~\cite{wei2018jn} due to their conservative nature and limited recall due to their inability to analyze dynamic language constructs which prevalent in modern languages~\cite{wen22usenixsecurity}. 
As showcased lately, \textit{ML-based} cross-language bug detection~\cite{yang2024learning} may potentially complement both static and dynamic approaches. 
Unfortunately, they struggle to generalize to new and unseen codebases, and their performance is highly dependent on the quality and quantity of training data, which (e.g., labeled buggy datasets~\cite{yang2025dissecting}) are particularly lacking in the domain of multi-language software.
Additionally, extant static, dynamic, and ML-based techniques are commonly limited in analyzing challenging language features (e.g., dynamic code constructs) hence 
missing highly stealthy cross-language bugs (e.g., those buried in implicit information flow). 

%To address semantic disparities between different languages, existing static techniques for multi-language software rely on heavy language-specific analyses, such as computing abstract summaries of native code or defining semantic rules for each interoperation API
%
%Tools like Broaden Horizon (Lee et al., 2020) and AXA (Park et al., 2023) attempt to address this by defining language-specific semantic rules or abstract summaries for interoperability APIs (Youn et al., 2023), but these require labor-intensive per-language engineering, rendering them inflexible for new language combinations. For instance, modeling Python-C interactions demands distinct logic from Java-JNI analysis, stifling extensibility.
%
%Static approaches like MLQL (SPE’24) and AXA (ASE’24) use coarse-grained models that overlook implicit flows, while Broaden Horizon (ASE’20) lacks support for dynamic language features.
%
%Static approaches like MLQL (SPE’24), AXA (ASE’24), and Broaden Horizon (ASE’20) have shown promise but are frequently criticized for their coarse-grained nature, low precision, and limited practicality—often requiring separate analysis infrastructures for each language.

%Existing solutions to cross-language vulnerability detection suffer from major limitations. Static approaches like MLQL (SPE’24), AXA (ASE’24), and Broaden Horizon (ASE’20) have shown promise but are frequently criticized for their coarse-grained nature, low precision, and limited practicality—often requiring separate analysis infrastructures for each language. Dynamic testing, including our group’s prior work, depends heavily on either handcrafted or randomly generated inputs that can rarely achieve complete code coverage. Similarly, deep learning-based methods such as xLoc struggle with generalizability, being overly reliant on the quality and scope of training data. These challenges motivate us to pursue a promising direction: a static, fine-grained, cross-language information flow analysis that strikes a better balance between precision and scalability.
%
%Existing solutions for detecting cross-language vulnerabilities have several shortcomings that limit their effectiveness and practicality. Static analysis tools like MLQL, AXA, and Broaden horizon often lack the granularity needed to accurately identify subtle cross-language interactions, resulting in low precision and a high rate of false positives. Moreover, these tools can be challenging to use in practice due to their limited support for diverse language combinations and the need for specialized expertise to interpret their results. Dynamic analysis techniques, while capable of detecting vulnerabilities at runtime, are constrained by their dependence on test inputs, which may not fully cover all possible execution paths and cross-language interactions. Deep learning-based approaches such as xLoc show promise in learning vulnerability patterns from code, but they often struggle to generalize to new and unseen codebases, and their performance is highly dependent on the quality and quantity of training data. The limitations of these existing solutions underscore the need for a more robust, precise, and scalable approach to cross-language vulnerability detection.
%
%Existing solutions inadequately address these challenges. Static approaches like MLQL (SPE’24) and AXA (ASE’24) use coarse-grained models that overlook implicit flows, while Broaden Horizon (ASE’20) lacks support for dynamic language features. Dynamic tools (e.g., cross-language fuzzers) are constrained by test input coverage, missing flows triggered by rare program states. Deep learning-based detectors (e.g., xLoc) struggle with generalizability, as their accuracy depends on the representativeness of training data. A promising alternative—static, fine-grained cross-language information flow analysis—remains elusive due to four interrelated challenges: (1) semantic disparities (e.g., C’s pointer arithmetic vs. Python’s object references), (2) interface diversity (e.g., Python’s ctypes vs. Java JNI), (3) dynamic language features (e.g., Python’s eval or metaprogramming), and (4) the precision-scalability tradeoff inherent to static analysis.

% what we do and the challenges in doing that
In this paper, we aim to \textit{statically} analyze \textit{cross-language information flow} while overcoming the %aforementioned 
limitations of extant approaches. %, through traditional static code analysis working synergistically with foundation large language models (LLMs) as an agent-based framework. 
%The intuition/rationale is that LLMs have shown great potential for understanding code across different languages~\cite{fang2024large,linlarge25ndss} and traditional program analysis may be effectively assisted by LLMs to deal with its inherent barriers~\cite{li2024enhancing,xie2024resym}. 
Static information flow analysis %(a.k.a static taint analysis) 
is a fundamental technique for vulnerability discovery~\cite{myers1999jflow,ferraiuolo2017verification,jovanovic2006pixy,huang2015supor,nan2015uipicker,li2025iris}, which formulates the detection of various kinds of vulnerabilities as a source-sink problem (with sources/sinks defined accordingly). It has %drawn great attention and 
been widely used in practice (e.g., underlying GitHub CodeQL~\cite{github_codeql} and Facebook Infer~\cite{calcagno2011infer}) \textit{for single-language software}. 
However, %in light of the known shortcomings of each and given the complexity of multi-language code, fulfilling our aim comes with  
developing a static information flow analysis\textit{across language boundaries} faces several key challenges.  

First (\textit{Challenge-1}), %the disparate language semantics pose a substantial barrier, especially for a static analysis. 
%(e.g., differences in type systems and memory management mechanisms)
different languages define and handle constructs (e.g., type systems, memory management, and control flow) differently. 
These %differences 
semantics disparities 
complicate the creation of a unified (especially static) analysis framework capable of 
accurately interpreting and reasoning about code across languages. 
Second (\textit{Challenge-2}), diverse language features (e.g., function pointers and inline assembly in C), especially %those due to 
dynamic code constructs (e.g., dynamic typing and reflection in Python), 
%result in intricacies that classical static analysis techniques struggle to address, even for single-language code. 
%These features 
can obscure the flow of information and make it difficult to analyze %program behavior at compile time, even for single-language code. 
even single-language code at compile time. 
Dealing with such features in/across multiple languages %, especially those inducing complex cross-language behaviors, 
is only harder. %more challenging. 
%Third (\textit{Challenge-3}), balancing cost-effectiveness while maintaining the scalability of fine-grained analysis is a long-standing challenge, which is only exacerbated for cross-language analysis---multi-language systems tend to have larger codebases to incur higher analysis costs, while offering a reasonable level of effectiveness (accuracy) is key for practical security applications of the analysis. 

These intrinsic static-analysis challenges could be tackled by large language models (LLMs), given their demonstrated potential for code understanding~\cite{fang2024large,linlarge25ndss} and reasoning~\cite{li2024enhancing,xie2024resym,li2025iris}. 
Yet (\textit{Challenge-3}), LLMs are not magic boxes---merely delegating a complex task like cross-language analysis to them may not help much. 
For one thing, their token/context-size limits %, it is not always feasible to even pass a single function to it
make it infeasible to feed them with the entire system, especially as multi-language codebases tend to be larger  
than single-language ones. Analyzing one function at a time alleviates this barrier, but the LLMs would not capture even %critical 
interprocedural context, not to mention 
inter-language effects---both of which are essential for effective cross-language analysis. 
%intraprocedural analyses 
For another, 
LLMs %are well-known to suffer hallucinations, l
may hallucinate, %likely producing unstable and even spurious results. 
producing spurious results~\cite{li2024enhancing,xie2024resym}.


%First, disparate language semantics—such as differences in type systems and memory management—pose a substantial barrier (Challenge 1). Second, the diversity of programming languages, their combinations, and the variety of interfacing mechanisms can severely undermine extensibility (Challenge 2). Third, dynamic language features, with their runtime-dependent behavior, introduce intricacies that classical static analysis techniques struggle to address (Challenge 3). Finally, there is a pressing need to balance cost-effectiveness with analysis precision: designing an approach that scales without compromising on the depth and accuracy of vulnerability detection (Challenge 4).

%Developing a static, fine-grained cross-language information flow analysis presents a multifaceted challenge, requiring careful consideration of several key factors. First and foremost is the issue of language semantics disparity, which arises from the differences in type systems, memory management mechanisms, and other language-specific features that govern how data is represented and manipulated. These disparities can lead to subtle yet critical vulnerabilities when data flows across language boundaries without proper validation or conversion. Second, the diversity of languages and language combinations, along with their corresponding interfacing mechanisms, poses a significant challenge to the extensibility and scalability of any cross-language analysis. Supporting a wide range of languages and their interactions requires a flexible and modular analysis framework that can adapt to new language features and interfacing paradigms. Third, the presence of dynamic language features, such as dynamic typing and reflection, introduces inherent challenges to static analysis, as these features can obscure the flow of information and make it difficult to reason about program behavior at compile time. Finally, balancing cost-effectiveness while maintaining the scalability of fine-grained analysis is a critical consideration, as the analysis must be both precise enough to detect subtle vulnerabilities and efficient enough to handle large and complex codebases without incurring excessive computational overhead. Addressing these challenges requires a holistic approach that combines the strengths of static analysis, dynamic analysis, and machine learning techniques.

%Designing a static cross-language analysis requires confronting these challenges head-on. First, reconciling divergent language semantics—such as C’s manual memory management with Python’s garbage collection—complicates data flow tracking, as aliasing and lifetime assumptions differ radically. Second, supporting heterogeneous interfacing mechanisms (e.g., foreign function interfaces, shared memory) demands an extensible framework, which existing monolithic tools lack. Third, dynamic features like runtime code generation or duck typing defy traditional static analysis, leading to under-constrained models. Finally, overly precise analyses (e.g., symbolic execution) become computationally intractable for large codebases, while overly coarse ones miss subtle vulnerabilities.

% what we do and how we (and what key insights we leverage to) deal with the challenges above
\begin{comment}
To overcome 
Overcoming
such challenges, we developed {\tech}, \textit{a context-, flow-, and path-sensitive cross-language static information flow analysis} via traditional static analysis working synergistically with foundation LLMs as an \textit{agentic} framework. 
%The intuition/rationale is that LLMs have shown great potential for understanding code across different languages~\cite{fang2024large,linlarge25ndss} and traditional program analysis may be effectively assisted by LLMs to deal with its inherent barriers~\cite{li2024enhancing,xie2024resym}. 
Specifically, harnessing the capabilities of LLMs in bridging semantic and syntactic gaps across languages, 
{\tech} resolves (especially implicit) control flow and propagates taints both within and across languages, for addressing \textit{Challenge-1}. 
However, LLMs are known to suffer from insufficiency in code reasoning, tendency to hallucinate, and limited context window sizes. %, for which the traditional 
To counter these issues, the static analysis guides the LLMs 
%static analysis provides close, context-aware guidance and mutual validation 
while narrowing down their analysis scope via a cross-language interprocedural control flow graph (CICFG). 
A multi-LLM negotiation and arbitration component, called \textit{expert panel}, is designed to further mitigate hallucinations and inaccuracy. 
%
%hence improving stability and accuracy of LLM-based results. 
Moreover, {\tech} explicitly identifies and handles language features that are challenging to static analysis and/or introduce implicit data/control flow throughout the multilingual code, while aiming to achieve analysis soundness via a fixed-point iteration of feature handling, hence addressing \textit{Challenge-2}. 
Importantly, {\tech} works in two main phases, first augmenting the CICFG hence enabling context-sensitive control-flow-based taint approximation, followed by LLM-driven path-sensitive taint propagation. %, while still explicitly dealing with language features inducing data flows that are implicit and/or hard to resolve. 
This multi-staged, refinement-based strategy, along with basing the traditional static analysis on a scalable, query-based analysis framework, addresses \textit{Challenge-3}.
\end{comment}
Overcoming
such challenges, we developed {\tech}, \textit{a context-, flow-, and path-sensitive cross-language static information flow analysis} via traditional static analysis working synergistically with foundation LLMs as an \textit{agentic} framework. 
%The intuition/rationale is that LLMs have shown great potential for understanding code across different languages~\cite{fang2024large,linlarge25ndss} and traditional program analysis may be effectively assisted by LLMs to deal with its inherent barriers~\cite{li2024enhancing,xie2024resym}. 
Given a multi-language system, we start with a lightweight cross-language interprocedural analysis, resulting in an approximate (incomplete and imprecise) representation of the whole system with only explicit control/data flow facts. 
Based on this representation, the static analysis works further as the agent's controller, invoking LLMs to analyze implicit flow facts, hence potentially augmenting the representation and propagating information between given sources and sinks through the system, so as to address \textit{Challenge-1}. 
To identify and resolve the implicit flows, which are induced by respective language features, 
we elicit the LLMs' relevant knowledge via few-shot in-context learning, while aiming to achieve analysis soundness via a fixed-point iteration of feature handling, hence addressing \textit{Challenge-2}. 
Importantly, the static analysis coordinates interprocedural and inter-language contexts, which allows the LLMs to only provide complementary assistance (e.g., 
handling the challenging features) in a minimal scope (a function or a control-flow path) on demand. 
Moreover, we leverage multiple LLMs formed as a negotiation/arbitration component, called \textit{expert panel}, to cross-validate results of every LLM query, 
while using static-analysis-produced facts to check those results. 
The careful guidance (adaptive scoping, context management, and fact checking) and negotiated-agreement procedure together address \textit{Challenge-3}.


%Our work leverages several core insights to systematically address these challenges. By harnessing the code comprehension capabilities of foundation large language models (LLMs), we mitigate the issues raised by language semantic disparities and interface diversity (addressing Challenges 1 and 2). Close-guidance integration with classical static analysis—embodied by representations such as CICFG—helps counteract LLMs’ inherent limitations in deep reasoning and context capturing, while explicitly identifying and managing dynamic language features to surmount Challenges 3 and 4. Furthermore, we adopt a scalable, query-based analysis paradigm, complemented by iterative, fixed-point refinement, thereby striking an effective balance between precision, scalability, and recall.

%To overcome these challenges, we propose a novel approach that leverages the strengths of Large Language Models (LLMs) and traditional static analysis in a synergistic manner. LLMs possess a remarkable ability to understand code written in various programming languages, enabling them to bridge the gap between different language semantics and identify potential vulnerabilities that might be missed by traditional static analysis techniques. However, LLMs also have limitations, including insufficient reasoning capabilities, limited context understanding, and a tendency to hallucinate or generate incorrect code. To mitigate these limitations, we use static analysis, represented by Combined Interprocedural Control Flow Graph (CICFG), to guide the LLM and provide it with a more structured and context-aware understanding of the code. Additionally, we explicitly identify and handle language features that are challenging to static analysis, such as dynamic typing and reflection, to improve the precision and recall of our analysis. Finally, we employ a scalable, query-based analysis paradigm, refined through close collaboration and mutual correction/enhancement between LLMs and static analysis, and dispatch an iterative fixed-point analysis update until convergence, ensuring analysis soundness and scalability.

%PolyFlow addresses these challenges through three synergistic innovations. First, it leverages foundation LLMs to bridge semantic and syntactic gaps across languages (C1, C2): LLMs parse multilingual code to infer cross-language data flows, while static constructs like Cross-Language Interprocedural Control-Flow Graphs (CICFG) ground these inferences in traditional analysis, mitigating hallucinations. Second, PolyFlow explicitly identifies and resolves dynamic language features (C3) via an iterative fixed-point process, where potential implicit flows (e.g., taint propagation through exception handlers) are incrementally validated and refined. Third, a hybrid query-based architecture balances precision and scalability (C4): lightweight static analysis (via Joern) extracts candidate flows, which LLMs then refine, iterating until convergence. This collaboration ensures scalability without sacrificing fine-grained accuracy.

% Implementation and evaluation 
For evaluation purposes, we implemented {\tech} for Python-C systems %using a query-based static analyzer, 
given their high and lasting popularity (e.g., in the impactful AI/ML software ecosystem)~\cite{wen22fse,li2024multilingual,yang2024multi} 
%~\cite{wen22fsetool,wen22fse,li2021understanding,li2024multilingual} 
and that existing multilingual code analyzers mostly target other combinations (e.g., Java-C~\cite{xue2018ndroid,lee2020broadening,hwang2021justgen,bae2019towards}). 
%
%To enhance its usability, {\tech} also comes with an automatic source/sink identification preprocessing module. 
%
%Following these insights, we designed PolyFlow as a synergistic framework that unfolds in two main phases. The first phase entails an initial static analysis to construct code representations and candidate flows, leveraging traditional tools to capture the program’s structural nuances. In the second phase, foundation LLMs are engaged in a close, iterative collaboration with static analysis outputs to refine the flows—resolving implicit flows and achieving fixed-point convergence. This dual-phased strategy enhances both the precision and the usability of the final vulnerability analysis.
%
%Guided by these insights, we developed PolyFlow, a purely static information flow analysis framework that harnesses the power of foundation LLMs and traditional static analysis in a synergistic manner. PolyFlow excels at identifying implicit flows that conventional static analysis often struggles to resolve due to dynamic language features, thanks to its fixed-point iterative feature handling process. PolyFlow operates in two primary phases: first, a static analysis phase constructs a CICFG to represent the code's structure and data flow; second, an LLM-guided phase refines the information flow by addressing dynamic language features and cross-language interactions, leveraging the LLM's ability to understand code semantics and identify potential vulnerabilities.
%
%PolyFlow operates in two phases. The static foundation phase constructs a CICFG using lightweight static analysis, capturing cross-language call graphs and data dependencies. The LLM-agent phase iteratively refines this graph: LLMs resolve ambiguities (e.g., dynamic dispatch in Python) by generating context-aware hypotheses, which are validated against static constraints (e.g., type consistency). For instance, when analyzing a Python-C extension, PolyFlow detects a PyObject passed to C, queries the LLM to infer possible C-level type casts, and cross-checks these against C’s pointer semantics. This process repeats, with each iteration narrowing the analysis until a fixed point is reached, ensuring sound handling of implicit flows.
%
%
%
To rigorously validate {\tech}, we curated \textit{xFlowBench}, the first cross-language static analysis benchmark with ground-truth information flow facts with respect to 
different language features. 
We then applied {\tech} to 14 real-world multi-language systems of diverse scales and application domains, while comparing it to various kinds of state-of-the-art (SOTA) 
%code-analysis- and learning-based 
baselines. %(MultiQL~\cite{youn2023declarative}, xLoc~\cite{yang2024learning}, PolyCruise~\cite{wen22usenixsecurity}, and PolyFuzz~\cite{wen23usenixsecurity}). 
%
%evaluated it on a comprehensive suite of benchmarks, including both microbench and real-world projects that span Python and C. This language combination is strategically chosen; Python’s dynamic features and C’s low-level intricacies represent a challenging yet representative set of languages in multilingual systems, ensuring that our evaluation addresses realistic and critical vulnerabilities in modern software deployments.
%
%To evaluate the effectiveness of PolyFlow, we conducted experiments on both microbenchmarks and real-world Python-C projects, selected for their relevance and representativeness of common cross-language interactions. Python, a high-level dynamic language, is frequently interfaced with C for performance-critical tasks, making it a prime target for cross-language vulnerabilities that can arise from improper data handling or memory management across the language boundary. By targeting Python-C interactions, we can assess PolyFlow's ability to handle the challenges posed by dynamic language features and cross-language semantics disparity.
%
%We evaluate PolyFlow on 15 microbenchmarks and 8 real-world Python-C projects, including NumPy and SciPy—critical targets due to Python’s dominance in AI/ML and its reliance on C for performance. Python-C systems exemplify the analysis challenge: Python’s dynamism (e.g., decorators, \_\_getattr\_\_) interacts unpredictably with C’s low-level memory operations. PolyFlow achieves 92\% precision and 88\% recall, outperforming MLQL (67\% precision) and AXA (58\% recall). It uncovered 15 previously unknown vulnerabilities, including a buffer overflow in a NumPy C extension where Python’s dynamic array reshaping was mishandled in C.
%
%Our empirical evaluations demonstrate that PolyFlow significantly outperforms existing techniques in detecting cross-language vulnerabilities. Across microbench scenarios, PolyFlow achieved high precision and recall, effectively resolving implicit flows that conventional static analyses miss. In real-world Python-C projects, our framework not only uncovered previously undetected vulnerabilities but also maintained scalable performance, underscoring its practicality and potential for broader adoption.

Our extensive experiments reveal {\tech}'s promising cost-effectiveness and scalability. 
On the microbench, {\tech} achieved 97.9\% precision, 87.3\% recall, and 91.8\% F1. On the real-world systems, it achieved 81.2\% precision and discovered 8 previously unknown, exploitable cross-language vulnerabilities---none of which are found by any of the baselines. 
%of which ?? could not be found by any of the baselines
%
% ---with ?\%--?\% higher precision. 
%For source/sink identification, it attained ?\% precision and ?\% recall. 
Ablation studies confirmed that each of its key design elements/components contributes significantly to its overall performance. 
{\tech} also reasonably scales to large-scale systems, incurring 12.62 hours and 380 MB peak memory on average per project; 
%in comparison, the best-performing (for vulnerability discovery) baseline took ?? hours with ?? MB peak memory. 
In terms of LLM costs, {\tech} only consumes on average 3.67 M tokens 
% and \$?? 
to analyze each multi-language system. 
%
%PolyFlow achieves high precision and recall in detecting cross-language vulnerabilities, surpassing existing static and dynamic analysis techniques. PolyFlow's ability to effectively address the challenges of language semantics disparity, language diversity, dynamic language features, and cost-effectiveness makes it a practical and scalable solution for securing multilingual software systems. These results underscore the potential of LLM-guided static analysis as a powerful tool for vulnerability detection and software assurance.

%PolyFlow reduces false positives by 40\% compared to MLQL and identifies 3× more true positives than AXA. Its LLM-agent resolved 85\% of dynamic feature-induced ambiguities (e.g., implicit flows via Python’s @property decorators), validating its iterative refinement process. The hybrid approach also scales to 500k-LoC codebases, demonstrating practical applicability.

%Through {\tech}, we demonstrated
{\tech} showcases
a novel neuro-symbolic, agentic approach % of combining traditional static analysis with LLMs for 
%to practical cross-language information flow analysis, where unlike in typical LLM-based agents the static analysis makes main decisions (not the LLMs). 
to %cross-language 
code analysis.  
Instead of LLM-based agents invoking external (symbolic) %-reasoning) 
tools, our agent is \textit{centered around a static analyzer},
which judiciously (1) utilizes LLMs where they offer the most value while traditional analysis falls short, 
(2) decides when, where, and how to employ LLMs while supplying contexts on demand, and (3) integrates LLM outputs as intermediate results to the analysis, 
hence combining the strengths of both methods while overcoming each other's shortcomings---the \textit{key insight and takeaway} of our work. 
%
%While for design validation we only implemented it for Python-C so far, the methodology can be applied to other language combinations, especially given the support of both the underlying static analysis framework and LLMs for different languages. 
%In summary, 
Our main contributions include: 

\begin{itemize}[leftmargin=*,topsep=2pt]
    \item {\tech}, a novel static %, fine-grained (statement-level) 
    %information flow 
    analysis of multi-language software that %synergistically integrates foundational LLMs with traditional static analysis to 
    holistically addresses cross-language %vulnerabilities, particularly those via implicit flows or 
    information flow, including implicit ones and those 
    induced by language features challenging to existing analyses ($\S$\ref{sec:technique}).

    \item An open-source implementation of {\tech} for Python-C software, which works with real-world % large-scale 
    systems across various scales and domains ($\S$\ref{sec:implementation}).
    
    \item \textit{xFlowBench}, an open multilingual static analysis benchmark, which %to the best of our knowledge also 
    is the first such benchmark with ground-truth cross-language information flow facts %analysis techniques, which is the first multilingual static analysis benchmark suite publicly available as we know 
    as we know
    ($\S$\ref{sec:microbench}).

    \item A comprehensive evaluation of {\tech} on both the micro-benchmarks and real-world multi-language systems, which demonstrates its promising merits in  
    cross-language analysis effectiveness and vulnerability discovery superior to SOTA baselines ($\S$\ref{sec:eval}). 
\end{itemize}

%**Contributions.**  

%- **Novel Problem Formulation:** Precisely defining the challenges inherent in cross-language vulnerability detection in multilingual systems.  
%- **Innovative Framework:** Introducing PolyFlow, a static information flow analysis framework that synergizes foundation LLM capabilities with conventional static analysis.  
%- **Overcoming Dynamic Complexity:** Establishing effective methods to handle implicit flows and dynamic language features through iterative fixed-point refinement.  
%- **Scalable and Precise Analysis:** Achieving a cost-effective balance between scalability and fine-grained vulnerability detection using a hybrid analysis paradigm.  
%- **Rigorous Evaluation:** Demonstrating substantial performance and practical utility in both microbench and real-world Python-C projects, setting a new baseline for multilingual vulnerability analysis.

%Our contributions can be summarized as follows:
%
%We introduce PolyFlow, a novel static information flow analysis framework that synergistically combines LLMs and traditional static analysis to enhance cross-language vulnerability detection.
%We present a comprehensive approach to handling implicit flows and dynamic language features in cross-language contexts, enabling more precise and accurate vulnerability detection.
%We propose a scalable and cost-effective design that balances precision and applicability, making PolyFlow suitable for analyzing large and complex multilingual software systems.
%We provide an evaluation on real-world Python-C projects that demonstrates the effectiveness of PolyFlow in detecting cross-language vulnerabilities, showcasing its potential as a valuable tool for software developers and security professionals.


% Contributions

% Unified Framework: The first static analysis framework to synergize LLMs and traditional static analysis for cross-language vulnerability detection, resolving both explicit and implicit flows.

% Semantic Bridging: A novel method using LLMs to infer cross-language semantics, grounded by CICFG to ensure robustness against hallucinations.

% Dynamic Feature Resolution: An iterative fixed-point algorithm to handle dynamic language features, ensuring soundiness without sacrificing scalability.

% Real-World Impact: Discovery of 15 critical vulnerabilities in widely-used Python-C projects, underscoring practical relevance.

% Open Artifact: Publicly available implementation, benchmarks, and reproducibility guidelines to advance research in multilingual security.

% PolyFlow redefines cross-language analysis, offering a scalable, precise solution for securing the multilingual foundations of modern software.

\noindent
The full 
{\tech} artifact %(code, datasets, documentation) is 
has been made available~\cite{polyflowAE}. 
%Our artifact is available at https://figshare.com/s/c8afb649409e3db9db65. 

==> Sections/01_intro.tex <==

\section{Introduction}


==> Sections/02_background-cai.tex <==
%!TEX root = paper.tex
\section{Background and Motivation}\label{sec:bkgmotive}
We introduce concepts in cross-language code analysis, and motivate our work via an 
example and a broader study. 
%a study that reveals challenges to static information flow analysis of multilingual code. 

\subsection{Multilingual Code Construction}

%Multi-language software refers to systems that incorporate multiple computer languages \textit{that interact}. The interactions %between languages 
%typically rely on \textit{Foreign Function Interfaces (FFIs)}, which enable cross-language communication through specific APIs. For example, Python and C each provide distinct FFI mechanisms---Python through the \textit{ctypes} library and C-extensions.

Multi-language systems are software written in multiple computer languages \textit{that interact}, where the program is referred to as \textit{multilingual code/program}.
The interactions %between languages 
typically rely on \textit{Foreign Function Interfaces (FFIs)}, a mechanism that enables code written in one (host) language to call functions written in another (guest) language. 

For example, Python provides FFIs for cross-language interfacing with C via modules like \textit{ctypes} and C-extensions. 
In particular, such interfacing involves two main types of \textit{cross-language functions}: native functions and foreign functions. Native functions are implemented by developers in a guest language to be invoked in the host language code, %different from the caller’s language, 
while foreign functions are provided by the host language to facilitate interoperability with the guest language code.

%A Foreign Function Interface (FFI) enables a program written in one programming language (the host) to call functions or use services written in another language (the guest). This interoperability is crucial for leveraging existing libraries, optimizing performance, or integrating components across different programming environments.

%Cross-language interfacing involves two primary function types: native functions and foreign functions. Native functions are implemented by developers in a language different from the caller’s language, while foreign functions are language-provided utilities that facilitate interactions with external code.


%To enable holistic static analysis of multi-language codebases, we introduce the \textbf{Cross-language Interprocedural Control Flow Graph (CICFG)}, a unified representation that captures control flow across language boundaries. Our methodology begins by constructing intraprocedural control flow graphs (CFGs) for individual methods generated by Joern, an industry static analyzer. These CFGs are then extended into an Interprocedural CFG (ICFG) by linking callers to callees and connecting return sites. Finally, we bridge language gaps by resolving foreign function calls, producing the complete CICFG. In this graph, nodes correspond to statements, and edges represent control flow relationships between them.



%we introduce the \textbf{Cross-language Interprocedural Control Flow Graph (CICFG)}, a unified representation that captures control flow across language boundaries. Our methodology begins by constructing intraprocedural control flow graphs (CFGs) for individual methods generated by Joern, an industry static analyzer. These CFGs are then extended into an Interprocedural CFG (ICFG) by linking callers to callees and connecting return sites. Finally, we bridge language gaps by resolving foreign function calls, producing the complete CICFG. In this graph, nodes correspond to statements, and edges represent control flow relationships between them.



% The CICFG provides a foundation for holistic static analysis of multi-language software, addressing a key limitation in existing approaches that struggle with cross-language dependencies.


% In multilingual codebases, the interfacing points between languages typically rely on Foreign Function Interfaces (FFIs), which enable language-level communication through defined APIs. Common FFIs include Python's \textit{ctypes} and C-extensions, Java's Native Interface (JNI), and JavaScript's bindings with WebAssembly. These interfaces facilitate data exchanges, type conversions, and memory management across languages, but the complexity of handling different semantic models at these interfaces creates potential vulnerabilities.

% To frame our discussion, we introduce several terminologies frequently employed in multilingual software analysis:
% \begin{itemize}[leftmargin=*,topsep=2pt]
%     \item \textbf{Cross-language Interprocedural Control Flow Graph (CICFG):} A unified graph representation that explicitly models interprocedural control flow across programming language boundaries. 
%     \item \textbf{Cross-Language Interface (CLI):} The explicit boundary where languages communicate and exchange data.
%     \item \textbf{Implicit Flow:} Data flows that are not explicitly defined but arise through control-flow or language semantics mismatches.
% \end{itemize}

% These terminologies provide a foundation for understanding the complexities inherent in multilingual software analysis.

\subsection{Motivating Example}
Different from those in a single-language program, vulnerabilities in multilingual code  may be rooted in vulnerable cross-language information flow~\cite{wen22fse,staicu2023bilingual}, where the information source lies in one language while the sink is located in another~\cite{wen22usenixsecurity}. 
Apparently, the vulnerabilities will be missed if we only analyze one language component. 
Moreover, certain language features may lead a static analyzer to miss even the intra-language flow segments, hence breaking the entire cross-language flow.  


% \begin{tcolorbox}[title=Motivating Example (from the Cvxopt project), 
%                   fonttitle=\bfseries\small, 
%                   colback=blue!5!white, 
%                   colframe=blue!50!black]
% \begin{minted}[fontsize=\scriptsize]{python}
% # Python: @app.route decorator obscures control flow
% @app.route('/process')  # SOURCE (user input)
% def process_data():
%     user_input = request.args.get('data')
%     c_module.validate(user_input) # native call
% \end{minted}

% \begin{minted}[fontsize=\scriptsize]{c}
% // C: Function pointer prevents control flow resolution
% void (*validator)(char*);  // Flow broken here

% void validate(char* input) {
%     if(validator) 
%         validator(input); // SINK (format-string vuln)
% }
% \end{minted}
% \end{tcolorbox}

\begin{figure}[t]
\centering
\begin{minipage}{0.48\textwidth}
%\begin{compactcode}
\begin{minted}[fontsize=\scriptsize]{python}
# Python: @app.route decorator obscures control flow
@app.route('/process')  # SOURCE (user input)
def process_data():
    user_input = request.args.get('data')
    c_module.validate(user_input) # native call
\end{minted}
%\caption{Python entry point with decorator}
%\label{fig:python-code}
%\end{compactcode}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
%\begin{compactcode}
\begin{minted}[fontsize=\scriptsize]{c}
// C: Function pointer prevents control flow resolution
void (*validator)(char*);  // Flow broken here

void validate(char* input) {
    if(validator) 
        validator(input); // SINK (format-string vuln)
}
\end{minted}
%\caption{C validation with function pointer}
%\label{fig:c-code}
%\end{compactcode}
\end{minipage}
%\caption{An example cross-language vulnerability.}
\caption{Code snippet adapted from the {\cvxopt} project.}
\label{fig:vuln-example}
\end{figure}

Consider the example of Figure~\ref{fig:vuln-example}, code snippet from a real-world Python-C project \Cvxopt. 
When handling optimization requests, user-submitted data enters through a Python endpoint registered via Flask's \colorbox{lightgray}{@app.route} 
%@app.route 
decorator, a challenging language feature that obscures control flow, where the input is collected without proper sanitization. 
This tainted data then crosses into C through a native module interface %(native\_module.validate()). 
(\colorbox{lightgray}{native\_module.validate()}). 
Within the C validation logic, a function pointer indirection %(void (*validator)(char*)) 
(\colorbox{lightgray}{void (*validator)(char*)})     
dynamically dispatches the input to a {\tt printf}-like sink, creating a format-string vulnerability exploitable through malicious payloads. 

Existing static analyzers may miss this critical flow: Python-focused tools may fail to recognize the decorator-registered route as an entry point, while C-focused analyzers stop tracking flow at the unresolved function pointer call. Moreover, without analyzing the cross-language flow from Python's HTTP handler to C's format-string sink, this
multilingual code vulnerability will not be detected. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\columnwidth]{Figures/func_pointer.pdf}
%       \caption{Function pointer real-world usage. The call path of the function pointer \code{word2bool} is marked with green lines.}
%     \label{fig:motivatingexample}
% \end{figure}
% The use of function pointers introduces indirect control-flow edges. The function \texttt{word2bool} (declared in line 1) is a utility function converting data from type \texttt{word} to \texttt{bool}, crucial for conditional decisions. It passes to the function \texttt{findletters} (line 2), which is declared in line 3, accepting function pointer \texttt{word2bool} as the third parameter \texttt{tobool} and invoking function \texttt{getsig} (line 7) declared in line 10, inside which the function \texttt{word2bool} is eventually invoked in line 19. Traditional static analyses struggle to resolve such indirect calls due to the dynamic nature of function pointers, causing incomplete CICFGs that miss these critical edges.

% start with CFG by Joern, enabled by, we define interprocedual control flow graph. based on ICFG for each language, we then connect the   for foreign language and native and get holistic graph. Each node is a statement, each edge represents a control flow relationship.



\subsection{Motivating Study}
%To systematically identify language features that challenge static analysis in cross-language environments beyond function pointers, we conducted a comprehensive investigation through three approaches: (1) analysis of prominent open-source Python-C projects, (2) review of developer discussions and technical blogs, and (3) empirical evaluation of static analysis tools. We analyzed prominent open-source Python-C projects mined from GitHub, building upon the dataset curated in the prior study on cross-language bugs~\cite{yang2025dissecting}. This analysis involved forward and backward traversals of cross-language information flows, using CICFG-based inspection to pinpoint critical locations and root causes of cross-language bugs. The study highlighted specific Python and C constructs—such as dynamic typing and language-specific APIs—that frequently hinder static analysis. This process revealed 14 problematic features across Python and C that significantly impede static analysis. We evaluated these features' impact on CFG generation by assessing Joern's ability to correctly process each case, with detailed results presented in Table \ref{tab:motivation-study}.
%
In Figure~\ref{fig:vuln-example}, the challenging features (decorators and function pointers) obstruct intra-language analysis, hence breaking the flow across the language boundary. These features often cause implicit information flow, which may bear stealthy vulnerabilities. 
%
To understand this problem, we intend to systematically identify such language features that challenge static analysis. %in multi-language environments. 
We again started for Python-C, and took a three-pronged study methodology: (1) analysis of prominent open-source Python-C projects on GitHub (including those in cross-language bug datasets~\cite{wen22fse,yang2025dissecting}), (2) review of developer discussions and official language documentation, and (3) empirical evaluation of popular static analysis tools. Via manual inspection, we track cross-language information flows to pinpoint critical locations and root causes of cross-language bugs in relation to specific Python and C %constructs 
features %---such as dynamic typing and language-specific APIs---
that frequently hinder the static analyzers (e.g., by breaking their control/data flow tracking). 

%This process identified 14 problematic features across both languages that significantly impede static analysis, whose impact on CFG generation we evaluated through Joern's ability to correctly process each case, with detailed results presented in Table~\ref{tab:motivation-study}.


\setlength{\tabcolsep}{2pt}
\begin{table}[tp]
\centering
%\caption{Summary of challenging language features and their support status in Joern and \tech, where $\protect\yes$ indicates support and $\protect\no$ indicates lack of support}
\caption{Challenging language features, impact on analysis, and support by various analyzers 
($\protect\yes$: support, $\protect\no$: no support, $\protect\rhalf$: partial/limited support, $\protect\cmark$: missing, -: no impact)}
% \resizebox{\columnwidth}{!}{%
% \renewcommand{\arraystretch}{0.9}
% \small
% \begin{tabular}{@{}lllcccc@{}}
% \toprule
% \textbf{Lang} & \textbf{Feature} & \textbf{Joern} & \textbf{Ent.} & \textbf{Flow} & \textbf{SA} & \textbf{LLM} \\
% \midrule
% \multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
% & Function Pointers & \xmark & -- & \cmark & -- & \cmark \\
% & Conditional Compilation & \xmark & \cmark & \cmark & -- & \cmark \\
% & External Functions & \xmark & \cmark & \cmark & -- & \cmark \\
% & Inline Assembly & \xmark & -- & \cmark & -- & \cmark \\
% & Macro Function Calls & \xmark & -- & \cmark & -- & \cmark \\
% & Goto Statements & \xmark & -- & \cmark & -- & \cmark \\
% & Setjmp/Longjmp & \xmark & -- & \cmark & -- & \cmark \\
% & Recursive Functions & \cmark & -- & -- & -- & \cmark \\
% \midrule
% \multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
% & Decorators & \xmark & -- & \cmark & -- & \cmark \\
% & First-Class Functions & \xmark & -- & \cmark & -- & \cmark \\
% & Lambda Functions & \xmark & \cmark & \cmark & -- & \cmark \\
% & Generators/Coroutines & \cmark & -- & -- & -- & \cmark \\
% & Reflection & \xmark & -- & \cmark & -- & \cmark \\
% & Dynamic Imports & \xmark & \cmark & \cmark & -- & \cmark \\
% \bottomrule
% \end{tabular}%
% }


% \resizebox{\columnwidth}{!}{%
% \renewcommand{\arraystretch}{0.85}
% \footnotesize
% \begin{tabular}{@{}llcccccc@{}}
% \toprule
% \textbf{Lang} & \textbf{Feature} & \textbf{Joern} & \textbf{CodeQL} & \textbf{Infer} & \textbf{SonarQube} & \textbf{Clang-SA} & \textbf{PolyFlow} \\
% \midrule
% \multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
% & Function Pointers & \xmark & \cmark & \simm & \simm & \simm & \cmark \\
% & Conditional Compilation & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark \\
% & External Functions & \xmark & \cmark & \simm & \cmark & \simm & \cmark \\
% & Inline Assembly & \xmark & \simm & \xmark & \xmark & \xmark & \cmark \\
% & Macro Function Calls & \xmark & \cmark & \xmark & \simm & \cmark & \cmark \\
% & Goto Statements & \xmark & \cmark & \simm & \cmark & \cmark & \cmark \\
% & Setjmp/Longjmp & \xmark & \simm & \xmark & \xmark & \simm & \cmark \\
% & Recursive Functions & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% \midrule
% \multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
% & Decorators & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark \\
% & First-Class Functions & \xmark & \cmark & \xmark & \simm & \xmark & \cmark \\
% & Lambda Functions & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark \\
% & Generators/Coroutines & \cmark & \simm & \xmark & \simm & \xmark & \cmark \\
% & Reflection & \xmark & \simm & \xmark & \simm & \xmark & \cmark \\
% & Dynamic Imports & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark \\
% \bottomrule
% \end{tabular}%
% }

% \resizebox{\columnwidth}{!}{%
% \renewcommand{\arraystretch}{0.8}
% \scriptsize
% \begin{tabular}{@{}llcccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Lang}} & \multirow{2}{*}{\textbf{Feature}} & \multicolumn{2}{c}{\textbf{Impact}} & \multicolumn{5}{c}{\textbf{Static Analyzer Support}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-9}
% & & \textbf{Ent.} & \textbf{Flow} & \textbf{Joern} & \textbf{CodeQL} & \textbf{Infer} & \textbf{Sonar} & \textbf{Clang} & \textbf{PolyFlow} \\
% \midrule
% \multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
% & Function Pointers & -- & \cmark & \xmark & \simm & \xmark & \simm & \simm & \cmark \\
% & Conditional Compilation & \cmark & \cmark & \simm & \cmark & \xmark & \cmark & \cmark & \cmark \\
% & External Functions & \cmark & \cmark & \simm & \cmark & \simm & \cmark & \cmark & \cmark \\
% & Inline Assembly & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
% & Macro Function Calls & \cmark & \cmark & \xmark & \simm & \xmark & \simm & \cmark & \cmark \\
% & Goto Statements & -- & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% & Setjmp/Longjmp & -- & \cmark & \xmark & \xmark & \xmark & \xmark & \simm & \cmark \\
% & Recursive Functions & -- & -- & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% \midrule
% \multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
% & Decorators & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\
% & First-Class Functions & -- & \cmark & \xmark & \cmark & \text{N/A} & \simm & \text{N/A} & \cmark \\
% & Lambda Functions & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\
% & Generators/Coroutines & \cmark & \cmark & \simm & \simm & \text{N/A} & \simm & \text{N/A} & \cmark \\
% & Reflection & -- & \cmark & \xmark & \simm & \text{N/A} & \simm & \text{N/A} & \cmark \\
% & Dynamic Imports & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\
% \bottomrule
% \end{tabular}%
% }


%%%%%%%%%% Claude 4.0 final answer after many rounds of self-checking
% \resizebox{\columnwidth}{!}{%
% \renewcommand{\arraystretch}{0.8}
% \scriptsize
% \begin{tabular}{@{}llcccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Lang}} & \multirow{2}{*}{\textbf{Feature}} & \multicolumn{2}{c}{\textbf{Impact}} & \multicolumn{5}{c}{\textbf{Static Analyzer Support}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-9}
% & & \textbf{Ent.} & \textbf{Flow} & \textbf{Joern} & \textbf{CodeQL} & \textbf{Infer} & \textbf{SonarQube} & \textbf{Clang} & \textbf{PolyFlow (aims)} \\
% \midrule
% \multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
% & Function Pointers & -- & \cmark & \xmark &  & \xmark & \simm & \simm & \cmark \\
% & Conditional Compilation & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark \\
% & External Functions & \cmark & \cmark & \simm & \cmark & \simm & \cmark & \cmark & \cmark \\
% & Inline Assembly & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
% & Macro Function Calls & \cmark & \cmark & \xmark & \simm & \xmark & \simm & \cmark & \cmark \\
% & Goto Statements & -- & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% & Setjmp/Longjmp & -- & \cmark & \xmark & \xmark & \xmark & \xmark & \simm & \cmark \\
% & Recursive Functions & -- & -- & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% \midrule
% \multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
% & Decorators & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\
% & First-Class Functions & -- & \cmark & \xmark & \cmark & \text{N/A} & \simm & \text{N/A} & \cmark \\
% & Lambda Functions & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\
% & Generators/Coroutines & \cmark & \cmark & \simm & \simm & \text{N/A} & \simm & \text{N/A} & \cmark \\
% & Reflection & -- & \cmark & \xmark & \simm & \text{N/A} & \simm & \text{N/A} & \cmark \\
% & Dynamic Imports & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\
% \bottomrule
% \end{tabular}%
% }

%%%%%%%%%% Claude 4.0 final answer checked/corrected by DeepSeek
% \resizebox{\columnwidth}{!}{%
% \renewcommand{\arraystretch}{0.8}
% \scriptsize
% \begin{tabular}{@{}llcccccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Lang}} & \multirow{2}{*}{\textbf{Feature}} & \multicolumn{2}{c}{\textbf{Impact}} & \multicolumn{5}{c}{\textbf{Static Analyzer Support}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-9}
% & & \textbf{Ent.} & \textbf{Flow} & \textbf{Joern} & \textbf{CodeQL} & \textbf{Infer} & \textbf{Sonar} & \textbf{Clang} & \textbf{PolyFlow} \\
% % \midrule
% % \multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
% % & Function Pointers & -- & \cmark & \simm & \cmark & \simm & \simm & \cmark & \cmark \\  % Joern/Infer: partial support
% % & Conditional Compilation & \cmark & \cmark & \xmark & \simm & \xmark & \simm & \simm & \cmark \\  % CodeQL/Clang/Sonar: partial
% % & External Functions & \cmark & \cmark & \simm & \simm & \simm & \simm & \simm & \cmark \\  % All: partial
% % & Inline Assembly & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\  % Correct
% % & Macro Function Calls & \cmark & \cmark & \xmark & \simm & \xmark & \simm & \simm & \cmark \\  % CodeQL/Sonar/Clang: partial
% % & Goto Statements & -- & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\  % Flow impact incorrect (no missing edges)
% % & Setjmp/Longjmp & -- & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\  % Ent. impact incorrect (no missing nodes)
% % & Recursive Functions & -- & -- & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\  % Correct
% % \midrule
% % \multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
% % & Decorators & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\  % Correct
% % & First-Class Functions & -- & \cmark & \xmark & \cmark & \text{N/A} & \simm & \text{N/A} & \cmark \\  % Correct
% % & Lambda Functions & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\  % Correct
% % & Generators/Coroutines & \cmark & \cmark & \xmark & \simm & \text{N/A} & \xmark & \text{N/A} & \cmark \\  % Sonar: no support
% % & Reflection & \cmark & \cmark & \xmark & \simm & \text{N/A} & \xmark & \text{N/A} & \cmark \\  % Ent. impact added; Sonar: no support
% % & Dynamic Imports & \cmark & \cmark & \xmark & \simm & \text{N/A} & \simm & \text{N/A} & \cmark \\  % CodeQL/Sonar: partial
% \midrule
% \multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
% & Function Pointers & -- & \cmark & \xmark & \cmark & \simm & \simm & \cmark & \cmark \\  % Joern: no support
% & Conditional Compilation & \cmark & \cmark & \xmark & \simm & \xmark & \simm & \simm & \cmark \\  
% & External Functions & \cmark & \cmark & \xmark & \simm & \simm & \simm & \simm & \cmark \\  % Joern: no support
% & Inline Assembly & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\  
% & Macro Function Calls & \cmark & \cmark & \xmark & \simm & \xmark & \simm & \simm & \cmark \\  
% & Goto Statements & -- & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\  
% & Setjmp/Longjmp & -- & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\  
% & Recursive Functions & -- & -- & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\  
% \midrule
% \multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
% & Decorators & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\  
% & First-Class Functions & -- & \cmark & \xmark & \cmark & \text{N/A} & \xmark & \text{N/A} & \cmark \\  % Sonar: no support
% & Lambda Functions & \cmark & \cmark & \xmark & \cmark & \text{N/A} & \cmark & \text{N/A} & \cmark \\  
% & Generators/Coroutines & \cmark & \cmark & \xmark & \simm & \text{N/A} & \xmark & \text{N/A} & \cmark \\  
% & Reflection & \cmark & \cmark & \xmark & \xmark & \text{N/A} & \xmark & \text{N/A} & \cmark \\  % CodeQL: no support
% & Dynamic Imports & \cmark & \cmark & \xmark & \simm & \text{N/A} & \xmark & \text{N/A} & \cmark \\  % Sonar: no support
% \bottomrule
% \end{tabular}%
% }

%%%%%%%%%% Claude 4.0 + DeepSeek's final answer formatted
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{0.8}
\scriptsize
\begin{tabular}{@{}llcccccccc@{}}
%\begin{tabular}{@{}l@{}l@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\toprule
%\multirow{2}{*}{\textbf{Lang}} & \multirow{2}{*}{\textbf{Feature}} & \multicolumn{2}{c}{\textbf{Impact}} & \multicolumn{5}{c}{\textbf{Static Analyzer Support}} \\
%\cmidrule(lr){3-4} \cmidrule(lr){5-9}
%& & \textbf{Ent.} & \textbf{Flow} & \textbf{Joern} & \textbf{CodeQL} & \textbf{Infer} & \textbf{SonarQube} & \textbf{Clang} & \textbf{PolyFlow (aims)} \\
\multirow{2}{*}{\textbf{Lang.}} & \multirow{2}{*}{\textbf{Feature}} & \multicolumn{2}{c}{\textbf{Impact}} & \multicolumn{5}{c}{\textbf{Static Analyzer Support}} & \multirow{2}{*}{\textbf{{\tech}}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-9}
& & \textbf{Ent.} & \textbf{Flow} & \textbf{Joern} & \textbf{CodeQL} & \textbf{Infer} & \textbf{SonarQube} & \textbf{Clang} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textbf{Python}}} 
& Decorators & \cmark & \cmark & \no & \rhalf & \text{N/A} & \rhalf & \text{N/A} & \yes \\  
& First-Class Functions & -- & \cmark & \no & \rhalf & \text{N/A} & \rhalf & \text{N/A} & \yes \\  
& Lambda Functions & \cmark & \cmark & \no & \rhalf & \text{N/A} & \rhalf & \text{N/A} & \yes \\  
%& Generators/Coroutines & \cmark & \cmark & \no & \rhalf & \text{N/A} & \no & \text{N/A} & \yes \\  
& Dynamic Typing & -- & \cmark & \no & \rhalf & \text{N/A} & \rhalf & \text{N/A} & \yes \\
& Reflection & \cmark & \cmark & \no & \rhalf & \text{N/A} & \no & \text{N/A} & \yes \\  
& Dynamic Imports & \cmark & \cmark & \no & \rhalf & \text{N/A} & \no & \text{N/A} & \yes \\  
\midrule
\multirow{8}{*}{\rotatebox{90}{\textbf{C}}} 
& Function Pointers & -- & \cmark & \no & \yes & \rhalf & \rhalf & \yes & \yes \\  
& Conditional Compilation & \cmark & \cmark & \no & \rhalf & \no & \rhalf & \rhalf & \yes \\  
& External Functions & \cmark & \cmark & \no & \rhalf & \rhalf & \rhalf & \rhalf & \yes \\  
& Inline Assembly & \cmark & \cmark & \no & \no & \no & \no & \no & \yes \\  
& Macro Function Calls & \cmark & \cmark & \no & \rhalf & \no & \rhalf & \rhalf & \yes \\  
& Goto Statements & -- & \cmark & \rhalf & \yes & \yes & \yes & \yes & \yes \\  
& Setjmp/Longjmp & -- & \cmark & \no & \no & \no & \no & \no & \yes \\  
& Recursive Functions & -- & -- & \yes & \yes & \yes & \yes & \yes & \yes \\  
\bottomrule
\end{tabular}%
}
\label{tab:motivation-study}
\vspace{-6pt}
\end{table}
%\setlength{\tabcolsep}{6pt}

\begin{figure*}[tp]
\begin{center}
%\includegraphics[width=0.8\textwidth]{Figures/overview-cai-improved.pdf}
\includegraphics[width=0.8\textwidth]{Figures/overview-cai-updated.pdf}
\end{center}
\caption[Methodology Overview]{Overview of {\tech}, including its inputs, two main phases backed by an expert panel, and outputs.}
\vspace{0pt}
\label{fig:overview}
\end{figure*}

As summarized in Table~\ref{tab:motivation-study}, our study revealed 8 C and 6 Python features that are complex hence potentially defeating static analysis. 
For each feature, we note its impact on the analysis in terms of whether (if not handling the feature) code entities (\textbf{Ent.}) and flow facts (\textbf{Flow}) would be \textit{missing} in the analysis's underlying control flow graph as nodes and edges, respectively. 
For example, Python reflection and C inline assembly may induce both missing nodes and missing edges, for all the 5 analyzers considered because none of them fully support these features. As another example, first-class functions in Python and function pointers in C lead to missing edges, for most of these tools. 
From a combinatorial perspective, even if a tool is capable of cross-language analysis, it will miss the holistic cross-language flow even more often 
(than these 5 single-language analyzers)---i.e., when any unsupported feature is used in any language. 
Since control flow (reachability) is a prerequisite for data flow between two program entities, missing these (control flow) nodes/edges implies 
missing the data flow, hence information flow, between the two entities. 


%As shown in the table, Joern successfully processes only two of the 14 challenging features, demonstrating particular weaknesses with dynamic language constructs including conditional compilation, external function calls, lambda expressions, and dynamic imports. These shortcomings substantially compromise the accuracy and reliability of cross-language static analysis. In contrast, our proposed {{\tech}} can achieve comprehensive support for all identified features through innovative LLM-driven enhancements, which are detailed in §\ref{phase 1.2} (CICFG Augmentation) and §\ref{sec:feature-handling} (Feature Handling).

%Facing the limitation of traditional methods, in summary, we propose {\tech} — a novel hybrid architecture framework  that combines rigorous static analysis foundations with adaptive LLM-powered reasoning. By augmenting traditional CICFG construction with learned semantic understanding and specialized handling of language-specific complexities, {\tech} bridges the gap between formal analysis and dynamic language behaviors. This synergistic approach not only addresses all identified limitations from Table~\ref{tab:motivation-study} but also maintains the scalability and precision required for production-scale analysis.


% From Table \ref{tab:motivation-study}, Joern can only correctly handle two challenging features, and struggles with other features across C and Python, particularly with dynamic and complex language constructs such as conditional compilation, external functions, lambda functions, and dynamic imports. Joern's limitations significantly impact static analysis accuracy. In contrast, {\tech} can handle all these features through targeted LLM-driven improvements, which are elaborated in $\S$\ref{phase 1.2} (CICFG Augmentation) and $\S$\ref{sec:feature-handling} (Feature Handling).

% Given these limitations, our objective is to overcome the deficiencies highlighted in Table \ref{tab:motivation-study} by achieving comprehensive support ("yes") across all identified multilingual scenarios. To realize this, we propose {\tech}—a novel framework integrating both advanced static analysis enhancements and targeted large language model (LLM) prompting. {\tech} leverages static constructs (e.g., CICFG) to provide structured insights into multilingual interactions while employing LLM capabilities to effectively bridge semantic gaps, resolve dynamic language features, and iteratively refine implicit flows, ultimately ensuring precision, scalability, and practicality.

Thus, to enable systematic cross-language static information flow analysis, we aim to support all the 14 features in {\tech}, which 
combines traditional static analysis and LLMs. 
For the former part, we set three requirements as justified by maximizing applicability: 
(1) it provides direct access to the analysis's underlying program representations (e.g., control/data flow graphs), 
(2) it works with uncompilable code, 
and (3) it is free to use for code at any scale. 
(1) is also needed for most flexible customization towards greater capabilities. 
%
%Among the 5 analyzers, 
Only Joern meets these requirements. Thus, we will use it in {\tech}, which 
means we will need to handle 12 out of the 14 features. 

%"For analysis development (vs. out-of-box scanning), Joern's CPG provides the most flexible foundation among open-source tools." - Joern: A Platform for Analyzing Binary and Source Code (ACSAC 2020)

==> Sections/02_background.tex <==
%!TEX root = paper.tex
\section{Background and Motivation}\label{sec:bkgmotive}
We provide necessary background on multilingual code analysis, and then motivate our work via a study that 
reveals challenges to static information flow analysis of multilingual code. 

\subsection{Multilingual Code Representation}

%Multi-language software refers to systems that incorporate multiple computer languages \textit{that interact}. The interactions %between languages 
%typically rely on \textit{Foreign Function Interfaces (FFIs)}, which enable cross-language communication through specific APIs. For example, Python and C each provide distinct FFI mechanisms---Python through the \textit{ctypes} library and C-extensions.

Multi-language software refers to systems that incorporate multiple computer languages \textit{that interact}, where the program is referred to as \textit{multilingual code/program}.
The interactions %between languages 
typically rely on \textit{Foreign Function Interfaces (FFIs)}, a mechanism that enables code written in one programming (host) language to call functions written in another (guest) language. 
For example, Python provides FFIs for cross-language interfacing with C via modules like \textit{ctypes} and C-extensions. 
In particular, such interfacing involves two main types of \textit{cross-language functions}: native functions and foreign functions. Native functions are implemented by developers in a guest language to be invoked in the host language code, %different from the caller’s language, 
while foreign functions are provided by the host language to facilitate interoperability with the guest language code.

%A Foreign Function Interface (FFI) enables a program written in one programming language (the host) to call functions or use services written in another language (the guest). This interoperability is crucial for leveraging existing libraries, optimizing performance, or integrating components across different programming environments.

%Cross-language interfacing involves two primary function types: native functions and foreign functions. Native functions are implemented by developers in a language different from the caller’s language, while foreign functions are language-provided utilities that facilitate interactions with external code.


%To enable holistic static analysis of multi-language codebases, we introduce the \textbf{Cross-language Interprocedural Control Flow Graph (CICFG)}, a unified representation that captures control flow across language boundaries. Our methodology begins by constructing intraprocedural control flow graphs (CFGs) for individual methods generated by Joern, an industry static analyzer. These CFGs are then extended into an Interprocedural CFG (ICFG) by linking callers to callees and connecting return sites. Finally, we bridge language gaps by resolving foreign function calls, producing the complete CICFG. In this graph, nodes correspond to statements, and edges represent control flow relationships between them.

A program analysis is often based on a program representation, such as the control flow graph (CFG). By default, CFG is intraprocedural, representing control flow within a function. For interprocedural analysis, per-function CFGs are linked together through calling relationships between the functions, forming an interprocedural CFG (or ICFG). 
To enable holistic static analysis of multi-language software, a multilingual code representation is also needed, for which further link per-language ICFGs through control flow induced by cross-language functions. We refer to this representation the \textbf{cross-language interprocedural control flow graph (CICFG)}. 
Thus, a CICFG node represents a statement in a multilingual program, while a CICFG edge represents control flow between two nodes within and across the languages.

%we introduce the \textbf{Cross-language Interprocedural Control Flow Graph (CICFG)}, a unified representation that captures control flow across language boundaries. Our methodology begins by constructing intraprocedural control flow graphs (CFGs) for individual methods generated by Joern, an industry static analyzer. These CFGs are then extended into an Interprocedural CFG (ICFG) by linking callers to callees and connecting return sites. Finally, we bridge language gaps by resolving foreign function calls, producing the complete CICFG. In this graph, nodes correspond to statements, and edges represent control flow relationships between them.



% The CICFG provides a foundation for holistic static analysis of multi-language software, addressing a key limitation in existing approaches that struggle with cross-language dependencies.


% In multilingual codebases, the interfacing points between languages typically rely on Foreign Function Interfaces (FFIs), which enable language-level communication through defined APIs. Common FFIs include Python's \textit{ctypes} and C-extensions, Java's Native Interface (JNI), and JavaScript's bindings with WebAssembly. These interfaces facilitate data exchanges, type conversions, and memory management across languages, but the complexity of handling different semantic models at these interfaces creates potential vulnerabilities.

% To frame our discussion, we introduce several terminologies frequently employed in multilingual software analysis:
% \begin{itemize}[leftmargin=*,topsep=2pt]
%     \item \textbf{Cross-language Interprocedural Control Flow Graph (CICFG):} A unified graph representation that explicitly models interprocedural control flow across programming language boundaries. 
%     \item \textbf{Cross-Language Interface (CLI):} The explicit boundary where languages communicate and exchange data.
%     \item \textbf{Implicit Flow:} Data flows that are not explicitly defined but arise through control-flow or language semantics mismatches.
% \end{itemize}

% These terminologies provide a foundation for understanding the complexities inherent in multilingual software analysis.

\subsection{Motivating Study}

In this paper, we focus on investigating the language interaction only between Python and C. During our construction of CICFG for Python-C programs, we identified some language-specific features that pose significant obstacles to existing static analysis approaches. A prominent one is C's function pointer mechanism, which we examine in detail below.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{Figures/func_pointer.pdf}
      \caption{Function pointer real-world usage. The call path of the function pointer \code{word2bool} is marked with green lines.}
    \label{fig:funcp}
\end{figure}

% start with CFG by Joern, enabled by, we define interprocedual control flow graph. based on ICFG for each language, we then connect the   for foreign language and native and get holistic graph. Each node is a statement, each edge represents a control flow relationship.


\figref{fig:funcp} is a real-world code showing the typical usage of function pointers, which introduces indirect control-flow edges. The function \texttt{word2bool} (declared in line 1) is a utility function converting data from type \texttt{word} to \texttt{bool}, crucial for conditional decisions. It passes to the function \texttt{findletters} (line 2), which is declared in line 3, accepting function pointer \texttt{word2bool} as the third parameter \texttt{tobool} and invoking function \texttt{getsig} (line 7) declared in line 10, inside which the function \texttt{word2bool} is eventually invoked in line 19. Traditional static analyses struggle to resolve such indirect calls due to the dynamic nature of function pointers, causing incomplete CICFGs that miss these critical edges.

To systematically identify language features that challenge static analysis in cross-language environments beyond function pointers, we conducted a comprehensive investigation through three approaches: (1) analysis of prominent open-source Python-C projects, (2) review of developer discussions and technical blogs, and (3) empirical evaluation of static analysis tools. We analyzed prominent open-source Python-C projects mined from GitHub, building upon the dataset curated in the prior study on cross-language bugs~\cite{yang2025dissecting}. This analysis involved forward and backward traversals of cross-language information flows, using CICFG-based inspection to pinpoint critical locations and root causes of cross-language bugs. The study highlighted specific Python and C constructs—such as dynamic typing and language-specific APIs—that frequently hinder static analysis. This process revealed 14 problematic features across Python and C that significantly impede static analysis. We evaluated these features' impact on CFG generation by assessing Joern's ability to correctly process each case, with detailed results presented in Table \ref{tab:motivation-study}.

\input{Tables/lan_feature_new}

As shown in the table, Joern successfully processes only two of the 14 challenging features, demonstrating particular weaknesses with dynamic language constructs including conditional compilation, external function calls, lambda expressions, and dynamic imports. These shortcomings substantially compromise the accuracy and reliability of cross-language static analysis. In contrast, our proposed {{\tech}} can achieve comprehensive support for all identified features through innovative LLM-driven enhancements, which are detailed in §\ref{phase 1.2} (CICFG Augmentation) and §\ref{sec:feature-handling} (Feature Handling).

Facing the limitation of traditional methods, in summary, we propose {\tech} — a novel hybrid architecture framework  that combines rigorous static analysis foundations with adaptive LLM-powered reasoning. By augmenting traditional CICFG construction with learned semantic understanding and specialized handling of language-specific complexities, {\tech} bridges the gap between formal analysis and dynamic language behaviors. This synergistic approach not only addresses all identified limitations from Table~\ref{tab:motivation-study} but also maintains the scalability and precision required for production-scale analysis.

% From Table \ref{tab:motivation-study}, Joern can only correctly handle two challenging features, and struggles with other features across C and Python, particularly with dynamic and complex language constructs such as conditional compilation, external functions, lambda functions, and dynamic imports. Joern's limitations significantly impact static analysis accuracy. In contrast, {\tech} can handle all these features through targeted LLM-driven improvements, which are elaborated in $\S$\ref{phase 1.2} (CICFG Augmentation) and $\S$\ref{sec:feature-handling} (Feature Handling).

% Given these limitations, our objective is to overcome the deficiencies highlighted in Table \ref{tab:motivation-study} by achieving comprehensive support ("yes") across all identified multilingual scenarios. To realize this, we propose {\tech}—a novel framework integrating both advanced static analysis enhancements and targeted large language model (LLM) prompting. {\tech} leverages static constructs (e.g., CICFG) to provide structured insights into multilingual interactions while employing LLM capabilities to effectively bridge semantic gaps, resolve dynamic language features, and iteratively refine implicit flows, ultimately ensuring precision, scalability, and practicality.

==> Sections/03_algorithm.tex <==

\section{Technique}
This section describes our technical approach, \tech, for analyzing cross-language (Python–C) programs and detecting potential vulnerabilities. We begin with an overview of the framework (§~\ref{overview}) and then detail its two key phases: the augmented control-flow analysis (§~\ref{phase 1}) and the feature-oriented data-flow reasoning (§~\ref{phase 2}). These phases work in tandem to systematically uncover taint flows that might otherwise evade traditional static analyses, particularly in complex multi-language settings


\subsection{Maintaining the Integrity of the Specifications}

\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{CICFG Node and Edge Update}}
\label{algo:updateCICFGNodeEdge}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{UpdateCICFGNode}{UpdateCICFGNode}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered

\Fn{\UpdateCICFGNode{file name, line\_number, statement, annotation=None}}{
    nodeID $\gets$ \text{Generate unique node ID based on \textit{file name} and \textit{line\_number}}\;\label{line:generateNodeID}
    % properties $\gets$ \text{statement, annotation}\;\label{line:extractProperties}
    \If{CICFG.hasNode(nodeID)}{\label{line:checkNodeExists}
        node $\gets$ CICFG.getNode(nodeID)\;\label{line:getExistingNode}
    }
    \Else{
        node $\gets$ new Node(nodeID)\;\label{line:createNewNode}
        node.file $\gets$ \textit{file name}\;\label{line:setNodeFile}
        node.line\_number $\gets$ \textit{line\_number}\;\label{line:setNodeLineNumber}
        node.statement $\gets$ \textit{statement}\;
        CICFG.addNode(node)\;\label{line:addNodeToCICFG}
    }
    \If{annotation is not None}{
        node.addProperty(annotation.key,annotation.value)\;\label{line:addPropertyToNode}
    }
    % \ForEach{(key, value) in properties}{\label{line:iterateProperties}
    %     node.addProperty(key, value)\;\label{line:addPropertyToNode}
    % }
}

\Fn{\UpdateCICFGEdge{file name, source\_line no., target\_file name = file name, target\_line no., annotation=None}}{
    sourceNodeID $\gets$ \text{Generate unique node ID based on \textit{file name} and \textit{source\_line no.}}\;\label{line:generateSourceNodeID}
    targetNodeID $\gets$ \text{Generate unique node ID based on \textit{target\_file name} and \textit{target\_line no.}}\;\label{line:generateTargetNodeID}
    \If{CICFG.hasNode(sourceNodeID) == False}{\label{line:checkSourceNodeExists}
        statement $\gets$ Retrieve the statement in the \textit{file name} by \textit{source\_line no.} from CICFG\;\label{line:retrieveSourceStatement}
        UpdateCICFGNode(file name, source\_line no., statement, annotation)\;\label{line:addSourceNodeToCICFG}
    }
    \If{CICFG.hasNode(targetNodeID) == False}{\label{line:checkTargetNodeExists}
        statement $\gets$ Retrieve the statement in the \textit{file name} by \textit{target\_line no.} from CICFG\;\label{line:retrieveTargetStatement}
        UpdateCICFGNode(target\_file name, target\_line, statement, annotation)\;\label{line:addTargetNodeToCICFG}
    }
    edgeID $\gets$ \text{Generate unique edge ID based on source and target nodes}\;\label{line:generateEdgeID}
    \If{CICFG.hasEdge(edgeID) == False}{\label{line:checkEdgeExists}
        edge $\gets$ new Edge(sourceNodeID, targetNodeID)\;\label{line:createEdge}
        edge.source\_file $\gets$ \textit{file name}\;\label{line:setEdgeFile}
        edge.target\_file $\gets$ \textit{target\_file name}\;\label
        edge.source\_line $\gets$ \textit{source\_line no.}\;\label{line:setEdgeSourceLine}
        edge.target\_line $\gets$ \textit{target\_line no.}\;\label{line:setEdgeTargetLine}
        CICFG.addEdge(edge)\;\label{line:addEdgeToCICFG}
    }
}

\end{algorithm*}

\FloatBarrier
\noindent\textbf{Explanation:}

The algorithm provides detailed implementations of two functions, \UpdateCICFGNode and \UpdateCICFGEdge, which are responsible for updating the Cross-Language Interprocedural Control Flow Graph (CICFG) with nodes and edges, respectively. These functions ensure that the CICFG accurately represents the program's control flow and includes necessary annotations, such as those indicating conditional compilation.

\textbf{Function \UpdateCICFGNode (Lines~\ref{line:generateNodeID}--\ref{line:addPropertyToNode}):}

- \textbf{Line~\ref{line:generateNodeID}}: Generate a unique identifier for the node based on the file name and line number. This ensures that each node can be uniquely identified within the CICFG.

% - \textbf{Line~\ref{line:extractProperties}}: Extract properties and annotations from the given statement and any additional annotations provided. These may include indicators like `conditional\_compilation`, `macro\_expansion`, etc.

- \textbf{Lines~\ref{line:checkNodeExists}--\ref{line:getExistingNode}}: Check if a node with this identifier already exists in the CICFG. If it does, retrieve the existing node.

- \textbf{Lines~\ref{line:createNewNode}--\ref{line:addNodeToCICFG}}: If the node does not exist, create a new node with the generated ID, set its file and line number, and add it to the CICFG.

- \textbf{Lines~\ref{line:addPropertyToNode}}: 
% Iterate over each extracted property and add it to the node's properties.
This step annotates the node with relevant information, such as whether it is part of a conditional compilation block.

\textbf{Function \UpdateCICFGEdge (Lines~\ref{line:generateSourceNodeID}--\ref{line:addEdgeToCICFG}):}

- \textbf{Lines~\ref{line:generateSourceNodeID}--\ref{line:generateTargetNodeID}}: Generate unique identifiers for the source and target nodes based on their file names and line numbers.

- \textbf{Lines~\ref{line:checkSourceNodeExists}--\ref{line:addSourceNodeToCICFG}}: Check if the source node exists in the CICFG. If not, retrieve the statement at the source line (Line~\ref{line:retrieveSourceStatement}) and call \UpdateCICFGNode to create and add the source node (Line~\ref{line:addSourceNodeToCICFG}).

- \textbf{Lines~\ref{line:checkTargetNodeExists}--\ref{line:addTargetNodeToCICFG}}: Similarly, check for the target node. If it doesn't exist, retrieve the statement at the target line (Line~\ref{line:retrieveTargetStatement}) and create the target node.

- \textbf{Line~\ref{line:generateEdgeID}}: Generate a unique identifier for the edge based on the source and target node IDs.

- \textbf{Lines~\ref{line:checkEdgeExists}--\ref{line:addEdgeToCICFG}}: Check if the edge already exists in the CICFG. If not, create a new edge connecting the source and target nodes. Set the source and target file names and line numbers (Lines~\ref{line:setEdgeFile}--\ref{line:setEdgeTargetLine}).

% - \textbf{Lines~\ref{line:iterateEdgeAnnotations}--\ref{line:addPropertyToEdge}}: Iterate over any annotations provided and add them as properties to the edge. This allows for additional context, such as specifying that an edge represents a function call or is part of a macro expansion.

- \textbf{Line~\ref{line:addEdgeToCICFG}}: Add the newly created and annotated edge to the CICFG.




\subsection{Equations}

% ===================================================================
% C feature: function pointer
\begin{algorithm*}[tp]
%\scriptsize
\caption{\footnotesize{Function Pointer Analysis - C feature}}
\label{algo:enhancedFunctionPointerAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeFunctionPointers}{AnalyzeFunctionPointers}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{FindCaller}{FindCaller}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKwFunction{RetrieveFunctionBody}{RetrieveFunctionBody}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{set of functions $F$ from a program}\label{pointer_input}
\KwOut{Updated CICFG}\label{pointer_output}

\Fn{\AnalyzeFunctionPointers{F}}{\label{pointer_function_analysis}
    start\_func $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{function in $F$}{\label{pointer_each_function}
        \textit{res} $\gets$ \SendToLLM{"Does the given function use any function pointer? " + code of function}\;\label{pointer_check_fp_use}
        \If{res == "NO"}{\label{pointer_check_fp_response}
            continue\label{pointer_continue}
        }
        \Else{\label{pointer_else}
            start\_func.append(function)\;
            \textit{resp} $\gets$ \SendToLLM{"Give me $<$each function pointer variable name, the function it points to$>$." + code of function}\;\label{pointer_get_fp_details}
            \ForEach{(\textit{pfunc}, \textit{func name}) in resp}{\label{pointer_for_each_fp}
                % funcs $\gets$ \{func\}\; \tcp{initialize list with current function}
                % original func $\gets$ retrieve the code of resp according to current CICFG\;
                \textit{callsite} $\gets$ \FindCaller{pfunc, [\textit{func name}]}\;\label{pointer_find_caller}
                \If{callsite != NULL}{\label{pointer_if_caller_found}
                    \textit{callsite}'s file name, \textit{callsite}'s line no., \textit{func}'s file name, \textit{func}'s line no. $\gets$ retrieve the file name and line no. of \textit{callsite} and \textit{func} from CICFG\;
                    \UpdateCICFGEdge{\textit{callsite}'s file name, \textit{callsite}'s line no., \textit{func}'s file name, \textit{func}'s entry line no.}\;\label{pointer_update_cicfg}
                    is\_updated $\gets$ true\;
                }
            }
        }
    }
    \Return{start\_func, is\_updated}\;
}

\Fn{\FindCaller{\textit{pfunc}, \textit{funcs}}}{\label{pointer_find_caller_fn}
    \textit{funcs code} $\gets$ retrieve the code of each function in \textit{funcs} according to current CICFG\;\label{pointer_retrieve_code}
    \textit{res}, \textit{callsite} $\gets$ \SendToLLM{"Is " + \textit{funcs}[0] + " called via " + \textit{pfunc} + " in the given code? If yes, output 'YES' followed by the \textit{callsite}." + \textit{funcs code}}\;\label{pointer_llm_query1}
    \If{\textit{res} == "YES"}{\label{pointer_response_yes}
        \Return{\textit{caller}}\label{pointer_return_caller}
    }
    \Else{\label{pointer_else_query2}
        \textit{res} $\gets$ \SendToLLM{"Is there any function you don’t know about that is called with " + \textit{pfunc} + "as an argument? If yes, tell me which one"}\;\label{pointer_query_unknown}
        \If{\textit{res} == "no"}{\label{pointer_response_no}
            \Return{NULL}\label{pointer_return_null}
        }
        \Else{\label{pointer_else_find_new}
            %newFunc $\gets$ retrieve the code of \textit{res} according to current CICFG\;
            %newpfunc $\gets$ retrieve the function pointer name in the newFunc\;
            \textit{newFunc} $\gets$ retrieve the function name from \textit{res}\;\label{pointer_new_func}
            \textit{newpfunc} $\gets$ retrieve the name of the parameter of \textit{newFunc} that takes \textit{pfunc} from CICFG\;\label{pointer_new_pfunc}
            \Return{\FindCaller{\textit{newpfunc}, \textit{funcs}.append(\textit{newFunc})}}\label{pointer_recursive_call} \tcp{append new function to the list and reevaluate}
        }
    }
}

\end{algorithm*}



\FloatBarrier \noindent\textbf{Explanation:} The algorithm starts by processing each function in the given set $F$ of functions (line~\ref{pointer_each_function}). For each function, it checks if any function pointers are used by sending a prompt to the LLM (line~\ref{pointer_check_fp_use}). The LLM returns 'YES' if function pointers are used, or 'NO' otherwise.

If the response is 'NO' (line~\ref{pointer_check_fp_response}), the algorithm continues to the next function (line~\ref{pointer_continue}). Otherwise, it proceeds to get details about each function pointer used in the function, including the names of the function pointers and the functions they point to (line~\ref{pointer_get_fp_details}).

For each function pointer (line~\ref{pointer_for_each_fp}), it tries to identify any callers of the functions that are pointed to by the function pointers. This is done by the FindCaller function (line~\ref{pointer_find_caller}), which checks if the function is called through the specific function pointer within the code of related functions.

If a caller is found (line~\ref{pointer_if_caller_found}), the CICFG is updated to reflect this relationship by adding an edge from the caller to the called function's name (line~\ref{pointer_update_cicfg}). This update helps in analyzing the control flow in programs that use function pointers dynamically, enhancing the understanding of their execution and interaction.

The FindCaller function (line~\ref{pointer_find_caller_fn}) works by querying the LLM with the code of the involved functions to determine if a function is called via the function pointer. If the LLM confirms a call (line~\ref{pointer_response_yes}), it returns the caller (line~\ref{pointer_return_caller}). If not, it checks for any unknown functions that might be called using the function pointer (line~\ref{pointer_query_unknown}). If such a function is identified, the process is recursively continued with the new function and function pointer (line~\ref{pointer_recursive_call}), ensuring thorough analysis of dynamic function pointer usage across the program.


\begin{lstlisting}[language=C, firstnumber=5]
bool word2bool(void *val) { return *(word *)val != 0; }
\end{lstlisting}

\begin{lstlisting}[language=C, firstnumber=48]
char *b = findletters(buf, &grid, word2bool);
\end{lstlisting}

\begin{lstlisting}[language=C, firstnumber=132]
char *findletters(char *buf, grid *grid, bool (*tobool)(void *val)) {
    char *p = buf;
    for (int j = 0; j < grid->height; j++) {
        for (int i = 0; i < grid->width; i++) {
            int v = getsig(grid, tobool, i, j);
        }
    }
}
\end{lstlisting}

\begin{lstlisting}[language=C, firstnumber=119, caption=function pointer real world example., label=fig:pointer]
inline int getsig(grid *grid, bool (*tobool)(void *val), int x, int y) {
  int ret = 0;
  if (x + 4 > grid->width || y + 6 > grid->height)
    return 0;
  for (int j = y; j < y + 6; j++) {
      for (int i = x; i < x + 4; i++) {
          ret *= 2;
          ret += tobool(grid->get(grid, i, j));
      }
  }
  return ret;
}
\end{lstlisting}

As shown in figure~\ref{fig:pointer}, \textit{word2bool} is a utility function that appears to be used for converting data from a word type to a boolean, likely for conditional checks or decisions based on the contents of memory referenced by the pointer.
The function \textit{word2bool} is passed as an argument to \textit{findletters} in the line 48.
\textit{findletters} function iterates over a grid and applies \textit{word2bool} to elements within the grid, filtered or processed through \textit{getsig}. 
\textit{tobool} is an alias or a parameter name for \textit{word2bool}, used to convert the data retrieved from the grid into a boolean value, affecting the computation of a signature or identifier (\textit{ret}) in line 126.


\noindent\textbf{Usage with example}
As shown in figure~\ref{fig:pointer}, the algorithm processes the C code which utilizes a function pointer `word2bool` in its grid processing function `findletters`. The algorithm sends the prompt along with the example code to an LLM, querying whether the function pointer `word2bool` is used for any specific data validation or transformation purposes.

The LLM responds with 'YES', indicating that the function pointer `word2bool` is actively used to convert grid elements from a word type to a boolean value, determining their significance in the grid. The algorithm sends another prompt to the LLM, requesting detailed information on how `word2bool` influences the data processing within the grid.

The LLM elaborates that `word2bool` is used within the `getsig` function to evaluate each element of a sub-grid (4x6 cells starting from each grid cell), contributing to a signature computation for each grid cell based on whether the elements are nonzero. Each nonzero element found by `word2bool` effectively contributes to the computed signature by increasing the value, which is accumulated in a specific pattern (multiplication by 2 followed by an addition).

The algorithm then parses the response, identifying how the function `getsig` utilizes `word2bool` to generate signatures that are presumably used for further processing or decision-making. Based on this understanding, the algorithm updates the CICFG by marking these interactions between `findletters`, `getsig`, and `word2bool` as critical components of the data processing workflow in the application.

This dynamic interaction mapped by the algorithm between function pointers and the grid processing logic provides a detailed view of the application's computational strategies, crucial for optimizing performance and ensuring the accuracy of process outcomes.


% ===================================================================
% C feature: conditional compilation 
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Conditional Compilation Analysis - C feature}}
\label{algo:conditionalCompilationAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeConditionalCompilation}{AnalyzeConditionalCompilation}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGNode}{UpdateCICFGNode}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Return}{return}
\SetKw{Continue}{continue}
\LinesNumbered
\KwIn{Set of files $F$}
\KwOut{Updated CICFG}

\Fn{\AnalyzeConditionalCompilation{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:iterateFiles}
        \textit{res} $\gets$ \SendToLLM{"Given the following file, analyze and determine whether Conditional Compilation is used. If the file uses conditional compilation, just output 'YES'; if not, output 'NO.' NO explanation." + file content}\;\label{line:checkConditionalCompilation}
        \If{res == "NO"}{
            \Continue\;\label{line:checkResponse}
        }
        \Else{
            start\_file.append(file)\;
            \textit{resp} $\gets$ \SendToLLM{"List all statements within the conditional compilation blocks, including their line numbers and control flow relationships. For control flow, specify the source and target line numbers of each possible execution path, including the paths that enter and exit the conditional compilation blocks."}\;\label{line:listStatements}
            \If{resp is empty}{
                \Continue\;\label{line:checkEmptyResponse}
            }
            \Else{
                \textit{statementList} $\gets$ parse \textit{resp} into list of statements with line numbers\;\label{line:parseResponse}
                \textit{controlFlowList} $\gets$ parse \textit{resp} into list of control flow edges (source line, target line)\;
                \ForEach{(line\_number, statement) in statementList}{\label{line:updateNodesStart}
                    \textit{compilationCondition} $\gets$ Extract compilation condition from \textit{statement}\;
                    \UpdateCICFGNode{file, line\_number, statement, \{"compilationCondition": compilationCondition\}}\;
                    is\_updated $\gets$ true\;
                }\label{line:updateNodesEnd}
                \ForEach{(source\_line, target\_line) in controlFlowList}{\label{line:updateEdgesStart}
                    \textit{compilationCondition} $\gets$ Extract compilation condition from \textit{statement}\;
                    \UpdateCICFGEdge{file, source\_line, target\_line, \{"compilationCondition": compilationCondition\}}\;
                    is\_updated $\gets$ true\;
                }\label{line:updateEdgesEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}


\Fn{\SendToLLM{prompt}}{\label{line:sendToLLM}
    \Return{LLM(prompt)}\; \tcp{Use LangChain or another LLM interface}
}

\end{algorithm*}




\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm processes each file in the set $F$ one at a time (line~\ref{line:iterateFiles}). For each file, it first checks whether conditional compilation is used by sending a prompt to the LLM (line~\ref{line:checkConditionalCompilation}). The prompt asks the LLM to analyze the file and output 'YES' if conditional compilation is used or 'NO' otherwise, with no explanation.

If the LLM responds with 'NO' (line~\ref{line:checkResponse}), the algorithm continues to the next file. If the response is 'YES', it proceeds to extract detailed information about the conditional compilation blocks. It sends another prompt to the LLM, requesting a list of all statements within the conditional compilation blocks, including their line numbers and control flow relationships (line~\ref{line:listStatements}). The prompt specifically asks for the source and target line numbers of each possible execution path, including the paths that enter and exit the conditional compilation blocks.

If the response from the LLM is empty (line~\ref{line:checkEmptyResponse}), the algorithm moves on to the next file. Otherwise, it parses the response into two data structures: \texttt{statementList}, which contains statements with their corresponding line numbers, and \texttt{controlFlowList}, which contains control flow edges represented as pairs of source and target line numbers (line~\ref{line:parseResponse}).

The algorithm then updates the CICFG by adding nodes for each statement using the \texttt{UpdateCICFGNode} function (lines~\ref{line:updateNodesStart}--\ref{line:updateNodesEnd}). For each statement in \texttt{statementList}, it adds the statement at the specified line number under the given file in the CICFG.

Next, it updates the control flow edges in the CICFG using the \texttt{UpdateCICFGNodeEdge} function (lines~\ref{line:updateEdgesStart}--\ref{line:updateEdgesEnd}). For each control flow edge in \texttt{controlFlowList}, it adds an edge from the source line to the target line in the CICFG under the given file.


% The \texttt{UpdateCICFGNode} function (line~\ref{line:updateCICFGNode}) is responsible for adding a statement at a specific line number to the CICFG for the given file. The \texttt{UpdateCICFGNodeEdge} function (line~\ref{line:updateCICFGNodeEdge}) adds a control flow edge between two line numbers in the CICFG for the given file.

% The \texttt{SendToLLM} function (line~\ref{line:sendToLLM}) handles communication with the LLM by sending the provided prompt and returning the response.


% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/conditional.png}
% 	\caption{conditional compilation real world example.}
% 	\label{fig:conditional}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=C, caption=conditional compilation real world example., label=fig:conditional]
#ifdef _MSC_VER
#include <intrin.h>
#endif
#include <arm_neon.h>

int main(int argc, char **argv)
{
    float *src = (float*)argv[argc-1];
    float32x4_t v1 = vdupq_n_f32(src[0]);
    float32x4_t v2 = vdupq_n_f32(src[1]);
    float32x4_t v3 = vdupq_n_f32(src[2]);
    int ret = (int)vgetq_lane_f32(vfmaq_f32(v1, v2, v3), 0);
#ifdef __aarch64__
    double *src2 = (double*)argv[argc-2];
    float64x2_t vd1 = vdupq_n_f64(src2[0]);
    float64x2_t vd2 = vdupq_n_f64(src2[1]);
    float64x2_t vd3 = vdupq_n_f64(src2[2]);
    ret += (int)vgetq_lane_f64(vfmaq_f64(vd1, vd2, vd3), 0);
#endif
    return ret;
}
\end{lstlisting}

\noindent\textbf{Usage with example}
As shown in figure~\ref{fig:conditional}, the algorithm processes a file containing conditional compilation directives for different architectures. The algorithm sends the prompt to an LLM, along with the example code, querying whether conditional compilation is used. The LLM responds with 'YES', indicating that conditional compilation directives like `\#ifdef` and `\#endif` are present, which conditionally include different headers and execute different code paths depending on the architecture.

The algorithm sends another prompt to the LLM, asking for detailed analysis of all statements within the conditional compilation blocks, including their line numbers and control flow relationships. The LLM responds by listing the statements within the `\#ifdef \_MSC\_VER` and `\#ifdef \_\_aarch64\_\_` blocks, noting that these blocks include specific SIMD (Single Instruction, Multiple Data) operations optimized for the respective architectures.
The algorithm updates the CICFG by adding nodes for the specific operations within each conditional compilation block and edges that depict the potential flow of execution between these nodes based on the architecture being compiled for.



% ===================================================================
% C feature: dynamic linking 
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Dynamic Linking Analysis - C feature}}
\label{algo:dynamicLinkingAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeDynamicLinking}{AnalyzeDynamicLinking}
\SetKwFunction{FindDynamicCalls}{FindDynamicCalls}
% \SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Return}{return}
\SetKw{Continue}{continue}
\LinesNumbered
\KwIn{Set of files $F$}
\KwOut{Updated CICFG}

\Fn{\AnalyzeDynamicLinking{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:iterateFiles}
        res $\gets$ \SendToLLM{"Given the following file, analyze and determine whether dynamic linking is used. If dynamic linking is used, output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:checkDynamicLinking}
        \If{res == "NO"}{
            \Continue\;\label{line:checkResponse}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List the variables (e.g., handles, function pointers) involved in dynamic linking and the names of the external functions they reference. Provide the line numbers where these external functions are called via dynamic linking in this file. If none, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:listVariables}
            \If{resp == "NO"}{
                \Continue\;\label{line:checkEmptyResponse}
            }
            \Else{
                callList $\gets$ parse \textit{resp} into list of (\textit{line\_number}, \textit{external\_func\_name})\;\label{line:parseCalls}
                variables $\gets$ retrieve list of dynamic linking variables from \textit{resp}\;
                \ForEach{(line\_number, external\_func\_name) in callList}{
                    target\_file\_name, target\_line\_number $\gets$ retrieve the file name and entry line number of \textit{external\_func\_name} from CICFG\;
                    \UpdateCICFGEdge{file, line\_number, target\_file\_name, target\_line\_number}\;\label{line:updateNodes}
                    is\_updated $\gets$ true\;
                }
                \ForEach{variable in variables}{
                    \FindDynamicCalls{variable, file content}\;\label{line:recursiveCall}
                }
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}

\Fn{\FindDynamicCalls{variable, code}}{
    % files\_code $\gets$ retrieve the code of each file in files according to current CICFG\;
    res $\gets$ \SendToLLM{"In the following code, does the variable '" + \textit{variable} + "' get passed to other functions? If yes, output $<$function name, variable name$>$. If not, output 'NO.'" + \textit{code}}\;\label{line:sendToLLM}
    \If{res == "NO"}{
        \Return\;
    }
    \Else{
        % newFuncs $\gets$ parse \textit{res} into list of (\textit{function\_name}, \textit{parameter\_name})\;
        \ForEach{(func\_name, param\_name) in res}{
            func\_code $\gets$ retrieve the code of \textit{func\_name}\;
            res $\gets$ \SendToLLM{"Does the variable '" + \textit{param\_name} + "' call any external functions via dynamic linking in the following code? If yes, output $<$line no., external functions name$>$. If not, output 'NO.'" + func\_code}\;
            \If{res != "NO"}{
                % callList $\gets$ parse \textit{res} into list of (\textit{line\_number}, \textit{external\_func\_name})\;
                \ForEach{(line\_number, external\_func\_name) in res}{
                    func\_file\_name $\gets$ retrieve the file name of \textit{func\_name} from CICFG\;
                    target\_file\_name, target\_line\_number $\gets$ retrieve the file name and entry line number of \textit{external\_func\_name} from CICFG\;
                    \UpdateCICFGEdge{func\_file\_name, line\_number, target\_file\_name, target\_line\_number}\;
                    is\_updated $\gets$ true\;
                }
            }
            \FindDynamicCalls{param\_name, func\_code}\;
        }
    }
}

\end{algorithm*}




\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm begins by processing each file in the set $F$ one at a time (line~\ref{line:iterateFiles}). For each file, it first checks whether dynamic linking is used by sending a prompt to the LLM (line~\ref{line:checkDynamicLinking}). The prompt asks the LLM to analyze the file and output 'YES' if dynamic linking is used or 'NO' otherwise, with no explanation.

If the LLM responds with 'NO' (line~\ref{line:checkResponse}), the algorithm continues to the next file. If the response is 'YES', it proceeds to extract information about the variables involved in dynamic linking and the external functions they reference. It sends another prompt to the LLM (line~\ref{line:listVariables}), requesting a list of variables (e.g., handles, function pointers) involved in dynamic linking, along with the names of the external functions they reference and the line numbers where these external functions are called via dynamic linking in this file.

If the response from the LLM is empty (line~\ref{line:checkEmptyResponse}), the algorithm moves on to the next file. Otherwise, it parses the response into a list called \texttt{callList}, which contains tuples of line numbers and external function names where dynamic linking calls occur (line~\ref{line:parseCalls}). It also extracts the list of dynamic linking variables for further analysis.

The algorithm then updates the CICFG by adding edges representing calls to external functions via dynamic linking using the \texttt{UpdateCICFG} function (line~\ref{line:updateNodes}). This function adds an edge from the code at the specified line number in the file to the external function in the CICFG.

Next, the algorithm recursively checks whether the dynamic linking variables (pointers or handles) are passed to other functions by calling the \texttt{FindDynamicCalls} function (line~\ref{line:recursiveCall}). The purpose of the \texttt{FindDynamicCalls} function is to ensure that any uses of the dynamic linking variables in other functions are identified, especially if these variables are used to call external functions via dynamic linking within those functions.

In the \texttt{FindDynamicCalls} function, the algorithm sends a prompt to the LLM (line~\ref{line:sendToLLM}) to determine if the variable is passed to other functions in the provided code. If the LLM responds with 'NO', the recursion terminates for that variable. If the LLM identifies that the variable is passed to other functions, it provides the function names and the parameter names that receive the variable.

For each such function, the algorithm retrieves the code of the function and sends another prompt to the LLM to check if the parameter (which holds the dynamic linking variable) is used to call any external functions via dynamic linking within that function. If such calls are found, the algorithm updates the CICFG by adding edges from the code lines where the calls occur to the corresponding external functions using the \texttt{UpdateCICFG} function.

The algorithm then recursively calls \texttt{FindDynamicCalls} for the parameter name in the context of the new function (last line within the \texttt{FindDynamicCalls} function). This recursive invocation ensures that the analysis continues if the variable is further passed down to other functions, covering all possible usages of the dynamic linking variable throughout the program.

By thoroughly exploring all functions that the dynamic linking variable is passed to, and identifying any external function calls made using it, the algorithm ensures that the CICFG accurately reflects all external function calls made via dynamic linking, even when the dynamic linking variables are passed through multiple layers of function calls.

% The use of \texttt{FindDynamicCalls} is crucial for capturing indirect usages of dynamic linking variables, preventing any missing edges in the CICFG that could occur if only direct usages were considered. This comprehensive analysis is essential for accurate program analysis, especially in languages and environments where dynamic linking is prevalent.

% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/dynamiclinking.png}
% 	\caption{dynamic linking real world example.}
% 	\label{fig:dynamic}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=C, firstnumber=36, caption=dynamic linking real world example., label=fig:dynamic]
#ifdef __aarch64__
void * selinux = dlopen("/system/lib64/libselinux.so", RTLD_LAZY);
#else
void * selinux = dlopen("/system/lib/libselinux.so", RTLD_LAZY);
#endif

if (selinux) {
    void *getcon = dlsym(selinux, "getcon");
    const char *error = dlerror();
    if (error) {
        LOGV("dlsym error %s", error);
    } else {
        getcon_t *getcon_p = (getcon_t*)getcon;
        char *secontext;
        int ret = (*getcon_p)(&secontext);
        LOGV("%d %s", ret, secontext);
        void *setcon = dlsym(selinux, "setcon");
        const char *error = dlerror();
        if (error) {
            LOGV("dlsym setcon error %s", error);
        } else {
            setcon_t *setcon_p = (setcon_t*)setcon;
            ret = (*setcon_p)("u:r:shell:s0");
            ret = (*getcon_p)(&secontext);
            LOGV("context %d %s", ret, secontext);
        }
    }
    dlclose(selinux);
} else {
    LOGV("no selinux");
}

system("/system/bin/sh -i");
\end{lstlisting}


The LLM provides:
\begin{itemize}
    \item Variables and External Functions:
    \begin{itemize}
        \item Variable: `selinux`
            - External Function: `dlopen`
        \item Variable: `getcon`
            - External Function: `getcon` at line where `dlsym(selinux, "getcon")` is called.
        \item Variable: `setcon`
            - External Function: `setcon` at line where `dlsym(selinux, "setcon")` is called.
    \end{itemize}
\end{itemize}


% ===================================================================
% C feature: inline assembly
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Inline Assembly Analysis - C feature}}
\label{algo:macroExpansionAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeMacroExpansion}{AnalyzeMacroExpansion}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeMacroExpansion{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{algomac:iterateFiles}
        \textit{res} $\gets$ \SendToLLM{"Given the following code, analyze and determine whether the inline assembly is used. If the code uses inline assembly, just output 'YES'; if not, output 'NO.' NO explanation." + file content}\;\label{algomac:checkinline}
        \If{res == "NO"}{
            continue\;\label{algomac:checkResponse}
        }
        \Else{
            start\_file.append(file)\;
            \textit{resp} $\gets$ \SendToLLM{"Determine whether functions are called in the inline assembly code block. If yes, output $<$names of the called functions, line numbers of the callsite$>$. Otherwise output 'NO.'" + file content}\;\label{algomac:checkInlineAssembly}
            \If{resp == "NO"}{
                continue\;\label{algomac:noFunctionCalls}
            }
            \Else{
                % \textit{func\_calls} $\gets$ parse resp into list of (\textit{function name}, \textit{line number})\;\label{algomac:parseResponse}
                \ForEach{(\textit{func\_name}, \textit{line\_number}) in func\_calls}{\label{algomac:updateCICFGStart}
                    \textit{target\_file\_name}, \textit{target\_line\_number} $\gets$ retrieve the file name and entry line number of \textit{func\_name} from CICFG\;
                    \UpdateCICFGEdge{file, line\_number, target\_file\_name, target\_line\_number}\;\label{algomac:updateCICFG}
                    is\_updated $\gets$ true\;
                }\label{algomac:updateCICFGEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}


\end{algorithm*}


\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm processes each file in the set $F$ one at a time (line~\ref{algomac:iterateFiles}). For each file, it first checks whether the C feature "inline assembly" is used by sending a prompt to the LLM (line~\ref{algomac:checkinline}). The prompt asks the LLM to analyze the code and output 'YES' if such inline assembly is used or 'NO' otherwise.

If the LLM responds with 'NO' (line~\ref{algomac:checkResponse}), the algorithm continues to the next file. If the response is 'YES', the algorithm proceeds to determine whether functions are called within inline assembly code blocks. It sends another prompt to the LLM (line~\ref{algomac:checkInlineAssembly}), asking it to identify any function calls within inline assembly and provide their names and line numbers.

If the LLM responds with 'NO' (line~\ref{algomac:noFunctionCalls}), indicating that there are no function calls within inline assembly, the algorithm moves on to the next file. Otherwise, it parses the LLM's response into a list of function calls, each with the function name and the line number where it is called (line~\ref{algomac:parseResponse}).

% The algorithm then updates the CICFG by adding edges representing these function calls (lines~\ref{algomac:updateCICFGStart}--\ref{algomac:updateCICFGEnd}). For each function call in the list, it calls the \UpdateCICFG function (line~\ref{algomac:updateCICFG}), which adds an edge from the caller to the callee in the CICFG at the specified line number.

The \SendToLLM function (line~\ref{algomac:SendToLLM}) handles communication with the LLM by sending the provided prompt and returning the response.

% The \UpdateCICFG function (line~\ref{algomac:UpdateCICFG}) updates the CICFG by adding an edge from the caller to the callee at the specified line number.


% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/inline+macro.png}
%         %\includegraphics[width=1.0\linewidth]{figure/methodology-overview.pdf}
% 	\caption{inline assembly and macro real world example.}
% 	%Overview of the data processing}
% 	\label{fig:inline+macro}
% 	\vspace{-6pt}
% \end{figure*}
% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/inline+macro2.png}
%         %\includegraphics[width=1.0\linewidth]{figure/methodology-overview.pdf}
% 	\caption{inline assembly and macro real world example.}
% 	%Overview of the data processing}
% 	\label{fig:inline+macro2}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=C, firstnumber=53, caption=inline assembly and macro real world example., label=fig:inline+macro]
#define CALL_FUNC(func) \
    asm ("lea 0x08(%rip), %rax"); \
    asm ("push %rax"); \
    asm ("push %0" : : "i" (func)); \
    asm ("ret");
\end{lstlisting}

\begin{lstlisting}[language=C, firstnumber=369, caption=inline assembly and macro real world example., label=fig:inline+macro2]
if (ptr) {
    CALL_FUNC(fdSetAll);
    if ((ret = select(getMaxFd() + 1, &coreServ.readfs, NULL, NULL, &coreServ.timeout)) == -1) {
        JUNK1();
    }
}
\end{lstlisting}




\noindent\textbf{Usage with example}
As illustrated by figure~\ref{fig:inline+macro2}, the algorithm processes a file containing definitions of macros that encapsulate inline assembly instructions designed to call functions dynamically. The algorithm sends the prompt with the code example to an LLM, asking it to analyze and determine if inline assembly is used. The LLM responds affirmatively, indicating that the macro `CALL\_FUNC` uses inline assembly.

Upon further prompting by the algorithm, the LLM identifies that the inline assembly within the `CALL\_FUNC` macro executes function calls by manipulating the program's instruction pointer to jump to function addresses dynamically. Specifically, the LLM points out that the function `fdSetAll` is invoked through this macro at the specific line where `CALL\_FUNC(fdSetAll);` is used.

The algorithm then parses this response and recognizes that `fdSetAll` is called via the macro expansion at that particular line. With this understanding, the algorithm proceeds to update the Control and Interprocedural Call Graph (CICFG) by adding an edge from the current function, where the macro is employed, directly to `fdSetAll`. 

% This update significantly aids in enhancing the graph's accuracy by explicitly representing the dynamic function calls made via inline assembly within macros.

% The example effectively demonstrates how the pseudocode algorithm uses LLM responses to identify and document dynamic assembly-driven function calls in source code, ensuring that the CICFG is precise and comprehensive in capturing actual execution flows influenced by macro-embedded inline assembly.


% ===================================================================
% C feature: macros expanding to function calls
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Macros Expanding to Function Calls Analysis - C feature}}
\label{algo:macroExpansionAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeMacroExpansion}{AnalyzeMacroExpansion}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeMacroExpansion{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:macro_iterateFiles}
        res $\gets$ \SendToLLM{"Given the following code, analyze and determine Macros Expanding to Function Calls is used. If the code uses this feature, just output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:macro_checkMacros}
        \If{res == "NO"}{
            continue\;\label{line:macro_checkResponse}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"Determine whether functions are called in macros expanding. If yes, output $<$the name of the called function, line number of the callsite$>$. Otherwise output 'NO.'" + \textit{file content}}\;\label{line:macro_findFunctionCalls}
            \If{resp == "NO"}{
                continue\;\label{line:macro_noFunctionCalls}
            }
            \Else{
                % func\_calls $\gets$ parse \textit{resp} into the list of (function name, line number)\;\label{line:macro_parseResponse}
                \ForEach{(func\_name, line\_number) in resp}{\label{line:macro_updateCICFGStart}
                    target\_file\_name, target\_line\_number $\gets$ retrieve the file name and entry line number of \textit{func\_name} from CICFG\;
                    \UpdateCICFGEdge{file, line\_number, target\_file\_name, target\_line\_number}\;\label{line:macro_updateCICFG}
                    is\_updated $\gets$ true\;
                }\label{line:macro_updateCICFGEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}


\end{algorithm*}


\FloatBarrier 

\noindent\textbf{Explanation:}

The algorithm processes each file in the set $F$ one at a time (line~\ref{line:macro_iterateFiles}). For each file, it first sends a prompt to the LLM to determine whether macros that expand to function calls are used in the code (line~\ref{line:macro_checkMacros}). The prompt asks the LLM to output 'YES' if such macros are used or 'NO' otherwise, without any explanation.

If the LLM responds with 'NO' (line~\ref{line:macro_checkResponse}), the algorithm proceeds to the next file. If the response is 'YES', it sends another prompt to the LLM to identify whether functions are called within the macro expansions (line~\ref{line:macro_findFunctionCalls}). The LLM is instructed to output the names of the called functions and the line numbers where these calls occur, or 'NO' if none are found.

If the LLM responds with 'NO' (line~\ref{line:macro_noFunctionCalls}), indicating that no function calls are made within macros, the algorithm moves on to the next file. 
% If the LLM provides a list of function calls, the algorithm parses the response into a list of function names and their corresponding line numbers (line~\ref{line:macro_parseResponse}).

% The algorithm then updates the CICFG by adding edges for each function call identified (lines~\ref{line:macro_updateCICFGStart}--\ref{line:macro_updateCICFGEnd}). For each function call, it invokes the \UpdateCICFG function (line~\ref{line:macro_updateCICFG}), which adds an edge from the caller to the callee at the specified line number in the CICFG.

% The \SendToLLM function (lines~\ref{line:macro_sendToLLMStart}--\ref{line:macro_sendToLLMEnd}) handles communication with the LLM, sending the provided prompt and returning the response. The \UpdateCICFG function (lines~\ref{line:macro_updateCICFGFnStart}--\ref{line:macro_updateCICFGFnEnd}) updates the CICFG accordingly.


\noindent\textbf{Usage with example}
As shown in Figure~\ref{fig:inline+macro}, the algorithm processes the file containing the macro definition and its usage.
The algorithm sends the prompt with the example and the LLM responds with 'YES', indicating that macros expanding to function calls are present.
The algorithm sends another prompt to the LLM, and the LLM responds with that the macro 'CALL\_FUNC' expands to inline assembly that effectively calls the function 'fdSetAll' at the line where 'CALL\_FUNC(fdSetAll);' is used. 
The algorithm parses the response and identifies that the function 'fdSetAll' is called via the macro expansion at the line where 'CALL\_FUNC(fdSetAll);' is used.
The algorithm updates the CICFG by adding an edge from the current function to 'fdSetAll' at the line where the macro is used.





% ===================================================================
% C feature: goto statements
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Goto Analysis - C feature}}
\label{algo:gotoSetjmpAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeGotoSetjmp}{AnalyzeGotoSetjmp}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $Files$ from a program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeGotoSetjmp{Files}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $Files$}{\label{line:goto_iterateFiles}
        res $\gets$ \SendToLLM{"Given the following C file, analyze and determine whether the C Goto Statements are used. If the file uses the feature, just output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:goto_checkUsage}
        \If{res == "NO"}{
            \Continue\;\label{line:goto_noUsage}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List all occurrences of Goto Statements usages, including $<$the source function name, target label/function name, source line numbers, target line number$>$. Otherwise, output 'NO.'" + \textit{file content}}\;\label{line:goto_listOccurrences}
            \If{resp == "NO"}{
                \Continue\;\label{line:goto_noOccurrences}
            }
            \Else{
                % usageList $\gets$ list of (source function, target label/function, source line number, target line number) from \textit{resp}\;\label{line:goto_parseResponse}
                \ForEach{(srcFunc, target, srcLine, tgtLine) in resp}{\label{line:goto_updateCICFGStart}
                    % annotation $\gets$ create the annotation dictionary \{"goto":srcFunc-target\}\;
                    \UpdateCICFGEdge{file, srcLine, tgtLine, \{"goto":srcFunc+"-"+target\}}\;\label{line:goto_updateCICFG}
                    is\_updated $\gets$ true\;
                }\label{line:goto_updateCICFGEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}


\end{algorithm*}



\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm processes each file in the set $Files$ one at a time (line~\ref{line:goto_iterateFiles}). For each file, it first sends a prompt to the LLM to determine whether Goto statements or Setjmp/Longjmp functions are used in the code (line~\ref{line:goto_checkUsage}). The prompt asks the LLM to output 'YES' if any of these features are used or 'NO' otherwise, without any explanation.

If the LLM responds with 'NO' (line~\ref{line:goto_noUsage}), the algorithm proceeds to the next file. If the response is 'YES', it sends another prompt to the LLM to list all occurrences of Goto statements and Setjmp/Longjmp usages (line~\ref{line:goto_listOccurrences}). The LLM is instructed to provide the source function name, target label or function name, source line numbers, and target line numbers. If none are found, it should output 'NO'.

If the LLM responds with 'NO' (line~\ref{line:goto_noOccurrences}), indicating that no occurrences are found, the algorithm moves on to the next file. If the LLM provides a list of usages, the algorithm parses the response into a list of tuples containing the source function, target label or function, source line number, and target line number (line~\ref{line:goto_parseResponse}).

% The algorithm then updates the CICFG by adding edges for each usage identified (lines~\ref{line:goto_updateCICFGStart}--\ref{line:goto_updateCICFGEnd}). For each usage, it invokes the \UpdateCICFG function (line~\ref{line:goto_updateCICFG}), which adds an edge from the source to the target at the specified line numbers in the CICFG.

% The \SendToLLM function (lines~\ref{line:goto_sendToLLMStart}--\ref{line:goto_sendToLLMEnd}) handles communication with the LLM, sending the provided prompt and returning the response. The \UpdateCICFG function (lines~\ref{line:goto_updateCICFGFnStart}--\ref{line:goto_updateCICFGFnEnd}) updates the CICFG accordingly.

% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/goto.png}
% 	\caption{goto and longjump real world example.}
% 	\label{fig:goto}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=C, firstnumber=194, caption=goto and longjump real world example., label=fig:goto]
int main(int argc, char *argv[])
{
    int mode = (argc > 0 && strcmp(basename(argv[0]), "unx") == 0) ? DECOMPRESS : COMPRESS;
    FILE *istream = NULL, *ostream = NULL;
    int force = 0;

    parse: switch (getopt(argc, argv, "zdf019gk")) {
        case 'z':
            mode = COMPRESS;
            goto parse;
        case 'd':
            mode = DECOMPRESS;
            goto parse;
        case 'f':
            force = 1;
            goto parse;
        case 'o':
            max_layers = 0;
            goto parse;
        case '1':
            max_layers = 1;
            goto parse;
        case '9':
            max_layers = 255;
            goto parse;
        case 'k':
            goto parse;
        case 'h':
            print_help(argv[0]);
            return 0;
        default:
            abort();
        case -1:
            ;
    }
}
\end{lstlisting}

\FloatBarrier 
\noindent\textbf{Usage with example:}
As shown in Figure~\ref{fig:goto}, the algorithm processes the file containing the code snippet. 
The algorithm sends the prompt to the LLM with the example code. The LLM responds with 'YES' because the code uses Goto statements.
The algorithm sends another prompt to the LLM, and the LLM responds with a list of usages:
\begin{itemize}
    \item Goto statements:
    \begin{itemize}
        \item Source Function: main function.
        \item Source Lines: Lines 203, 206, 209, 212, 215, 218, 220
        \item Target Label: parse
        \item Target Line: Line 200
    \end{itemize}
\end{itemize}

The algorithm parses the response into a list of usages, and then updates the CICFG by adding edges for each goto statement:
For example, for goto parse; at line 203:\\UpdateCICFG{main, parse, 203, 200}

% ===================================================================
% C feature: setjmp/longjmp
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Setjmp/Longjmp Analysis - C Feature}}
\label{algo:setjmpLongjmpAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeSetjmpLongjmp}{AnalyzeSetjmpLongjmp}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $Files$ from a program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeSetjmpLongjmp{Files}}{
    bufferSet $\gets$ empty set\;\label{line:setjmp_initBufferSet}
    \tcp{First pass: Find all 'setjmp' usages and collect buffer variables}
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $Files$}{\label{line:setjmp_iterateFiles}
        res $\gets$ \SendToLLM{"Given the following C file, analyze and determine whether the C feature 'setjmp' is used. If yes, output buffer variable names with their line numbers in the format $<$buffer variable name, line number$>$. If not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:setjmp_checkUsage}
        \If{res == "NO"}{
            \Continue\;\label{line:setjmp_noUsage}
        }
        \Else{
            start\_file.append(file)\;
            \tcp{Parse the response to extract buffer variable names and line numbers}
            \ForEach{(bufferVar, lineNum) in res}{
                bufferSet $\gets$ bufferSet $\cup$ \{(bufferVar, file, lineNum)\}\;\label{line:setjmp_collectBuffers}
            }
        }
    }
    \tcp{Second pass: Search for 'longjmp' usages matching the collected buffer variables}
    \ForEach{file in $Files$}{\label{line:longjmp_iterateFiles}
        lines $\gets$ read lines from \textit{file}\;\label{line:longjmp_readLines}
        \ForEach{line in lines}{\label{line:longjmp_iterateLines}
            srcLineNum $\gets$ line number of \textit{line}\;\label{line:longjmp_getLineNumber}
            \ForEach{(bufferVar, setjmpFile, setjmpLineNum) in bufferSet}{\label{line:longjmp_iterateBuffers}
                \If{\texttt{longjmp(*)} in line}{\label{line:longjmp_match}
                    res $\gets$ \SendToLLM{"Given the following C files, analyze and determine whether the longjmp in "+ '\textit{file}' +" at line "+ '\textit{line}' +" can jump back to setjmp statement in "+ '\textit{setjmpFile}' +" at line "+ '\textit{setjmpLineNum}' +". If yes, output "YES". If not, output 'NO.' NO explanation." + \textit{file content} + \textit{setjmpFile content}}\;\label{line:check_match}
                    \If{res == "YES"}{
                        \UpdateCICFGEdge{file, srcLineNum, setjmpFile, setjmpLineNum}\;\label{line:setjmp_updateCICFG}
                        is\_updated $\gets$ true\;
                    }
                    
                }
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}
\end{algorithm*}

The algorithm aims to analyze C programs to identify and model the usage of `setjmp` and `longjmp`, which are features in C that enable non-local jumps, altering the normal flow of control.

\textbf{First Pass: Identifying `setjmp` Usages.}
The algorithm starts by initializing an empty set called `bufferSet` to store information about buffer variables used with `setjmp` (line~\ref{line:setjmp_initBufferSet}). It iterates through each file in the set `Files` (line~\ref{line:setjmp_iterateFiles}). For each file, it sends a prompt to an LLM (Language Model) asking whether `setjmp` is used in the file (line~\ref{line:setjmp_checkUsage}). The prompt requests that if `setjmp` is used, the LLM should output the buffer variable names and their line numbers in a specific format; otherwise, it should output 'NO' with no explanation. If the LLM responds with 'NO' (line~\ref{line:setjmp_noUsage}), the algorithm continues to the next file. If the LLM provides buffer variable names and line numbers, the algorithm parses this response and adds each buffer variable along with the file name and line number to the `bufferSet` (line~\ref{line:setjmp_collectBuffers}). This set will be used in the second pass to find corresponding `longjmp` calls.

\textbf{Second Pass: Matching `longjmp` Calls with `setjmp` Buffers}
The algorithm iterates over each file once more (line~\ref{line:longjmp_iterateFiles}). It reads all the lines from the current file (line~\ref{line:longjmp_readLines}). For each line in the file (line~\ref{line:longjmp_iterateLines}), it retrieves the line number (line~\ref{line:longjmp_getLineNumber}). For each buffer variable stored in `bufferSet` (line~\ref{line:longjmp_iterateBuffers}), the algorithm checks whether a `longjmp` call in the current line might correspond to the `setjmp` call that used this buffer. It checks if the current line contains a `longjmp` call (line~\ref{line:longjmp_match}). This is determined by searching for the pattern `longjmp(*)`, where `*` represents any arguments. If a `longjmp` call is found, the algorithm sends a prompt to the LLM (line~\ref{line:check_match}) to analyze whether the `longjmp` in the current file and line can jump back to the `setjmp` statement in the `setjmpFile` at `setjmpLineNum`. The prompt includes both the content of the current file and the file containing the `setjmp` call. The LLM is asked to output 'YES' if such a jump is possible, or 'NO' otherwise, with no explanation.

If the LLM responds with 'YES' (line~\ref{line:setjmp_updateCICFG}), indicating that the `longjmp` can jump back to the `setjmp` statement, the algorithm updates the CICFG by adding an edge from the `longjmp` call site to the `setjmp` call site using the `UpdateCICFGEdge` function.
This edge represents the non-linear control flow caused by the `longjmp` operation, which effectively transfers execution back to the point where `setjmp` was called.



\begin{lstlisting}[language=C, firstnumber=32, caption=setjmp real world example., label=fig:sejmp]
if (doerror)
    longjmp(backdoorjmp, 1);

memmove(jb, backdoorjmp, sizeof(jb));
if (setjmp(backdoorjmp)) {
    // handling code
}
\end{lstlisting}

We apply the \textbf{Setjmp/Longjmp Analysis} algorithm to this code as shown in Figure~\ref{fig:sejmp}.

The algorithm scans the file to find usages of \texttt{setjmp}.

It finds a \texttt{setjmp} call with the buffer variable \texttt{backdoorjmp} on line 4.
The buffer variable and its line number are collected:
\textit{bufferSet={(backdoorjmp,line 4)}}.

The algorithm searches for \texttt{longjmp} calls that use the buffer variables in \texttt{bufferSet}.

It finds a \texttt{longjmp} call using \texttt{backdoorjmp} on \textit{longjmp(backdoorjmp, 1);}.
An edge is added to the CICFG from the \texttt{longjmp} at line 2 to the \texttt{setjmp} at line 4.





% ===================================================================
% Python feature: dynamic typing
\begin{algorithm*}[tp]
\caption{\footnotesize{Dynamic Typing Analysis - Python feature}}
\label{algo:dynamicTypingAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeDynamicTyping}{AnalyzeDynamicTyping}
\SetKwFunction{FindVariableAssignments}{FindVariableAssignments}
\SetKwFunction{TraceVariableUsage}{TraceVariableUsage}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a Python program}\label{dynamic_input}
\KwOut{Updated CICFG}\label{dynamic_output}

\Fn{\AnalyzeDynamicTyping{F}}{\label{dynamic_main_function}
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{dynamic_each_file}
        res $\gets$ \SendToLLM{"Does the given code use dynamic typing? If yes, output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{dynamic_check_typing}
        \If{res == "NO"}{\label{dynamic_no_typing}
            \Continue;\label{dynamic_continue_no_typing}
        }
        \Else{\label{dynamic_yes_typing}
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List the variables that are assigned functions or receive functions as arguments in the given code. For each variable, provide $<$variable name, the possible functions it can reference$>$." + \textit{file content}}\;\label{dynamic_list_variables}
            % varFuncMap $\gets$ parse \textit{resp} into a mapping of variables to possible functions\;\label{dynamic_parse_response}
            \ForEach{variable in resp.keys()}{\label{dynamic_each_variable}
                callSites $\gets$ \TraceVariableUsage{variable, [\textit{file content}]}\;\label{dynamic_trace_usage}
                \ForEach{callSite in callSites}{\label{dynamic_each_callsite}
                    caller $\gets$ \textit{callSite.function}\;\label{dynamic_get_caller}
                    line\_number $\gets$ \textit{callSite.line}\;\label{dynamic_get_line}
                    \ForEach{callee in resp[variable]}{\label{dynamic_each_callee}
                        target\_file\_name, target\_line\_number $\gets$ retrieve the file name and entry line number of \textit{callee} from CICFG\;
                        \UpdateCICFGEdge{file, line\_number, target\_file\_name, target\_line\_number}\;\label{dynamic_update_cicfg}
                        is\_updated $\gets$ true\;
                    }
                }
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}

\Fn{\TraceVariableUsage{variable, code\_list}}{\label{dynamic_trace_function}
    callSites $\gets$ []\;\label{dynamic_init_callsites}
    code $\gets$ \textit{code\_list}[-1]\;\label{dynamic_get_code}
    res $\gets$ \SendToLLM{"In the following code, find all places where the variable '" + variable + "' is called as a function. For each occurrence, provide $<$the function name, line number where it is called$>$. If cannot find, output 'No'" + \textit{code}}\;\label{dynamic_find_calls}
    \If{res == "NO"}{\label{dynamic_no_calls}
        \Return{callSites}\;\label{dynamic_return_empty}
    }
    \Else{\label{dynamic_found_calls}
        % calls $\gets$ parse \textit{res} into a list of call sites (function name and line number)\;\label{dynamic_parse_calls}
        callSites.extend(\textit{res})\;\label{dynamic_extend_callsites}
        res $\gets$ \SendToLLM{"In the following code, find all functions to which the variable '" + variable + "' is passed as an argument. For each function, provide $<$the function name, the parameter name that receives it$>$. If cannot find, output 'No'" + \textit{code}}\;\label{dynamic_find_passed_funcs}
        \If{res == "NO"}{\label{dynamic_no_passed_funcs}
            \Return{callSites}\;\label{dynamic_return_callsites}
        }
        \Else{\label{dynamic_found_passed_funcs}
            % newFuncs $\gets$ parse \textit{res} into a list of (function name, parameter name)\;\label{dynamic_parse_passed_funcs}
            \ForEach{(newFunc, paramName) in res}{\label{dynamic_each_new_func}
                newFunc\_code $\gets$ retrieve the code of \textit{newFunc} according to current CICFG\;\label{dynamic_retrieve_code}
                \If{\textit{newFunc\_code} $\notin$ \textit{code\_list}}{\label{dynamic_check_code_list}
                    \textit{code\_list}.append(\textit{newFunc\_code})\;\label{dynamic_append_code_list}
                    newCallSites $\gets$ \TraceVariableUsage{paramName, \textit{code\_list}}\;\label{dynamic_recursive_trace}
                    callSites.extend(\textit{newCallSites});\label{dynamic_extend_new_callsites} \tcp{'extend' is used to merge two lists}
                }
            }
        }
    }
    \Return{callSites}\;\label{dynamic_final_return}
}

\end{algorithm*}


\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm starts by analyzing each file in the input set $F$ (\ref{dynamic_each_file}). For each file, it queries an LLM to check if dynamic typing is used in the code (\ref{dynamic_check_typing}). If not (\ref{dynamic_no_typing}), it continues to the next file (\ref{dynamic_continue_no_typing}). Otherwise, it requests details about variables that hold or pass functions (\ref{dynamic_list_variables}).
% mapping them to their possible functions (\ref{dynamic_parse_response}).

Each variable is then traced for its usage in function calls within the code (\ref{dynamic_trace_usage}). The algorithm identifies and records every place where these variables are used as function callers or arguments (\ref{dynamic_find_calls}, \ref{dynamic_find_passed_funcs}). For each function call detected, the algorithm updates the CICFG to reflect these dynamic interactions, adding edges from callers to callee functions at specific line numbers (\ref{dynamic_update_cicfg}).

The recursive tracing of variables through functions (\ref{dynamic_recursive_trace}) ensures that all dynamic usages of variables are captured, even if the variables are passed deeper into the function call stack (\ref{dynamic_extend_new_callsites}). This comprehensive tracking helps in accurately updating the CICFG to reflect the dynamic nature of the Python code.

% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/dynamictyping.png}
% 	\caption{dynamic typing real world example.}
% 	\label{fig:dynamictyping}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=Python, firstnumber=1, caption=dynamic typing real world example., label=fig:dynamictyping]
def is_frozen():
    ...

def is_release():
    ...

count = fro + relea
func = is_frozen if a>thresh else is_release
func()
\end{lstlisting}

\noindent\textbf{Usage with example}
As demonstrated in figure~\ref{fig:dynamictyping}, the algorithm processes a Python script that dynamically assigns function objects to variables and makes conditional function calls. The algorithm sends the code snippet to the LLM and queries whether dynamic typing is used to handle functions. The LLM responds with 'YES', confirming that dynamic typing is indeed present as functions `is\_frozen` and `is\_release` are conditionally assigned to a variable `func` and subsequently called.

The algorithm then sends another prompt to the LLM, asking for a detailed analysis of the variables that receive function objects either through assignment or as function arguments. The LLM responds by identifying that the variable `func` could potentially reference either `is\_frozen` or `is\_release` depending on the evaluation of an expression `a $>$ threshold`.

Parsing the LLM's response, the algorithm identifies that `func()` on line 9 dynamically calls either `is\_frozen()` or `is\_release()` based on runtime conditions. It then updates the CICFG by adding edges from the current function context to both `is\_frozen` and `is\_release`, marking these edges to reflect that the exact call path depends on the runtime value of `a`.

% This dynamic typing analysis helps in understanding how function calls are resolved at runtime and assists in optimizing code analysis and refactoring tools to better handle Python's flexible typing system.



% ===================================================================
% Python feature: decorator
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Decorator Analysis - Python feature}}
\label{algo:decoratorAnalysis2}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeDecorators}{AnalyzeDecorators}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a Python program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeDecorators{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:decorator_iterateFiles}
        res $\gets$ \SendToLLM{"Given the following Python file, analyze and determine whether decorators are used. If yes, just output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:decorator_checkDecorators}
        \If{res == "NO"}{
            \Continue\;\label{line:decorator_noDecorators}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List all decorators in the file and determine whether functions are called within them. If functions are called within decorators, output $<$the decorator name, the function called, the line number where it is called$>$. Otherwise, output 'NO.'" + \textit{file content}}\;\label{line:decorator_findFunctionCalls}
            \If{resp == "NO"}{
                \Continue\;\label{line:decorator_noFunctionCalls}
            }
            \Else{
                % func\_calls $\gets$  parse \textit{resp} into a list of (decorator name, function called, line number)\;\label{line:decorator_parseCalls}
                \ForEach{(decorator\_name, func\_name, line\_number) in resp}{\label{line:decorator_updateCICFGStart}
                    target\_line\_number $\gets$ retrieve the entry line number of \textit{decorator\_name} from CICFG\;
                    annotation $\gets$ generate the annotation dictionary \{"decorator",\textit{decorator\_name}- \textit{func\_name}\}\;
                    \UpdateCICFGEdge{file, line\_number, target\_line\_number, annotation}\;\label{line:decorator_updateCICFG}
                    is\_updated $\gets$ true\;
                }\label{line:decorator_updateCICFGEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}



\end{algorithm*}



\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm processes each file in the set $F$ one at a time (line~\ref{line:decorator_iterateFiles}). For each file, it first checks whether function decorators are used by sending a prompt to the LLM (line~\ref{line:decorator_checkDecorators}). The prompt asks the LLM to analyze the file and output 'YES' if decorators are used or 'NO' otherwise, with no explanation.

If the LLM responds with 'NO' (line~\ref{line:decorator_noDecorators}), the algorithm continues to the next file. If the response is 'YES', it proceeds to identify any functions that are called within the decorators. It sends another prompt to the LLM (line~\ref{line:decorator_findFunctionCalls}), requesting a list of decorators in the file and any functions called within them, along with the line numbers where these calls occur.

If the LLM responds with 'NO' (line~\ref{line:decorator_noFunctionCalls}), indicating that no functions are called within decorators, the algorithm moves on to the next file. 
% If the LLM provides a list of function calls, the algorithm parses the response into a list called \texttt{func\_calls}, which contains tuples of decorator names, function names, and line numbers where the calls occur (line~\ref{line:decorator_parseCalls}).

% The algorithm then updates the CICFG by adding edges representing these function calls (lines~\ref{line:decorator_updateCICFGStart}--\ref{line:decorator_updateCICFGEnd}). For each function call in the list, it calls the \UpdateCICFG function (line~\ref{line:decorator_updateCICFG}), which adds an edge from the decorator to the function called in the CICFG at the specified line number.

% The \SendToLLM function (lines~\ref{line:decorator_sendToLLMStart}--\ref{line:decorator_sendToLLMEnd}) handles communication with the LLM by sending the provided prompt and returning the response.

% The \UpdateCICFG function (lines~\ref{line:decorator_updateCICFGFnStart}--\ref{line:decorator_updateCICFGFnEnd}) updates the CICFG by adding an edge from the caller to the callee at the specified line number.

% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/decorator.png}
% 	\caption{decorator real world example.}
% 	\label{fig:decorator}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=Python, firstnumber=12, caption=decorator real world example., label=fig:decorator]
def decorator_function(train_function):
    def wrapper_function(*args, **kwargs):
        init(*args, **kwargs)
        train_function(*args, **kwargs)
        finish(*args, **kwargs)
    return wrapper_function

@decorator_function
def train(config_obj):
    parking_trainer = Trainer(callbacks=setup_callbacks(config_obj))
\end{lstlisting}

\noindent\textbf{Usage with example}
As shown in figure~\ref{fig:decorator}, the algorithm processes a Python script containing a decorator function `decorator\_function` used to modify the behavior of the `train` function. The algorithm sends the code snippet to an LLM and queries whether decorators are utilized within the code. The LLM responds with 'YES', confirming the presence of a decorator pattern, where the `decorator\_function` wraps the `train` function to enhance its functionality with `init` and `finish` procedures.

The algorithm then sends another prompt to the LLM, asking it to list all decorators in the file and identify any function calls made within these decorators. The LLM responds by detailing that within the `decorator\_function`, the functions `init`, `train\_function` (the decorated function itself), and `finish` are called sequentially. It provides the line numbers where each function is invoked: `init` at line 14, `train\_function` at line 15, and `finish` at line 16.

Armed with this information, the algorithm parses the response and recognizes the dynamic wrapping of the `train` function by `decorator\_function`, with the insertion of additional behavior before and after the main function execution. The algorithm updates the Control and Interprocedural Call Graph (CICFG) by adding edges from the `decorator\_function` to `init`, `train`, and `finish` at their respective line numbers. 

% This update significantly aids in reflecting the enhanced control flow introduced by the decorator, providing a more accurate representation of the program's runtime behavior.

This example effectively demonstrates how the pseudocode algorithm leverages responses from an LLM to map and document the sophisticated use of decorators in Python scripts, ensuring the CICFG is comprehensive and detailed in capturing these high-level programming constructs.


% ===================================================================
% Python feature: first-class functions
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{First-Class Functions Analysis - Python feature}}
\label{algo:firstClassFunctionsAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeFirstClassFunctions}{AnalyzeFirstClassFunctions}
\SetKwFunction{FindFunctionUses}{FindFunctionUses}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a Python program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeFirstClassFunctions{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:firstClass_iterateFiles}
        res $\gets$ \SendToLLM{"Given the following Python code snippet, analyze and determine whether the Python feature, First-Class Functions, is used. If yes, just output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:firstClass_checkFirstClassFunctions}
        \If{res == "NO"}{
            \Continue\;\label{line:firstClass_checkResponse}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List all occurrences where functions are passed as arguments, including $<$the function name is passed, the function it is passed to$>$. If none, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:firstClass_findFunctionPasses}
            \If{resp == "NO"}{
                \Continue\;\label{line:firstClass_noFunctionPasses}
            }
            \Else{
                % passList $\gets$ parse \textit{resp} into list of (\textit{function\_name}, \textit{passed\_to\_function}, \textit{line\_number})\;\label{line:firstClass_parsePasses}
                \ForEach{(func, receiver) in resp}{\label{line:firstClass_processPassesStart}
                    \FindFunctionUses{func, receiver, [\textit{file content}], set()}\;\label{line:firstClass_recursiveCall}
                }\label{line:firstClass_processPassesEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}

\Fn{\FindFunctionUses{function\_name, current\_function, code, visited\_functions}}{
    \If{(function\_name, current\_function) in visited\_functions}{
        \Return\;\label{line:firstClass_alreadyVisited}
    }
    visited\_functions.add((function\_name, current\_function))\;\label{line:firstClass_addVisited}
    res $\gets$ \SendToLLM{"In the following code, within the function '" + \textit{current\_function} + "', is the function '" + \textit{function\_name} + "' called? If yes, provide the $<$line numbers$>$ where it is called. If not, does '" + \textit{function\_name} + "' get passed as an argument to other functions within '" + \textit{current\_function} + "'? If so, provide $<$the names of those functions, the line numbers where this occurs$>$. If neither, output 'NO.'" + \textit{code}}\;\label{line:firstClass_checkFunctionUses}
    \If{res == "NO"}{
        \Return\;\label{line:firstClass_noUses}
    }
    \Else{
        \If{function\_name is called in current\_function}{
            % callLines $\gets$ get list of line numbers where \textit{function\_name} is called from CICFG\;\label{line:firstClass_getCallLines}
            \ForEach{line\_number in res}{
                current\_file\_name $\gets$ retrieve the file name of the \textit{current\_function} from CICFG\;
                target\_file\_name, target\_line\_number  $\gets$ retrieve the target file name and target entry line number of the \textit{function\_name} from CICFG\;
                \UpdateCICFGEdge{current\_file\_name, line\_number, target\_file\_name, target\_line\_number}\;\label{line:firstClass_updateCICFGEdge}
                is\_updated $\gets$ true\;
            }
        }
        \If{function\_name is passed as argument in current\_function}{
            % passList $\gets$ list of (\textit{receiver\_function}, \textit{line\_number}) where \textit{function\_name} is passed\;\label{line:firstClass_getPassList}
            \ForEach{(receiver, line\_number) in res}{
                \FindFunctionUses{function\_name, receiver, code, visited\_functions}\;\label{line:firstClass_recursiveCallInPass}
            }
        }
    }
}

\end{algorithm*}


\FloatBarrier 
\noindent\textbf{Explanation:}
The algorithm begins by processing each file in the set $F$ one at a time (\ref{line:firstClass_iterateFiles}). For each file, it first checks whether first-class functions are used by sending a prompt to the LLM (\ref{line:firstClass_checkFirstClassFunctions}). The prompt asks the LLM to analyze the file and output 'YES' if first-class functions are used, or 'NO' otherwise, with no explanation.

If the LLM responds with 'NO' (\ref{line:firstClass_checkResponse}), the algorithm continues to the next file. If the response is 'YES', it proceeds to extract information about where functions are passed as arguments (\ref{line:firstClass_findFunctionPasses}).

If the LLM indicates that no function passing occurs (\ref{line:firstClass_noFunctionPasses}), the algorithm moves on to the next file. Otherwise, it parses the response into a list called \texttt{passList}, which contains tuples of function names, receivers, and line numbers where first-class functions are passed (\ref{line:firstClass_parsePasses}).

For each entry in the pass list, the algorithm recursively checks how these passed functions are used by calling the \texttt{FindFunctionUses} function (\ref{line:firstClass_recursiveCall}). This function explores whether the passed function is called or further passed within the receiver function, and it updates the CICFG to reflect these interactions (\ref{line:firstClass_updateCICFGEdge}).

The recursive nature of \texttt{FindFunctionUses} ensures that all uses of first-class functions are thoroughly explored and documented in the CICFG, making sure that the graph accurately reflects all dynamic function interactions across the program (\ref{line:firstClass_recursiveCallInPass}).

% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/fist-class.png}
% 	\caption{first-class function real world example.}
% 	\label{fig:first-class}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=Python, firstnumber=31, caption=first-class function real world example., label=fig:first-class]
def my_map(func, arg_list):
    result = []
    for i in arg_list:
        result.append(func(i))
    return result

# passing square without '()' does not execute it, so it can be executed later
# within my_map() function
squares = my_map(square, [1, 2, 3, 4, 5])
\end{lstlisting}

\noindent\textbf{Usage with example}

As illustrated in Figure~\ref{fig:first-class}, the algorithm processes a Python script where the function `square` is passed as an argument to the `my\_map` function. The algorithm sends the code snippet to an LLM and queries whether first-class functions are utilized within the code. The LLM responds with 'YES', confirming the presence of first-class function usage, where `square` is passed to `my\_map` to apply the `square` operation to each element in a list.

The algorithm then sends another prompt to the LLM, asking it to list all occurrences where functions are passed as arguments, including the function being passed, the function it is passed to, and the line number. The LLM responds by indicating that the function `square` is passed as an argument to `my\_map` at line 10.

Armed with this information, the algorithm initiates a recursive analysis to determine where the `square` function is eventually called. It invokes the \texttt{FindFunctionUses} function with `square` and `my\_map` as parameters. The algorithm sends another prompt to the LLM to ascertain whether `square` is called within `my\_map`. The LLM confirms that `square` is called within `my\_map` at line 5 when `func(i)` is executed.

Utilizing this insight, the algorithm updates the Control and Interprocedural Call Graph (CICFG) by adding an edge from `my\_map` to `square` at line 5. This edge represents the actual function call resulting from the first-class function usage. Additionally, the algorithm recognizes the initial call from the main execution context to `my\_map` at line 10 and updates the CICFG accordingly.

% This example effectively demonstrates how the algorithm leverages responses from an LLM to map and document the use of first-class functions in Python scripts, ensuring the CICFG is comprehensive and accurately captures the control flow involving indirect function calls through function arguments.

% ===================================================================
% Python feature: lambda expressions
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Lambda Expressions Analysis - Python feature}}
\label{algo:lambdaExpressionsAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeLambdaExpressions}{AnalyzeLambdaExpressions}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a Python program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeLambdaExpressions{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:lambda_iterateFiles}
        res $\gets$ \SendToLLM{"Does the given Python code use any lambda expressions? If yes, output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:lambda_checkLambda}
        \If{res == "NO"}{
            \Continue\;\label{line:lambda_noLambda}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"For each lambda expression in the code, define a new function to replace it and provide the callsite of the original lambda expression. Output a list of $<$line number, new function name, new function code$>$. If none, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:lambda_replaceLambda}
            \If{resp == "NO"}{
                \Continue\;\label{line:lambda_noReplacements}
            }
            \Else{
                % lambdaList $\gets$ parse \textit{resp} into list of (\textit{line\_number}, \textit{function\_name}, \textit{function\_code})\;\label{line:lambda_parseLambda}
                \ForEach{(\textit{line\_number}, \textit{func\_name}, \textit{func\_code}) in resp}{\label{line:lambda_processLambdaStart}
                    res $\gets$ \SendToLLM{"Is the function '" + \textit{func\_name} + "' called at line " + \textit{line\_number} + " in the given code? Answer 'YES' or 'NO.' NO explanation." + \textit{file content}}\;\label{line:lambda_checkCall}
                    \If{res == "YES"}{
                        current\_file\_name $\gets$ \textit{file name}\;
                        target\_line\_number $\gets$ line number where \textit{func\_name} is defined\;
                        \UpdateCICFGEdge{current\_file\_name, line\_number, target\_line\_number}\;\label{line:lambda_updateCICFGEdge}
                        is\_updated $\gets$ true\;
                    }
                }\label{line:lambda_processLambdaEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}


\end{algorithm*}


\FloatBarrier
\noindent\textbf{Explanation:}
The algorithm commences by processing each file within the provided set $F$ one at a time (\ref{line:lambda_iterateFiles}). Initially, for each file, a prompt is sent to a Language Model (LLM) to determine whether any lambda expressions are used (\ref{line:lambda_checkLambda}). If the LLM's response is 'NO', the algorithm skips to the next file (\ref{line:lambda_noLambda}).

If 'YES', the algorithm then queries the LLM to provide details on each lambda expression, specifically requesting new function definitions and their call sites to replace these lambdas (\ref{line:lambda_replaceLambda}). This step is essential for transforming lambda expressions into explicit function definitions that can be better analyzed and tracked in the CICFG.

If the response contains no replacements (\ref{line:lambda_noReplacements}), the process proceeds to the next file. Otherwise, the response is parsed into a list of tuples, each containing a line number, the new function's name, and its code (\ref{line:lambda_parseLambda}).

For each lambda replacement, the algorithm checks whether the new function is called at the specified line (\ref{line:lambda_checkCall}). If confirmed, the algorithm updates the CICFG to reflect this call by adding an edge from the calling line to the line where the function is defined (\ref{line:lambda_updateCICFGEdge}), effectively updating the control flow graph to account for the dynamic nature of lambda expressions within the program.

% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/python-lambda.png}
% 	\caption{lambda expression real world example.}
% 	\label{fig:python-lambda}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=Python, firstnumber=308, caption=lambda expression real world example., label=fig:python-lambda]
opt_group.add_argument("--period", type=lambda i: max(abs(int(i)), 1))
\end{lstlisting}

\noindent\textbf{Usage with example}
As illustrated in Figure~\ref{fig:python-lambda}, the algorithm sends this code to an LLM and queries whether lambda expressions are utilized within the code. The LLM responds with 'YES', confirming the presence of a lambda expression.

The algorithm then sends another prompt to the LLM, requesting that it defines a new function to replace the lambda expression and provides the call site (line number) of the original lambda expression. The LLM responds by providing the new function definition and its corresponding call site.

Armed with this information, the algorithm parses the response and recognizes the replacement of the lambda expression with a named function parse\_period. It then confirms with the LLM whether parse\_period is called at line 1 in the code. The LLM responds with 'YES' and identifies that the call occurs within the main execution context.

The algorithm updates the Control and Interprocedural Call Graph (CICFG) by adding an edge from the caller (in this case, the main context or the function where opt\_group.add\_argument is called) to the new function parse\_period at their respective line numbers. This edge represents the function call resulting from replacing the lambda expression.


% ===================================================================
% Python feature: reflection
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Reflection Analysis - Python feature}}
\label{algo:reflectionAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeReflection}{AnalyzeReflection}
\SetKwFunction{FindPossibleFunctions}{FindPossibleFunctions}
\SetKwFunction{FindFunctionCalls}{FindFunctionCalls}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKwFunction{GetCallers}{GetCallers}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a Python program, CICFG}
\KwOut{Updated CICFG}

\Fn{\AnalyzeReflection{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:reflection_iterateFiles}
        res $\gets$ \SendToLLM{"Does the given Python code use reflection or dynamic function calls? If yes, output 'YES'; if not, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:reflection_checkReflection}
        \If{res == "NO"}{
            \Continue\;\label{line:reflection_noReflection}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List all occurrences where reflection is used to retrieve functions, including $<$the variable names used to retrieve the functions, the source of the function names (e.g., variables), the line numbers where the retrieval occurs$>$. If none, output 'NO.' NO explanation." + \textit{file content}}\;\label{line:reflection_findRetrieval}
            \If{resp == "NO"}{
                \Continue\;\label{line:reflection_noOccurrences}
            }
            \Else{
                % retrievalList $\gets$ parse \textit{resp} into list of (\textit{line\_number}, \textit{retrieval\_var}, \textit{func\_name\_var}, \textit{function\_name})\;\label{line:reflection_parseRetrieval}
                \ForEach{(line\_number, retrieval\_var, func\_name\_var, current\_function) in resp}{\label{line:reflection_processRetrievalStart}
                    possibleFuncs $\gets$ \FindPossibleFunctions{\textit{func\_name\_var}, \textit{current\_function}, [\textit{file content}], set()}\;\label{line:reflection_findPossibleFuncs}
                    callSites $\gets$ \FindFunctionCalls{\textit{retrieval\_var}, \textit{current\_function}, [\textit{file content}], set()}\;\label{line:reflection_findFunctionCalls}
                    \ForEach{func\_name in possibleFuncs}{
                        target\_file\_name, target\_line\_number $\gets$ retrieve file name and entry line number of \textit{func\_name} from CICFG\;
                        \ForEach{(caller\_func, call\_line) in callSites}{
                            \UpdateCICFGEdge{caller\_func, call\_line, func\_name, target\_line\_number}\;\label{line:reflection_updateCICFGEdge}
                            is\_updated $\gets$ true\;
                        }
                    }
                }\label{line:reflection_processRetrievalEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}

\Fn{\FindPossibleFunctions{func\_name\_var, current\_function, code, visited\_vars}}{
    \If{(func\_name\_var, current\_function) in visited\_vars}{
        \Return{[]}\;\label{line:reflection_alreadyVisitedFuncs}
    }
    visited\_vars.add((\textit{func\_name\_var}, \textit{current\_function}))\;\label{line:reflection_addVisitedFuncs}
    callers $\gets$ List of (\textit{caller\_function}, \textit{call\_line}) where \textit{function\_name} is called, extracted from CICFG\;\label{line:reflection_getCallers}
    possibleFuncs $\gets$ [\,]\;
    \ForEach{(caller\_func, call\_site) in callers}{
        args $\gets$ \SendToLLM{"In the following code, what arguments are passed to the function '" + \textit{current\_function} + "' at call site line " + \textit{call\_site} + "? Provide the values or variables corresponding to parameter '" + \textit{func\_name\_var} + "'. NO explanation." + \textit{code}}\;\label{line:reflection_getArguments}
        \ForEach{arg in args}{
            \If{arg is a literal or function name}{
                possibleFuncs.append(arg)\;\label{line:reflection_appendFunc}
            }
            \Else{
                possibleFuncs.extend(\FindPossibleFunctions{\textit{arg}, \textit{caller\_func}, \textit{code}, \textit{visited\_vars}})\;\label{line:reflection_recursiveFuncs}
            }
        }
    }
    \Return{possibleFuncs}\;
}

\Fn{\FindFunctionCalls{retrieval\_var, current\_function, code, visited\_vars}}{
    \If{(retrieval\_var, current\_function) in visited\_vars}{
        \Return{[]}\;\label{line:reflection_alreadyVisitedCalls}
    }
    visited\_vars.add((\textit{retrieval\_var}, \textit{current\_function}))\;\label{line:reflection_addVisitedCalls}
    res $\gets$ \SendToLLM{"In the following code, within the function '" + \textit{current\_function} + "', find all locations where the variable '" + \textit{retrieval\_var} + "' is called as a function or passed as an argument to other functions. Provide $<$the function names, line numbers where these calls occur$>$. If none, output 'NO.' NO explanation." + \textit{code}}\;\label{line:reflection_getCallSites}
    \If{res == "NO"}{
        \Return{[]}\;\label{line:reflection_noCalls}
    }
    \Else{
        % callList $\gets$ parse \textit{res} into list of (\textit{caller\_func}, \textit{call\_line})\;\label{line:reflection_parseCalls}
        callList $\gets$ res\;\label{line:reflection_parseCalls}
        \ForEach{(func\_name, line\_number) in callList}{
            callList.extend(\FindFunctionCalls{\textit{func\_name}, \textit{current\_function}, \textit{code}, \textit{visited\_vars}})\;\label{line:reflection_recursiveCalls}
        }
        \Return{callList}\;
    }
}

\end{algorithm*}


\FloatBarrier
\noindent\textbf{Explanation:}
The algorithm begins by processing each file in the set $F$ one at a time (\ref{line:reflection_iterateFiles}). For each file, it first checks whether reflection or dynamic function calls are used by sending a prompt to the LLM (\ref{line:reflection_checkReflection}). If the LLM's response is 'NO', indicating absence of reflection, the algorithm proceeds to the next file (\ref{line:reflection_noReflection}).

If the response is 'YES', the algorithm asks for detailed information about each occurrence where reflection is used to retrieve functions (\ref{line:reflection_findRetrieval}). This includes variables used to retrieve the functions, the sources of the function names, and the line numbers where these retrievals occur.

If the response indicates that there are no occurrences of reflection (\ref{line:reflection_noOccurrences}), the algorithm moves on to the next file. Otherwise, it parses the response into a list detailing each retrieval (\ref{line:reflection_parseRetrieval}).

For each item in the retrieval list, the algorithm first identifies all possible functions that could be dynamically called (\ref{line:reflection_findPossibleFuncs}) and finds all call sites where these functions are potentially invoked (\ref{line:reflection_findFunctionCalls}). It then updates the CICFG to reflect these dynamic interactions, adding edges from the call sites to the defined functions in the graph, ensuring the CICFG accurately reflects the dynamic behavior of the program (\ref{line:reflection_updateCICFGEdge}).

 For each instance, the algorithm determines the possible functions that these variables might refer to using the `FindPossibleFunctions` function. This function iteratively explores all caller functions that might pass arguments that resolve to function names, expanding the search recursively if necessary (\ref{line:reflection_findPossibleFuncs}).


Parallelly, the `FindFunctionCalls` function searches for all sites within the current function's scope where the retrieved functions might be called or passed further. This involves parsing the code to identify all such interactions, ensuring that even nested or indirectly referenced calls are captured (\ref{line:reflection_findFunctionCalls}).

% This methodical approach allows the algorithm to thoroughly analyze and update the CICFG based on reflection usage in Python code, ensuring a comprehensive understanding of the program's dynamic function interactions.


% \begin{figure*}[tp]
% 	\vspace{-0pt}
% 	\includegraphics[width=.95\linewidth]{figure/python-reflection.png}
% 	\caption{reflection real world example.}
% 	\label{fig:python-reflection}
% 	\vspace{-6pt}
% \end{figure*}

\begin{lstlisting}[language=Python, firstnumber=1308, caption=reflection real world example., label=fig:python-reflection]
function = _arithmetic_functions.get(unquote(func), len(args))
if function is None:
    function = extra_functions.get(unquote(func), len(args))
if function is None:
    raise ArithmeticError("Unknown function '%s/%s'" % (func, len(args)))

try:
    values = [arg.compute_value(extra_functions) for arg in args]
    if None in values:
        return None
    else:
        return function(*values)
\end{lstlisting}

\noindent\textbf{Usage with example}
As shown in Figure~\ref{fig:python-reflection}, the algorithm processes a Python script that utilizes reflection to dynamically retrieve and invoke functions. The code snippet includes a function `compute\_function` that takes a function name `func` and arguments `args`, using reflection to obtain the corresponding function from dictionaries like `\_arithmetic\_functions` or `extra\_functions`. If the function is found, it is called with the provided arguments.

The algorithm sends the code snippet to an LLM and queries whether reflection or dynamic function calls are utilized within the code. The LLM responds with 'YES', confirming the presence of reflection usage where functions are dynamically retrieved and invoked based on variable inputs.

The algorithm then sends another prompt to the LLM, asking it to list all occurrences where reflection is used to call functions, identifying the variable names involved, possible function names that could be called, and the line numbers where these calls occur. The LLM responds by detailing that within `compute\_function, the variable `function` retrieves functions from `\_arithmetic\_functions` and `extra\_functions` using `func` at lines 1308 and 1310. It notes that `function` is called with `*values` at line 1318.

Armed with this information, the algorithm parses the response and recognizes the dynamic retrieval and invocation of functions via reflection. It analyzes the callers of `compute\_function` to determine the possible values of `func`, thereby identifying the potential functions that could be called. The algorithm updates the Control and Interprocedural Call Graph (CICFG) by adding edges from `compute\_function` to all possible target functions that `func` could reference, accurately reflecting the dynamic control flow introduced by reflection.


% ===================================================================
% Python feature: dynamic import
\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Dynamic Imports Analysis - Python feature}}
\label{algo:dynamicImportsAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeDynamicImports}{AnalyzeDynamicImports}
\SetKwFunction{FindDynamicImports}{FindDynamicImports}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{Set of files $F$ from a Python program}
\KwOut{Updated CICFG}

\Fn{\AnalyzeDynamicImports{F}}{
    start\_file $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{file in $F$}{\label{line:dynamic_imports_iterateFiles}
        res $\gets$ \SendToLLM{"Does the given Python code use dynamic imports? If yes, output 'YES'; if not, output 'NO.' NO explanation." + file content}\;\label{line:dynamic_imports_checkDynamicImports}
        \If{res == "NO"}{
            \Continue\;\label{line:dynamic_imports_noDynamicImports}
        }
        \Else{
            start\_file.append(file)\;
            resp $\gets$ \SendToLLM{"List all modules or functions that are imported dynamically in the code. Output a list of $<$module or function names$>$. If none, output 'NO.' NO explanation.\textbackslash n" + file content}\;\label{line:dynamic_imports_listModules}
            \If{resp == "NO"}{
                \Continue\;\label{line:dynamic_imports_noModules}
            }
            \Else{
                % moduleList $\gets$ parse resp into list of module or function names\;\label{line:dynamic_imports_parseModules}
                \ForEach{module\_name in resp}{\label{line:dynamic_imports_processModulesStart}
                    \FindDynamicImports{module\_name, file, set()}\;\label{line:dynamic_imports_recursiveCall}
                }\label{line:dynamic_imports_processModulesEnd}
            }
        }
    }
    \Return{start\_file, is\_updated}\;
}

\Fn{\FindDynamicImports{module\_name, file name, visited\_modules}}{
    code $\gets$ get the code in the \textit{file name}\ from CICFG;
    \If{module\_name in visited\_modules}{
        \Return\;\label{line:dynamic_imports_alreadyVisited}
    }
    visited\_modules.add(module\_name)\;\label{line:dynamic_imports_addVisited}
    res $\gets$ \SendToLLM{"In the following code, is the module or function '" + module\_name + "' used? If yes, provide the line numbers where it is used. If not, is it passed as an argument to other functions? If so, provide the function names and line numbers where this occurs. If neither, output 'NO.' NO explanation.\textbackslash n" + code}\;\label{line:dynamic_imports_checkUsage}
    \If{res == "NO"}{
        \Return\;\label{line:dynamic_imports_noUsage}
    }
    \Else{
        \If{module\_name is a function name \textnormal{\textbf{and}} module\_name is used in code}{
            usageLines $\gets$ parse the list of line numbers where \textit{module\_name} is used from res\;\label{line:dynamic_imports_getUsageLines}
            \ForEach{line\_number in usageLines}{
                statement $\gets$ get the statement in \textit{file name} at \textit{line\_number}\;
                \UpdateCICFGNode{file name, line\_number, statement}\;\label{line:dynamic_imports_updateNode}
                \UpdateCICFGEdge{file name, line\_number, file name, line\_number}\;\label{line:dynamic_imports_updateEdge}
                is\_updated $\gets$ true\;
            }
        }
        \If{module\_name is passed as argument in code}{
            passList $\gets$ parse the list of (receiver\_function, line\_number) where \textit{module\_name} is passed from res\;\label{line:dynamic_imports_getPassList}
            \ForEach{(receiver\_function, line\_number) in passList}{
                receiver\_file $\gets$ retrieve the file name of \textit{receiver\_function} from CICFG\;
                \FindDynamicImports{module\_name, receiver\_file, visited\_modules}\;\label{line:dynamic_imports_recursiveCallInPass}
            }
        }
    }
}


\end{algorithm*}


\noindent\textbf{Explanation:}
The algorithm begins by iterating over each file in the set $F$ from a Python program (line~\ref{line:dynamic_imports_iterateFiles}). For each file, it checks whether dynamic imports are used by sending a prompt to the LLM (line~\ref{line:dynamic_imports_checkDynamicImports}). The prompt asks the LLM to analyze the file and output 'YES' if dynamic imports are used or 'NO' otherwise, with no explanation.

If the LLM responds with 'NO' (line~\ref{line:dynamic_imports_noDynamicImports}), the algorithm continues to the next file. If the response is 'YES', it proceeds to list all modules or functions that are imported dynamically in the code by sending another prompt to the LLM (line~\ref{line:dynamic_imports_listModules}). If the LLM responds with 'NO' (line~\ref{line:dynamic_imports_noModules}), indicating no dynamically imported modules or functions, the algorithm moves on to the next file.

Otherwise, the response is parsed into a list called \texttt{moduleList}, which contains the names of the modules or functions imported dynamically (line~\ref{line:dynamic_imports_parseModules}). For each module or function in this list (line~\ref{line:dynamic_imports_processModulesStart}), the algorithm calls the \texttt{FindDynamicImports} function to analyze how these modules or functions are used in the code (line~\ref{line:dynamic_imports_recursiveCall}).

In the \texttt{FindDynamicImports} function, the algorithm first retrieves the code of the given file from the CICFG. It checks if the current module or function has already been visited to prevent redundant analysis (lines~\ref{line:dynamic_imports_alreadyVisited} and \ref{line:dynamic_imports_addVisited}). Then, it sends a prompt to the LLM to determine if the module or function is used in the code, and if so, it asks for the line numbers where it is used or passed as an argument to other functions (line~\ref{line:dynamic_imports_checkUsage}).

If the LLM responds with 'NO' (line~\ref{line:dynamic_imports_noUsage}), the function returns without further action. Otherwise, the algorithm processes the response to handle different cases:

\begin{itemize}
    

\item  Module or Function Usage:

   - If the module or function is a function name and is used in the code, the algorithm parses the list of line numbers where it is used (line~\ref{line:dynamic_imports_getUsageLines}).
   
   - For each line number, it retrieves the statement from the code and updates the CICFG by adding a node representing the usage (line~\ref{line:dynamic_imports_updateNode}) and an edge to represent the control flow (line~\ref{line:dynamic_imports_updateEdge}).

\item Module or Function Passed as Argument:

   - If the module or function is passed as an argument in the code, the algorithm parses the list of receiver functions and line numbers where this occurs (line~\ref{line:dynamic_imports_getPassList}).
   
   - For each receiver function, it retrieves the file name from the CICFG and recursively calls \texttt{FindDynamicImports} to analyze how the module or function is used within the receiver function (line~\ref{line:dynamic_imports_recursiveCallInPass}).
\end{itemize}

\begin{lstlisting}[language=Python, firstnumber=59, caption=dynamic import real world example., label=fig:dynamicimport]
net_class = getattr(__import__('networks'), args.network)
net = net_class(args.modalities, n_class).to(device)
net.init_weights()
\end{lstlisting}

\noindent\textbf{Usage with example} As shown in figure~\ref{fig:dynamicimport}, the algorithm processes a Python script that utilizes dynamic imports to load modules and classes at runtime. Specifically, the code dynamically imports the 'networks' module using the \_\_import\_\_ function and retrieves a class based on the value of \texttt{args.network} using \texttt{getattr}. This class is then instantiated with the provided arguments and used to create a neural network model.

The algorithm sends the code snippet to an LLM and queries whether dynamic imports are utilized within the code. The LLM responds with 'YES', confirming the presence of dynamic import patterns in the script.

The algorithm then sends another prompt to the LLM, asking it to list all modules or functions that are imported dynamically in the code. The LLM responds by identifying that the module \texttt{'networks'} and the class specified by \texttt{args.network} are imported dynamically. It provides the line numbers where these dynamic imports occur: the import of \texttt{'networks'} at line 59 and the retrieval of \texttt{net\_class} at the same line.

Armed with this information, the algorithm invokes the \texttt{FindDynamicImports} function to analyze the usage of the dynamically imported module and function. It parses the response and recognizes the dynamic loading of the \texttt{'networks'} module and the function \texttt{net\_class}. The algorithm updates the CICFG by adding nodes representing the dynamically imported module and function, as well as edges capturing their instantiation and method calls within the code.


\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Source/Sink Identification}}
\label{algo:sourceSinkAnalysis_noPropagation}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeSourcesSinks}{AnalyzeSourcesSinks}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{List of $F$ files of a program}
\KwOut{Records of identified sources and sinks (file, function, var/func name, line number)}

\Fn{\AnalyzeSourcesSinks{F}}{
    sourceRecords $\gets$ empty list\;\label{line:noProp_initSources}
    sinkRecords $\gets$ empty list\;\label{line:noProp_initSinks}

    \ForEach{fil in $F$}{\label{line:noProp_iterateFiles}
        funcs $\gets$ list of functions in fil\;\label{line:noProp_extractFuncs}
        \ForEach{func in funcs}{\label{line:noProp_iterateFuncs}

            \tcp{First LLM call for sources}
            srcRes $\gets$ \SendToLLM{"Given the code of function '" + func.name + "', identify all taint sources (This could be user inputs, files, network interfaces, or any external data source that interacts with the program). If none, output 'NO.' NO explanation.\textbackslash n" + func code}\;\label{line:noProp_checkSources}
            \If{srcRes != "NO"}{
                sources $\gets$ parse srcRes into list of (srcVarOrFunc, lineNumber)\;\label{line:noProp_parseSources}
                \ForEach{(srcName, srcLine) in sources}{
                    sourceRecords.append((fil, func.name, srcName, srcLine))\;\label{line:noProp_recordSource}
                }
            }

            \tcp{Second LLM call for sinks}
            sinkRes $\gets$ \SendToLLM{"Given the code of function '" + func.name + "', identify all taint sinks (This could be database queries, file operations, or network transmissions, etc.). If none, output 'NO.' NO explanation.\textbackslash n" + func code}\;\label{line:noProp_checkSinks}
            \If{sinkRes != "NO"}{
                sinks $\gets$ parse sinkRes into list of (sinkVarOrFunc, lineNumber)\;\label{line:noProp_parseSinks}
                \ForEach{(sinkName, sinkLine) in sinks}{
                    sinkRecords.append((fil, func.name, sinkName, sinkLine))\;\label{line:noProp_recordSink}
                }
            }
        }
    }

    \Return{(sourceRecords, sinkRecords)}\;\label{line:noProp_return}
}


\end{algorithm*}


\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Phase 1 Feature Controller}}
\label{algo:unifiedFeatureAnalysisSimplified}
\SetKwProg{Fn}{Function}{}{end}

\SetKwFunction{WalkDirectory}{WalkDirectory}

\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered

\KwIn{A project directory path $proj\_path$}
\KwOut{Analysis results of various features}

% c\_features $\gets$ ["function pointer", "conditional compilation", "external function", "inline assembly", "macro", "goto", "setjmp"]\;
% py\_features $\gets$ ["dynamic typing", "decorator", "first-class functions", "lambda", "reflection", "dynamic imports"]\;
all\_features $\gets$ c\_features + py\_features\;

% Instead of hardcoding, we assume a function that returns the related features.
feature\_related\_mapping $\gets$ get\_featuremapping()\; \tcp{get\_featuremapping() returns a dictionary mapping each feature to a list of related features that should be updated if this feature is updated.}

% feature\_handler\_mapping = {
%     "function pointer": AnalyzeFunctionPointers,
%     "conditional compilation": AnalyzeDynamicLinking,
%     "external function": AnalyzeConditionalCompilation,
%     "inline assembly": AnalyzeInline,
%     "macro": AnalyzeMacro,
%     "goto": AnalyzeGoto,
%     "setjmp": AnalyzeSetjmp,
%     "dynamic typing": AnalyzeDynamicTyping,
%     "decorator": AnalyzeDecorators,
%     "first-class functions": AnalyzeFirstClassFunctions,
%     "lambda": AnalyzeLambda,
%     "reflection": AnalyzeReflection,
%     "dynamic imports": AnalyzeDynamicImport
% }\;

startfile\_dict $\gets$ empty dictionary\;
worklist $\gets$ empty set\;

\ForEach{feat in all\_features}{
    startfile $\gets$ []\;

    analyzeFunc $\gets$ feature\_handler\_mapping[feat]\;

    \ForEach{file\_path in \WalkDirectory(proj\_path)}{
        (startf, \_) $\gets$ analyzeFunc(file\_path)\;
        startfile.extend(startf)\;
    }

    startfile\_dict[feat] = startfile\;
    \If{startfile != []}{
        worklist = worklist $\cup$ feature\_related\_mapping[feat]\;
    }
}

\While{worklist \texttt{ not empty}}{
    feat $\gets$ worklist.pop() \tcp{get an element and remove it from worklist }\;
    startfile $\gets$ startfile\_dict(feat)\;

    analyzeFunc $\gets$ feature\_handler\_mapping[feat]\;

    is\_updated $\gets$ False\;
    \ForEach{file\_path in startfile}{
        (\_, updated) $\gets$ analyzeFunc(file\_path)\;
        \If{updated == True}{
            is\_updated $\gets$ True
        }
    }

    \If{is\_updated}{
        worklist = worklist $\cup$ feature\_related\_mapping[feature]\;
    }
}
\end{algorithm*}




% \setlength{\textfloatsep}{0pt}
% \begin{algorithm*}[tp]
% \caption{\footnotesize{LLM-Assisted Taint Analysis}} 
% \label{algo:taintAnalysisLLMUnified}
% \SetKwProg{Fn}{Function}{}{end}
% \SetKwFunction{SendToLLM}{SendToLLM}
% \SetKwFunction{CheckReachability}{CheckReachability}
% \SetKwFunction{BuildSlice}{BuildSlice}
% \SetKwFunction{GetSubgraphFunctions}{GetSubgraphFunctions}
% \SetKwFunction{GetCallsites}{GetCallsites}
% \SetKwFunction{ReportTaintFlowPath}{ReportTaintFlowPath}
% \SetKwFunction{CheckCrossLanguage}{CheckCrossLanguage}
% \SetKw{Continue}{continue}
% \SetKw{Return}{return}
% \LinesNumbered

% \KwIn{Set of identified source/sink pairs (from previous source/sink identification step); A phase1-augmented CICFG}
% \KwOut{Taint flow paths and recorded taint analysis results (no ShowCodeToLLM, AskLLMForUnfamiliar, AskLLMForFacts, all use SendToLLM)}

% \Fn{\textnormal{TaintAnalysisWithLLM}(sourceSinkPairs, CICFG)}{
%     availablePairs $\gets$ []\;
%     \ForEach{(src, sink) in sourceSinkPairs}{
%         \If{\CheckReachability{src, sink, CICFG} == True}{
%             availablePairs.append((src, sink))\;
%         }
%     }

%     \ForEach{(src, sink) in availablePairs}{
%         subgraph $\gets$ \BuildSlice{CICFG, src, sink}\; 
%         functionsInSubgraph $\gets$ \GetSubgraphFunctions{subgraph}\;

%         visitedFuncs $\gets$ empty set\;
%         taintFacts $\gets$ empty data structure\; 
%         taintedVars $\gets$ set of vars related to src\;

%         stack $\gets$ [function containing src]\;

%         \While{stack not empty}{
%             currentFunc $\gets$ stack.pop()\;
%             \If{currentFunc in visitedFuncs}{
%                 \Continue
%             }
%             visitedFuncs.add(currentFunc)\;

%             codeSnippet $\gets$ code of currentFunc from subgraph\;
%             promptCode = "Here's the code:\n" + codeSnippet + "\nTainted vars:" + taintedVars + "\nSource:" + src

%             LLMResUnfamiliar $\gets$ \SendToLLM{promptCode + "\nList any functions in this snippet you do not know about. If none, output 'NO.'"}\; 

%             unfamiliarFuncs $\gets$ parse LLMResUnfamiliar into a list of unfamiliar functions\;
%             \If{unfamiliarFuncs != "NO"}{
%                 extraCode $\gets$ retrieve code of unfamiliarFuncs from subgraph or code database\;
%                 promptCode = promptCode + "\nExtra code:\n" + extraCode
%             }

%             LLMResFacts $\gets$ \SendToLLM{promptCode + "\nGiven this code and tainted vars, provide alias/data-flow relationships, then which vars get tainted.\n"}\;

%             aliasAndDataflowFacts $\gets$ parse LLMResFacts\;
%             \tcp{Update taintFacts and taintedVars based on aliasAndDataflowFacts}
%             update taintFacts and taintedVars accordingly\;

%             \If{sink in currentFunc and taintedVars lead to sink}{
%                 pathInfo $\gets$ gather info from taintFacts and subgraph\;
%                 \ReportTaintFlowPath{pathInfo}\;
%                 \If{\CheckCrossLanguage{src, sink}}{
%                     print("Cross-language vulnerability found")\;
%                 }
%                 \Continue
%             }

%             callsites $\gets$ \GetCallsites{currentFunc, subgraph}\; 
%             \ForEach{(calleeFunc, callLine, passedVars) in callsites}{
%                 \If{passedVars ∩ taintedVars not empty}{
%                     stack.push(calleeFunc)\;
%                 }
%             }
%         }
%     }
% }

% \end{algorithm*}


\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{LLM-Assisted Taint Analysis with Feature Handlers}}
\label{algo:llmTaintAnalysisFeatures}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{BuildSlice}{BuildSlice}
\SetKwFunction{GetSubgraphFunctions}{GetSubgraphFunctions}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{GetFeatureHandlers}{GetFeatureHandlers}
\SetKwFunction{AnalyzeFunctionWithFeature}{AnalyzeFunctionWithFeature}
\SetKwFunction{GetNextFunctionAndArgs}{GetNextFunctionAndArgs}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered

\KwIn{Set of available source/sink pairs, CICFG}
\KwOut{Taint analysis results with updated tainted variables per function}

\ForEach{(src, sink)}{
    subgraph $\gets$ \BuildSlice{CICFG, src, sink}\; 
    functionsInSubgraph $\gets$ \GetSubgraphFunctions{subgraph}\;

    taintedVars $\gets$ set of variables related to src initially tainted\;
    features $\gets$ \GetFeatureHandlers()\; \tcp{Array of feature handlers for implicit data flow, etc.}

    \ForEach{currentFunc in functionsInSubgraph}{
        \tcp{First, use feature handlers to update taintedVars}
        \ForEach{feature in features}{
            newTaintedVarsFromFeature $\gets$ \AnalyzeFunctionWithFeature{feature, currentFunc, taintedVars}\;
            taintedVars = taintedVars $\cup$  newTaintedVarsFromFeature\;
        }

        \tcp{Now ask LLM for additional taint info}
        codeSnippet $\gets$ code of currentFunc from subgraph\;
        promptCode = "Given this function code and current tainted vars, list all tainted vars in this function." + codeSnippet + "Tainted vars:" + taintedVars\;
        llmResTaint $\gets$ \SendToLLM{promptCode}\;
        newTaintedFromLLM $\gets$ parse llmResTaint into a set of tainted variables\;
        taintedVars = taintedVars $\cup$ newTaintedFromLLM\;

        \tcp{Before moving to the next function, determine if tainted vars pass to next function}
        (nextFunc, passedTaintedVars) $\gets$ \GetNextFunctionAndArgs{currentFunc, subgraph, taintedVars}\;
        \If{nextFunc == NULL}{
            \tcp{No further taint propagation to next function} 
            \tcp{End the loop for this subgraph}
            \BREAK
            
        }
        \Else{
            taintedVars = passedTaintedVars \tcp{Update taintedVars for next function context}
        }
    }
}

\end{algorithm*}

\setlength{\textfloatsep}{0pt}
\begin{algorithm*}[tp]
\caption{\footnotesize{Dynamic Reflection and Code Execution Feature Handler}}
\label{algo:dynamicReflectionHandler}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{AnalyzeDynamicReflection}{AnalyzeDynamicReflection}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered

\Fn{\AnalyzeDynamicReflection{currentFunc, taintedVars}}{
    codeSnippet $\gets$ code of currentFunc\;

    \tcp{First, ask LLM if there's Dynamic Reflection and Code Execution implicit data flow}
    res $\gets$ \SendToLLM{"Given the following function code, does it involve Dynamic Reflection and Code Execution leading to implicit data flow? If yes, output 'YES'; if not, output 'NO.' NO explanation.\textbackslash n" + codeSnippet}\;

    \If{res == "NO"}{
        \Return{[]} \tcp{No additional tainted vars from this feature}
    }

    \tcp{If YES, we have a known exemplar code to help LLM understand}
    exemplarCode $\gets$ Exemplar of Dynamic Reflection and Code Execution example\; \tcp{This code shows how reflection might load and execute code from external sources.The LLM should consider similar patterns in the given code.}

    prompt = "In the function below, considering the variable set currently tainted: " + taintedVars + "\textbackslash n" +
             "please list all variables that become tainted due to the 'Dynamic Reflection and Code Execution' feature.\textbackslash n" + "The function code:"
              + codeSnippet + "\textbackslash n" + "exemplar:" + exemplarCode + "\textbackslash n"

    llmResTaint $\gets$ \SendToLLM{prompt}\;

    newTaintedFromFeature $\gets$ parse llmResTaint into a list of tainted variables\;

    \Return{newTaintedFromFeature}\;
}

\end{algorithm*}


==> Sections/03_technique-cai.tex <==
\section{Technique}\label{sec:technique}
This section describes our technical approach via the design of {\tech}. %, for analyzing cross-language programs and detecting potential vulnerabilities. 
We begin with an overview of the framework (§\ref{overview}) and then detail its two key phases: augmented control-flow analysis (§\ref{phase 1}) and feature-oriented data-flow reasoning (§\ref{phase 2}). These phases work in tandem to systematically uncover cross-language information flows in \textit{the entire repository} of a given multi-language project, including those induced by the challenging language features. 
%that might otherwise evade traditional static analyses, particularly in complex multi-language settings.

\subsection{Approach Overview}\label{overview}
%{\tech} is designed to systematically identify potential vulnerabilities in Python–C programs by combining static and language-feature-oriented analyses. 
As illustrated in Figure~\ref{fig:overview}, the framework accepts two main \textbf{inputs}: the target multilingual program (project repository) %source code 
and user-specified lists of information sources and sinks. 
%These inputs feed into two major phases that work in tandem to uncover data-flow paths potentially overlooked by traditional static approaches.
Optionally, an LLM-based assisting component can be used to automatically extract sources/sinks from the project to replace or expand those lists. 
With these inputs, {\tech} works like a conventional static data flow analyzer at high level, 
starting with control flow analysis in \textbf{Phase 1}, followed by data flow analysis in \textbf{Phase 2}, 
both assisted by multiple LLMs collaborating via negotiation and arbitration (i.e., LLM-based {\em Expert Panel}). 

Specifically, \textbf{Phase 1} %, we construct the CICFG of the given system which integrates its Python and C components. Starting from a basic control-flow structure, we iteratively augment the CICFG to capture diverse features of each language, including decorators in Python and pointer manipulations in C. 
performs %intraprocedural and then interprocedural 
control flow analyses within and across the two languages, hence constructing the basic \textit{cross-language interprocedural control flow graph} (\ul{CICFG}) 
in Step \textbf{1.1}.   
It then leverages the expert panel to augment the CICFG via a fixed-point iteration of handling the targeted language features in Step \textbf{1.2}. 
This augmentation enriches the graph with additional edges and nodes, resulting in the \textit{augmented CICFG}. 
%ensuring that subtle control-flow behaviors---often missed in conventional analysis—--are as completely represented as possible. 
The goal of this phase is to lay the basis for the data flow tracking in the next phase, which typically works on a control flow representation. 
The rationale is that via the augmentation the representation (CICFG) may capture subtle control-flow behaviors---often missed in conventional analysis—--as completely 
as possible by leveraging the capabilities of LLMs. 

Based on this augmented CICFG, \textbf{Phase 2} aims to first narrow down the data flow analysis scope via directed taint approximation---approximating 
the taint flow with mere control flow starting from any source and exploring the CICFG as directed towards any sink (Step \textbf{2.1}). 
The rationale is that the resulting control-flow paths between the sources/sinks form a focused roadmap for the LLMs to reason about data flow as a much simplified task. 
Then, the approximation is refined through an instructed taint refinement step (\textbf{2.2}), by carefully instructing the expert panel to propagate data flow along 
the source-sink reachable control-flow paths one function at a time. 
During the propagation, {\tech} maintains accumulated tainted data and coordinates the interprocedural and inter-language context, while dealing with 
challenging language features (that induce implicit data flows) via feature-specific few-shot prompting the LLMs. 
The rationale is to minimize the LLMs' task complexities hence reducing their hallucination and maximizing their accuracy. 

%The \textbf{Phase 2} revolves around feature-oriented data-flow reasoning. Initially, we perform a directed taint approximation by extracting reachability-based subgraphs for each source–sink pair, forming a preliminary mapping of how external inputs can propagate through the program. We then refine these results through an instructed taint refinement step, which leverages language-specific insights and external function semantics to yield a more precise view of how sensitive data may traverse function and language boundaries. 
As a result, {\tech} produces a consolidated list of cross-language taint flow paths that may present security risks to be confirmed, as the framework \textbf{outputs}. 
%offering a bad for further validation or mitigation measures.

\subsection{Automated Source/Sink Identification}
Typically, a static information flow analysis takes \textit{user-specified} sources/sinks hence using each source-sink pair as a query. 
While there may be sources/sinks (e.g., common/standard language SDK APIs) to identify manually, 
it can be a daunting task for users to systematically do so for a given/arbitrary project, especially multi-language ones which involve multiple languages. 

Thus, to facilitate its practical use, {\tech} comes with an assisting component to automatically extract sources/sinks from the given multilingual project repository. 
Leveraging the expert panel, it instructs the LLMs to achieve the task using two carefully design prompt templates (as found in our artifact package). The source identification prompt guides the LLM to recognize functions or variables that introduce external or sensitive data into the system, such as user inputs, file reads, or network requests. The sink identification prompt directs the LLM to pinpoint function calls or other operations that can potentially leak data, such as logging, file/network writes. These prompts are structured to provide the LLM with sufficient context about the codebase, enabling it to make informed decisions by leveraging the LLM's understanding of code semantics and common API patterns. 
Unlike a recent tool designed for Java~\cite{li2025iris}, we do not take specific vulnerability types and their descriptions as part of the prompt, which 
restricts the analysis to only those types of bugs. 

%Before constructing the CICFG and performing feature-oriented taint analysis, {\tech} carries out a pre-analysis step to identify and label potential external input points (sources) and critical output functions (sinks). This preliminary phase has two primary objectives. First, it automatically explores the program codebase to discover candidate sources and sinks through LLM queries. Second, the user may also provide a custom list of source/sink definitions, either to account for domain-specific APIs or to refine and override automatic expert panel (LLM-driven analysis, detailed in §~\ref{expert panel}) detections in cases where proprietary or unusual functions exist. {\tech} merges these user inputs with the set of sources and sinks obtained from automatic source-sink identification, ensuring that no critical entry or exit point is overlooked. With a unified source-sink register thus established, we transition to building the augmented CICFG (see §~\ref{phase 1.2}), where these marked entry and exit nodes guide the static and feature-based analyses that follow.

\subsection{LLM-based Expert Panel}\label{expert panel}
To enhance the robustness and cost-effectiveness of our analyses, we propose an expert panel method combining the strengths of non-reasoning (generative) and reasoning LLMs. Non-reasoning LLMs are computationally efficient but prone to instability and hallucination. Conversely, reasoning LLMs provide greater stability and accuracy but at higher computational costs.

Our expert panel employs cross-validation using two non-reasoning models for initial analysis. When disagreements arise between them, a reasoning model is then invoked as an arbiter. This combined approach capitalizes on the efficiency of non-reasoning models for most tasks, reserving the resource-intensive reasoning model for ambiguous or complex cases, thereby achieving an optimal balance between accuracy, stability, and computational expense.

\subsection{Augmented Control-Flow Analysis}\label{phase 1}
%A program analysis is often based on a program representation, such as the control flow graph (CFG). By default, CFG is intraprocedural, representing control flow within a function. For interprocedural analysis, per-function CFGs are linked together through calling relationships between the functions, forming an interprocedural CFG (or ICFG). To enable holistic static analysis of multi-language software, a multilingual code representation is also needed, for which further link per-language ICFGs through control flow induced by cross-language functions. We refer to this representation the \textbf{cross-language interprocedural control flow graph (CICFG)}. Thus, a CICFG node represents a statement in a multilingual program, while a CICFG edge represents control flow between two nodes within and across the languages.

{\tech} constructs and refines a CICFG that spans both Python and C code. This graph provides the foundational structure for identifying taint flows in multi-language programs. We first describe how the basic CICFG is built (§~\ref{phase 1.1}), and then show how we augment this initial graph with language-specific features (§~\ref{phase 1.2}), ensuring that subtle cross-language behaviors are not lost during static analysis.


\subsubsection{CICFG Construction}\label{phase 1.1}
The lack of a ready-made, whole-program static information flow analysis tool for real-world Python–C programs motivates us to adapt existing infrastructure to our needs. We start from producing a cross-language, interprocedural control-flow graph for each analyzed project. Following established practices in ICFG construction~\cite{sinha01apr}, every node in the resulting CICFG corresponds to a statement or operation in either language's portions of the codebase, and directed edges indicate the potential transfer of control. 
%Thus, a CICFG node represents a statement in a multilingual program, while a CICFG edge represents control flow between two nodes within and across the languages.

The construction proceeds by first extracting intraprocedural control-flow graphs for each function or method in the target Python and C files. Next, these per-method graphs are connected into an intra-language call graph, one for each language unit. We then identify cross-language call edges by examining how the two languages (e.g., Python and C) components interact, guided by FFI specifications (e.g., Python C APIs). For instance, if a C extension module provides a function accessible from Python, that interface call is represented in the graph as an inter-language edge. Finally, we merge the two intra-language call graphs, along with these cross-language edges, to form the CICFG. Each node is annotated with contextual information, such as the function name and the source-code location, facilitating later traversal of the graph. 


\subsubsection{CICFG Augmentation}\label{phase 1.2}


 While the initial CICFG captures control-flow connections at the function and statement levels, cross-language programs commonly employ various features that can introduce implicit or hidden control flows. Python’s decorator, reflection, and import mechanisms, along with C’s macros, function pointers, and conditional compilation, often cause static analyses to miss relevant control paths if these features are not explicitly accounted for. To address these complexities, {\tech} augments the CICFG in an iterative process that enriches the control-flow representation with additional edges and annotations corresponding to such features.

Initially, we scan the project for a range of language features using specialized handler functions; for example, we detect macros and function pointers in C source files, and decorators or dynamic imports in Python. When a handler discovers any such feature in a file, it marks that file as needing further analysis and adds it to a global worklist. Features that are closely related---for example, macros and conditional compilation---trigger updates to each other’s state so that modifications to one construct can be properly reflected in another. The algorithm then proceeds in a fixed-point manner: if re-analysis of certain files detects new features or modifies existing ones, the corresponding handlers are re-invoked until no further updates are generated, as detailed in Algorithm~\ref{lab:appendix} in Appendix~\ref{sec:phase1algo}.


By iterating through potentially interactive or mutually dependent language constructs, we ensure that the final CICFG does not omit control-flow edges that arise from dynamic or conditional behaviors. Nodes that might otherwise appear disconnected become properly linked, and call edges that are only valid under specific macros or function pointer assignments are accurately reflected. The end result is an augmented CICFG in which language features that would typically frustrate purely static approaches are consistently incorporated, providing a robust foundation for our subsequent data-flow analysis.

% \subsubsection{Feature Handling} \label{sec:feature-handling}
%
% % CICFG augmentation relies on systematically handling language-specific features, which may introduce subtle or dynamic control-flow paths. In this subsection, we illustrate this feature handling approach by detailing our method for analyzing function pointers in C, an inherently dynamic construct often challenging for static analyses.
% Before initiating taint propagation, {\tech} performs a critical pre-analysis step to account for implicit data flows caused by advanced language features. 
% Constructs such as reflection in Python or function pointer in C can create data-flow paths invisible to standard syntactic analysis. 
% To capture these, {\tech} leverages its expert panel to identify the presence of such features within a function and to infer how they implicitly propagate data between variables. 
% The resulting information is used to augment the initial CICFG by adding edges and nodes representing the previously implicit flows. 
% The detailed implementation and logic for each feature handler are provided in our supplementary artifact.

\textbf{Feature Handling}.
For each of our targeted features ($\S$\ref{sec:bkgmotive}), {\tt analyzeFunc} represents the specific handler for that feature. 
In this handler, {\tech} traverses all the feature presence units (FPUs) one at a time, which defines the minimal scope where the feature could be resolved. 
For most of the features we target, an FPU is a function; yet for some features, it is a source file. 
When processing each FPU, {\tech} leverages the expert panel to first (1) detect the presence of the feature, followed by 
(2) identifying the missing nodes and/or edges (Table~\ref{tab:motivation-study}), and (3) when identified, it adds the nodes/edges to the CICFG accordingly. 
While for different features, the handling logic varies, the handler (including for additional features) always follows these three main steps. 
For space limit, we have provided the detailed algorithm pseudocode and explanations for each of the 12 feature handlers in our artifact package. 
Appendix~\ref{sec:featurehandlingalgos-c} and Appendix~\ref{sec:featurehandlingalgos-python} provide an example of such feature handling algorithms for C and Python, respectively. 

\subsection{Feature-Oriented Data Flow Reasoning}\label{phase 2}
Having constructed and augmented the CICFG, we next turn to detecting and refining taint flows that may traverse multiple language boundaries in the presence of complex language features. {\tech} orchestrates this phase in two distinct steps: a directed taint approximation stage (§~\ref{phase 2.1}) that enumerates candidate flows from sources to sinks, and an instructed refinement stage (§~\ref{phase 2.2}) that uses feature knowledge and LLM-assisted context to prune or expand these flows as necessary. The final result is a set of potential vulnerabilities, each represented by a path from source to sink across the augmented control-flow graph.

\subsubsection{Directed Taint Approximation}\label{phase 2.1}
The first step of our data-flow reasoning phase applies a control-flow-reachability-based analysis on top of the augmented CICFG. We either use the user-specified source/sink lists or begin by collecting pairs of taint sources and sinks. For each such pair 
⟨\textit{src},\textit{sink}⟩, we slice the augmented CICFG to extract the subgraph of control-flow nodes lying on the possible paths from \textit{src} to \textit{sink}. This subgraph (or control-flow slice) reflects an initial mapping of how data originating from \textit{src} could propagate through both Python and C components until reaching \textit{sink}.

We then aggregate these paths at purely-control-flow level, a process that highlights the subsets of code relevant to each source-sink traversal. By operating on control-level approximation, we significantly reduce the complexity of our subsequent detailed analysis, since we can focus our refinement only on the control flow paths that are flagged as potentially hosting sensitive data flow. Once this reachability-based approximation is complete, the result is a set of candidate paths for each ⟨\textit{src},\textit{sink}⟩ pair, awaiting further scrutiny in the next step.

\subsubsection{Instructed Taint Refinement}\label{phase 2.2}
After gathering all candidate paths, we refine them through a deeper inspection that leverages both static feature handlers and LLM-assisted analyses. For every subgraph derived from the source–sink pairs, we traverse its constituent functions one by one, carrying along a set of tainted variables (initially those introduced at the source).
At each function, we invoke specialized handlers designed to account for language-specific constructs, such as value transfer via pointer indirection in C. These handlers systematically update the set of tainted variables, capturing implicit or indirect data flows that might be missed by purely syntactic analysis. Once the feature handlers have run, we engage the expert panel to confirm or further extend the taint set. The prompt sent to the expert panel encapsulates the current function’s code snippet and any already tainted variables, asking for potential aliases, hidden references, or dynamic behaviors. The expert panel’s response may identify additional variables as tainted, which we then merge back into our working set of tainted data.


In scenarios where a function passes tainted variables across language boundaries—for instance, when Python invokes a C extension function or when C calls back into Python—{\tech} consults prior knowledge of cross-language APIs and the rules established in CICFG. If these variables reach a sink node, we record a fully realized taint flow spanning the entire path from source to sink. Once all subgraphs have been traversed, the system produces a consolidated view of verified vulnerabilities, each annotated with the final chain of tainted variables and functions that lead to an external output. By merging feature-driven insights with LLM guidance, we gain a precise and robust perspective on taint propagation—even in multi-language programs with advanced or unusual language constructs. The full details are provided in Appendix~\ref{sec:phase2algo}.

 

%\subsubsection{Feature Handling}\label{phase 2.3}
\textbf{Feature Handling}.
Before initiating taint propagation, we explicitly handle language-specific features that might introduce implicit or indirect data flows. Certain advanced constructs inherent to Python and C—such as dynamic reflection and runtime code execution, protocol implementations and magic methods in Python, or unions, type punning, and volatile or atomic operations in C—can obfuscate or complicate data-flow analysis. Detecting these implicit flows early ensures improved accuracy and completeness in subsequent taint analysis.

To capture such implicit data flows, {\tech} employs an expert-driven approach leveraging LLM assistance. For each function within the augmented CICFG, we first invoke the expert panel to detect the presence of these complex language features. Given a function's code snippet, the panel identifies whether it utilizes any implicit-flow-causing features. 
If any such features are detected, the expert panel further determines how these constructs implicitly propagate tainted data. Specifically, the panel infers which additional variables might become tainted through the identified implicit flows, supplementing our initial tainted variable set. The results from this expert-assisted analysis are integrated into the initial taint sets for each function.
%
By proactively addressing implicit flows at the outset of our analysis, we significantly enhance the precision and effectiveness of subsequent taint propagation steps. This structured handling of complex language features equips {\tech} with a robust foundation for detecting vulnerabilities.

==> Sections/03_technique.tex <==
\section{Technique}\label{sec:technique}
This section describes our technical approach, \tech, for analyzing cross-language (Python–C) programs and detecting potential vulnerabilities. We begin with an overview of the framework (§\ref{overview}) and then detail its two key phases: the augmented control-flow analysis (§\ref{phase 1}) and the feature-oriented data-flow reasoning (§\ref{phase 2}). These phases work in tandem to systematically uncover taint flows that might otherwise evade traditional static analyses, particularly in complex multi-language settings.

\begin{figure*}[tp]
\begin{center}
\includegraphics[width=0.8\textwidth]{Figures/overview-cai-improved.pdf}
\end{center}
\caption[Methodology Overview]{Overview of the {\tech} framework, including its inputs, two main phases backed by an expert panel, and outputs.}
\vspace{0pt}
\label{fig:overview}
\end{figure*}

\subsection{Approach Overview}\label{overview}
{\tech} is designed to systematically identify potential vulnerabilities in Python–C programs by combining static and language-feature-oriented analyses. As illustrated in Figure~\ref{fig:overview}, the framework accepts two main inputs: the target Python–C source code and user-specified source/sink lists. These inputs feed into two major phases that work in tandem to uncover data-flow paths potentially overlooked by traditional static approaches.

In \textbf{Phase 1}, we construct the CICFG of the given system which integrates its Python and C components. Starting from a basic control-flow structure, we iteratively augment the CICFG to capture diverse features of each language, including decorators in Python and pointer manipulations in C. This augmentation enriches the graph with additional edges and nodes, ensuring that subtle control-flow behaviors---often missed in conventional analysis—--are as completely represented as possible.

The \textbf{Phase 2} revolves around feature-oriented data-flow reasoning. Initially, we perform a directed taint approximation by extracting reachability-based subgraphs for each source–sink pair, forming a preliminary mapping of how external inputs can propagate through the program. We then refine these results through an instructed taint refinement step, which leverages language-specific insights and external function semantics to yield a more precise view of how sensitive data may traverse function and language boundaries. Upon completion of these steps, {\tech} outputs a consolidated list of cross-language taint flows that may present security risks, offering a crucial foundation for further validation or mitigation measures.

% \subsection{Pre-analysis}
% Before constructing the CICFG and performing feature-oriented taint analysis, {\tech} carries out a pre-analysis step to identify and label potential external input points (sources) and critical output functions (sinks). This preliminary phase has two primary objectives. First, it automatically explores the program codebase to discover candidate sources and sinks through LLM queries. Second, the user may also provide a custom list of source/sink definitions, either to account for domain-specific APIs or to refine and override automatic expert panel (LLM-driven analysis, detailed in §~\ref{expert panel}) detections in cases where proprietary or unusual functions exist. {\tech} merges these user inputs with the set of sources and sinks obtained from automatic source-sink identification, ensuring that no critical entry or exit point is overlooked. With a unified source-sink register thus established, we transition to building the augmented CICFG (see §~\ref{phase 1.2}), where these marked entry and exit nodes guide the static and feature-based analyses that follow.

\subsubsection{Expert Panel}\label{expert panel}
To enhance the robustness and cost-effectiveness of our analyses, we propose an expert panel method combining the strengths of non-reasoning (generative) and reasoning LLMs. Non-reasoning LLMs are computationally efficient but prone to instability and hallucination. Conversely, reasoning LLMs provide greater stability and accuracy but at higher computational costs.

Our expert panel employs cross-validation using two non-reasoning models for initial analysis. When disagreements arise between them, a reasoning model is then invoked as an arbiter. This combined approach capitalizes on the efficiency of non-reasoning models for most tasks, reserving the resource-intensive reasoning model for ambiguous or complex cases, thereby achieving an optimal balance between accuracy, stability, and computational expense.

\subsection{Augmented Control-Flow Analysis}\label{phase 1}
{\tech} constructs and refines a CICFG that spans both Python and C code. This graph provides the foundational structure for identifying taint flows in multi-language programs. We first describe how the basic CICFG is built (§~\ref{phase 1.1}), and then show how we augment this initial graph with language-specific features (§~\ref{phase 1.2}), ensuring that subtle cross-language behaviors are not lost during static analysis.


\subsubsection{CICFG Construction}\label{phase 1.1}
The lack of a ready-made, whole-program static information flow analysis tool for real-world Python–C programs motivates us to adapt existing infrastructure to our needs. We start from producing a cross-language, interprocedural control-flow graph for each analyzed project. Following established practices in ICFG construction~\cite{sinha01apr}, every node in the resulting CICFG corresponds to a statement or operation in either the Python or C portions of the codebase, and directed edges indicate the potential transfer of control.

The construction proceeds by first extracting intraprocedural control-flow graphs for each function or method in the target Python and C files. Next, these per-method graphs are connected into an intra-language call graph, one for each language unit. We then identify cross-language call edges by examining how the Python and C components interact, guided by foreign function interface specifications (e.g., Python C APIs). For instance, if a C extension module provides a function accessible from Python, that interface call is represented in the graph as an inter-language edge. Finally, we merge the two intra-language call graphs, along with these cross-language edges, to form the CICFG. Each node is annotated with contextual information, such as the function name and the source-code location, facilitating later traversal of the graph.


\subsubsection{CICFG Augmentation}\label{phase 1.2}

\setlength{\textfloatsep}{0pt} \label{line:1}
\begin{algorithm}[tp]
\scriptsize
\caption{\footnotesize{Phase 1 Feature Controller}}
\label{algo:feature_controller}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{WalkDirectory}{WalkDirectory}
\SetKw{Continue}{continue}
\SetKw{Return}{return}
\LinesNumbered

\KwIn{A project directory path \texttt{proj\_path}}
\KwOut{Analysis results of various features}

\BlankLine
all\_features $\gets$ c\_features + py\_features \; \label{l:allfeatures}
feature\_related\_mapping $\gets$ get\_featuremapping() \; \label{l:featuremapping}

startfile\_dict $\gets$ empty dictionary \; \label{l:startfile_dict}
worklist $\gets$ empty set \; \label{l:worklist}

\ForEach{\texttt{feat} in \texttt{all\_features}}{ \label{l:forFeature}
    startfile $\gets$ [] \; \label{l:startfile_init}
    analyzeFunc $\gets$ feature\_handler\_mapping[\texttt{feat}] \; \label{l:analyzeFunc}
    \ForEach{\texttt{file\_path} in \WalkDirectory(\texttt{proj\_path})}{ \label{l:walkDir}
        (startf, \_) $\gets$ analyzeFunc(\texttt{file\_path}) \; \label{l:analyzeCall}
        startfile.extend(startf) \; \label{l:startfileExtend}
    }
    startfile\_dict[\texttt{feat}] = startfile \; \label{l:startfileDictAssign}
    \If{startfile $\neq$ []}{ \label{l:ifStartfile}
        worklist = worklist $\cup$ feature\_related\_mapping[\texttt{feat}] \; \label{l:worklistUnion}
    }
}

\While{worklist \texttt{ not empty}}{ \label{l:whileWorklist}
    feat $\gets$ worklist.pop() \; \label{l:popFeat}
    startfile $\gets$ startfile\_dict(\texttt{feat}) \; \label{l:getStartfile}
    analyzeFunc $\gets$ feature\_handler\_mapping[\texttt{feat}] \; \label{l:getAnalyzeFunc}
    is\_updated $\gets$ False \; \label{l:isUpdatedInit}
    \ForEach{\texttt{file\_path} in startfile}{ \label{l:forFilePath}
        (\_, updated) $\gets$ analyzeFunc(\texttt{file\_path}) \; \label{l:analyzeAgain}
        \If{updated == True}{ \label{l:checkUpdated}
            is\_updated $\gets$ True \; \label{l:setIsUpdated}
        }
    }
    \If{is\_updated}{ \label{l:ifIsUpdated}
        worklist = worklist $\cup$ feature\_related\_mapping[\texttt{feat}] \; \label{l:worklistUnion2}
    }
}
\end{algorithm}

 While the initial CICFG captures control-flow connections at the function and statement levels, cross-language programs commonly employ various features that can introduce implicit or hidden control flows. Python’s decorator, reflection, and import mechanisms, along with C’s macros, function pointers, and conditional compilation, often cause static analyses to miss relevant control paths if these features are not explicitly accounted for. To address these complexities, {\tech} augments the CICFG in an iterative process that enriches the control-flow representation with additional edges and annotations corresponding to such features.

Initially, we scan the project for a range of language features using specialized handler functions; for example, we detect macros and function pointers in C source files, and decorators or dynamic imports in Python. When a handler discovers any such feature in a file, it marks that file as needing further analysis and adds it to a global worklist. Features that are closely related---for example, macros and conditional compilation---trigger updates to each other’s state so that modifications to one construct can be properly reflected in another. The algorithm then proceeds in a fixed-point manner: if re-analysis of certain files detects new features or modifies existing ones, the corresponding handlers are re-invoked until no further updates are generated.


This process is summarized in Algorithm~\ref{algo:feature_controller}. Lines~\ref{l:allfeatures}-\ref{l:featuremapping} define the union of \texttt{c\_features} and \texttt{py\_features} as \texttt{all\_features}, and retrieve a \texttt{feature\_related\_mapping} that specifies dependencies among features. Lines~\ref{l:startfile_dict} and~\ref{l:worklist} initialize a dictionary for storing file lists (\texttt{startfile\_dict}) and an empty \texttt{worklist} for iterative processing. 
From lines~\ref{l:forFeature}-\ref{l:worklistUnion}, the algorithm iterates over each feature, invokes the corresponding handler on every file found in the project directory, and collects returned \texttt{startfile} information. If \texttt{startfile} is non-empty, the algorithm merges related features into the \texttt{worklist} based on \texttt{feature\_related\_mapping}. 
Lines~\ref{l:whileWorklist}-\ref{l:worklistUnion2} process features in the \texttt{worklist}. Each popped feature retrieves its file list (\texttt{startfile}) and runs the handler again. If any file is updated, the algorithm merges the dependent features into the \texttt{worklist}, ensuring that changes in one feature analysis can trigger re-analysis of related features until all dependencies are stable.

By iterating through potentially interactive or mutually dependent language constructs, we ensure that the final CICFG does not omit control-flow edges that arise from dynamic or conditional behaviors. Nodes that might otherwise appear disconnected become properly linked, and call edges that are only valid under specific macros or function pointer assignments are accurately reflected. The end result is an augmented CICFG in which language features that would typically frustrate purely static approaches are consistently incorporated, providing a robust foundation for our subsequent data-flow analysis.

\subsubsection{Feature Handling} \label{sec:feature-handling}

CICFG augmentation relies on systematically handling language-specific features, which may introduce subtle or dynamic control-flow paths. In this subsection, we illustrate this feature handling approach by detailing our method for analyzing function pointers in C, an inherently dynamic construct often challenging for static analyses.

\begin{algorithm}[tp]
\scriptsize
\caption{\footnotesize{Function Pointer Analysis - C feature}}
\label{algo:enhancedFunctionPointerAnalysis}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{AnalyzeFunctionPointers}{AnalyzeFunctionPointers}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{FindCaller}{FindCaller}
\SetKwFunction{UpdateCICFGEdge}{UpdateCICFGEdge}
\SetKwFunction{RetrieveFunctionBody}{RetrieveFunctionBody}
\SetKw{Return}{return}
\LinesNumbered
\KwIn{set of functions $F$ from a program}\label{pointer_input}
\KwOut{Updated CICFG}\label{pointer_output}

\Fn{\AnalyzeFunctionPointers{F}}{\label{pointer_function_analysis}
    start\_func $\gets$ []\;
    is\_updated $\gets$ false\;
    \ForEach{function in $F$}{\label{pointer_each_function}
        \textit{res} $\gets$ \SendToLLM{"Does the given function use any function pointer? " + code of function}\;\label{pointer_check_fp_use}
        \If{res == "NO"}{\label{pointer_check_fp_response}
            continue\label{pointer_continue}
        }
        \Else{\label{pointer_else}
            start\_func.append(function)\;
            \textit{resp} $\gets$ \SendToLLM{"Give me $<$each function pointer variable name, the function it points to$>$." + code of function}\;\label{pointer_get_fp_details}
            \ForEach{(\textit{pfunc}, \textit{func name}) in resp}{\label{pointer_for_each_fp}
                % funcs $\gets$ \{func\}\; \tcp{initialize list with current function}
                % original func $\gets$ retrieve the code of resp according to current CICFG\;
                \textit{callsite} $\gets$ \FindCaller{pfunc, [\textit{func name}]}\;\label{pointer_find_caller}
                \If{callsite != NULL}{\label{pointer_if_caller_found}
                    \textit{callsite}'s file name, \textit{callsite}'s line no., \textit{func}'s file name, \textit{func}'s line no. $\gets$ retrieve the file name and line no. of \textit{callsite} and \textit{func} from CICFG\;
                    \UpdateCICFGEdge{\textit{callsite}'s file name, \textit{callsite}'s line no., \textit{func}'s file name, \textit{func}'s entry line no.}\;\label{pointer_update_cicfg}
                    is\_updated $\gets$ true\;
                }
            }
        }
    }
    \Return{start\_func, is\_updated}\;
}

\Fn{\FindCaller{\textit{pfunc}, \textit{funcs}}}{\label{pointer_find_caller_fn}
    \textit{funcs code} $\gets$ retrieve the code of each function in \textit{funcs} according to current CICFG\;\label{pointer_retrieve_code}
    \textit{res}, \textit{callsite} $\gets$ \SendToLLM{"Is " + \textit{funcs}[0] + " called via " + \textit{pfunc} + " in the given code? If yes, output 'YES' followed by the \textit{callsite}." + \textit{funcs code}}\;\label{pointer_llm_query1}
    \If{\textit{res} == "YES"}{\label{pointer_response_yes}
        \Return{\textit{caller}}\label{pointer_return_caller}
    }
    \Else{\label{pointer_else_query2}
        \textit{res} $\gets$ \SendToLLM{"Is there any function you don’t know about that is called with " + \textit{pfunc} + "as an argument? If yes, tell me which one"}\;\label{pointer_query_unknown}
        \If{\textit{res} == "no"}{\label{pointer_response_no}
            \Return{NULL}\label{pointer_return_null}
        }
        \Else{\label{pointer_else_find_new}
            %newFunc $\gets$ retrieve the code of \textit{res} according to current CICFG\;
            %newpfunc $\gets$ retrieve the function pointer name in the newFunc\;
            \textit{newFunc} $\gets$ retrieve the function name from \textit{res}\;\label{pointer_new_func}
            \textit{newpfunc} $\gets$ retrieve the name of the parameter of \textit{newFunc} that takes \textit{pfunc} from CICFG\;\label{pointer_new_pfunc}
            \Return{\FindCaller{\textit{newpfunc}, \textit{funcs}.append(\textit{newFunc})}}\label{pointer_recursive_call} \tcp{append new function to the list and reevaluate}
        }
    }
}

\end{algorithm}

Algorithm~\ref{algo:enhancedFunctionPointerAnalysis} describes our approach to handling function pointers, using an expert panel to accurately capture dynamic control-flow edges introduced by pointer usage.
The algorithm begins by processing each function in a provided set  (line~\ref{pointer_each_function}). It employs an expert panel to semantically analyze each function and detect the use of function pointers (line~\ref{pointer_check_fp_use}). If no pointers are found, the analysis skips to the next function (lines~\ref{pointer_check_fp_response}--\ref{pointer_continue}).
Upon detecting a function pointer, the algorithm queries the LLM again to identify the names of function pointer variables and their corresponding target functions (line~\ref{pointer_get_fp_details}). For each pointer-target pair, the \texttt{FindCaller} function is invoked to locate and validate the corresponding call sites (line~\ref{pointer_find_caller}). If valid call sites exist, the CICFG is augmented by adding edges representing these dynamic calls (line~\ref{pointer_update_cicfg}).
The \texttt{FindCaller} function operates recursively, querying the LLM with function and pointer details to verify invocation relationships (lines~\ref{pointer_find_caller_fn}--\ref{pointer_recursive_call}). If the LLM identifies an indirect or previously unknown call relationship, the algorithm expands its analysis scope accordingly, ensuring comprehensive mapping of dynamic control-flow edges.

Applying Algorithm~\ref{algo:enhancedFunctionPointerAnalysis}, we can systematically identify and incorporate function-pointer-included control-flow paths like we presented in our motivation example (\figref{fig:funcp}) into the augmented CICFG, ensuring more sound static analysis.



\subsection{Feature-Oriented Data Flow Reasoning}\label{phase 2}
Having constructed and augmented the CICFG, we next turn to detecting and refining taint flows that may traverse multiple language boundaries in the presence of complex language features. {\tech} orchestrates this phase in two distinct steps: a directed taint approximation stage (§~\ref{phase 2.1}) that enumerates candidate flows from sources to sinks, and an instructed refinement stage (§~\ref{phase 2.2}) that uses feature knowledge and LLM-assisted context to prune or expand these flows as necessary. The final result is a set of potential vulnerabilities, each represented by a path from source to sink across the augmented control-flow graph.

\subsubsection{Directed Taint Approximation}\label{phase 2.1}
The first step of our data-flow reasoning phase applies a control-flow-reachability-based analysis on top of the augmented CICFG. We either use the user-specified source/sink lists or begin by collecting pairs of taint sources and sinks. For each such pair 
⟨\textit{src},\textit{sink}⟩, we slice the augmented CICFG to extract the subgraph of control-flow nodes lying on the possible paths from \textit{src} to \textit{sink}. This subgraph (or control-flow slice) reflects an initial mapping of how data originating from \textit{src} could propagate through both Python and C components until reaching \textit{sink}.

We then aggregate these paths at purely-control-flow level, a process that highlights the subsets of code relevant to each source-sink traversal. By operating on control-level approximation, we significantly reduce the complexity of our subsequent detailed analysis, since we can focus our refinement only on the control flow paths that are flagged as potentially hosting sensitive data flow. Once this reachability-based approximation is complete, the result is a set of candidate paths for each ⟨\textit{src},\textit{sink}⟩ pair, awaiting further scrutiny in the next step.

\subsubsection{Instructed Taint Refinement}\label{phase 2.2}
After gathering all candidate paths, we refine them through a deeper inspection that leverages both static feature handlers and LLM-assisted analyses. For every subgraph derived from the source–sink pairs, we traverse its constituent functions one by one, carrying along a set of tainted variables (initially those introduced at the source).
At each function, we invoke specialized handlers designed to account for language-specific constructs, such as value transfer via pointer indirection in C. These handlers systematically update the set of tainted variables, capturing implicit or indirect data flows that might be missed by purely syntactic analysis. Once the feature handlers have run, we engage the expert panel to confirm or further extend the taint set. The prompt sent to the expert panel encapsulates the current function’s code snippet and any already tainted variables, asking for potential aliases, hidden references, or dynamic behaviors. The expert panel’s response may identify additional variables as tainted, which we then merge back into our working set of tainted data.


In scenarios where a function passes tainted variables across language boundaries—for instance, when Python invokes a C extension function or when C calls back into Python—{\tech} consults prior knowledge of cross-language APIs and the rules established in CICFG. If these variables reach a sink node, we record a fully realized taint flow spanning the entire path from source to sink. Once all subgraphs have been traversed, the system produces a consolidated view of verified vulnerabilities, each annotated with the final chain of tainted variables and functions that lead to an external output. By merging feature-driven insights with LLM guidance, we gain a precise and robust perspective on taint propagation—even in multi-language programs that incorporate advanced or unusual language constructs.

\begin{algorithm}[tp]
\scriptsize
\caption{\footnotesize{LLM-Assisted Taint Analysis with Feature Handlers}}
\label{algo:llmTaintAnalysisFeatures}
\SetKwProg{Fn}{Function}{}{end}
\SetKwFunction{BuildSlice}{BuildSlice}
\SetKwFunction{GetSubgraphFunctions}{GetSubgraphFunctions}
\SetKwFunction{SendToLLM}{SendToLLM}
\SetKwFunction{GetFeatureHandlers}{GetFeatureHandlers}
\SetKwFunction{AnalyzeFunctionWithFeature}{AnalyzeFunctionWithFeature}
\SetKwFunction{GetNextFunctionAndArgs}{GetNextFunctionAndArgs}
\SetKw{Break}{break}
\SetKw{Return}{return}
\LinesNumbered

\KwIn{A set of source/sink pairs $S$, a Control-Integrated Control Flow Graph $CICFG$}
\KwOut{Taint analysis results with updated tainted variables per function}

% Instead of \Fn{\LLMAnalysisWithFeatures{$S,\,CICFG$}}, we do:
\Fn{LLMAnalysisWithFeatures($S,\, CICFG$)}{
    \ForEach{$(src,\, sink) \in S$}{ \label{algoLine1}
        subgraph $\gets$ \BuildSlice{$CICFG,\; src,\; sink$}\; \label{algoLine2}
        functionsInSubgraph $\gets$ \GetSubgraphFunctions{$subgraph$}\; \label{algoLine3}

        taintedVars $\gets$ set of variables initially tainted by $src$\; \label{algoLine4}
        features $\gets$ \GetFeatureHandlers{}\; \label{algoLine5}
        \tcp{features represents a set of feature handlers for implicit data flow, etc.}

        \ForEach{$currentFunc \in functionsInSubgraph$}{ \label{algoLine6}
            \tcp{(1) Update taintedVars using feature handlers}
            \ForEach{$feature \in features$}{ \label{algoLine7}
                newTaintedVarsFromFeature $\gets$ \AnalyzeFunctionWithFeature{feature,\; currentFunc,\; taintedVars}\; \label{algoLine8}
                taintedVars $\gets$ taintedVars $\cup$ newTaintedVarsFromFeature\; \label{algoLine9}
            }

            \tcp{(2) Ask the LLM for additional taint information}
            codeSnippet $\gets$ code of $currentFunc$ from $subgraph$\; \label{algoLine10}
            promptCode $\gets$ "Given this function code and current tainted vars, list all tainted vars in this function:"
                + codeSnippet + \text{" Tainted vars:"} + taintedVars\; \label{algoLine11}
            llmResTaint $\gets$ \SendToLLM{$\text{promptCode}$}\; \label{algoLine12}
            newTaintedFromLLM $\gets$ parse($\text{llmResTaint}$) into a set of tainted variables\; \label{algoLine13}
            taintedVars $\gets$ taintedVars $\cup$ newTaintedFromLLM\; \label{algoLine14}

            \tcp{(3) Determine and pass tainted vars to the next function}
            (nextFunc, passedTaintedVars) $\gets$ \GetNextFunctionAndArgs{currentFunc,\; subgraph,\; taintedVars}\; \label{algoLine15}
            \If{$\text{nextFunc} = \text{NULL}$}{ \label{algoLine16}
                \tcp{No further propagation, end loop for this subgraph}
                \Break
            }
            \Else{ \label{algoLine17}
                taintedVars $\gets$ passedTaintedVars\; \label{algoLine18}
            }
        }
    }
    \Return taintedVars\; \label{algoLine19}
}
\end{algorithm}

Specifically, as shown in  Algorithm~\ref{algo:llmTaintAnalysisFeatures}
For each $(src, sink)$ pair in the input set $S$, this method first builds a subgraph (\emph{subgraph}) that captures paths from \emph{src} to \emph{sink} in the $CICFG$, then extracts all functions appearing in that subgraph (Lines~\ref{algoLine1}--\ref{algoLine3}).
Initialize a set of tainted variables (\emph{taintedVars}) based on the source $src$, and retrieve a collection of feature handlers (\emph{features}). These handlers can account for additional data-flow scenarios such as implicit flows or specific language constructs (Lines~\ref{algoLine4}--\ref{algoLine5}).
For each function in the subgraph, iterate over every feature handler to identify and add new tainted variables (\emph{newTaintedVarsFromFeature}) to the existing \emph{taintedVars} (Lines~\ref{algoLine6}--\ref{algoLine9}).
Use the code of the current function (\emph{codeSnippet}) to query the expert panel. The expert panel response may introduce further tainted variables (\emph{newTaintedFromLLM}). Merge these into \emph{taintedVars} (Lines~\ref{algoLine10}--\ref{algoLine14}).
Determine which tainted variables, if any, should be passed to the next function. If there is no next function (\emph{nextFunc} = NULL), end the loop for this subgraph. Otherwise, update \emph{taintedVars} accordingly and continue (Lines~\ref{algoLine15}--\ref{algoLine18}).
After analyzing all \emph{(src, sink)} pairs, return the resulting tainted variables. This final tainted variable set can then be used for further security analysis or vulnerability detection ({Line~\ref{algoLine19}). 

\subsubsection{Feature Handling}\label{phase 2.3}

Before initiating taint propagation, we explicitly handle language-specific features that might introduce implicit or indirect data flows. Certain advanced constructs inherent to Python and C—such as dynamic reflection and runtime code execution, protocol implementations and magic methods in Python, or unions, type punning, and volatile or atomic operations in C—can obfuscate or complicate data-flow analysis. Detecting these implicit flows early ensures improved accuracy and completeness in subsequent taint analysis.

To capture such implicit data flows, {\tech} employs an expert-driven approach leveraging LLM assistance. For each function within the augmented CICFG, we first invoke the expert panel to detect the presence of these complex language features. Given a function's code snippet, the panel identifies whether it utilizes any implicit-flow-causing features such as:

If any such features are detected, the expert panel further determines how these constructs implicitly propagate tainted data. Specifically, the panel infers which additional variables might become tainted through the identified implicit flows, supplementing our initial tainted variable set. The results from this expert-assisted analysis are integrated into the initial taint sets for each function.

By proactively addressing implicit flows at the outset of our analysis, we significantly enhance the precision and effectiveness of subsequent taint propagation steps. This structured handling of complex language features equips {\tech} with a robust foundation for detecting vulnerabilities.

==> Sections/04_implementation.tex <==
\section{Implementation and Limitations}\label{sec:implementation}
% We have implemented {\tech} to support programs developed in two popular languages: Python and C. 


%\textbf{Pre-analysis.} For source and sink identification, we implemented the Expert Panel described previously. Additionally, our framework provides flexibility by allowing users to manually specify the source and sink points. Users can define these points explicitly by providing detailed metadata, including filename, function names, and line numbers, ensuring precise and tailored analysis according to specific project requirements.

% \textbf{CICFG Augmentation.} To facilitate accurate control-flow analysis across Python–C codebases, we integrated the open-source static code analysis tool Joern. Joern generates intraprocedural control-flow graphs for both Python and C, focusing exclusively on function-level control-flow without handling interprocedural or cross-language flows directly. In our implementation, CICFG nodes represent individual statements, while edges denote the control-flow transitions between these statements. Interprocedural connections are subsequently established through an additional layer of analysis, identifying callsites and return statements to bridge functions. Specifically, cross-language invocation mappings are resolved by analyzing Python C Extension interfaces, enabling linkage of Python and C functions within the CICFG.

% \textbf{Feature-oriented Data-flow Analysis.} To ensure effective and efficient path coverage, we implemented a depth-first search (DFS)-based algorithm to first verify reachability between specified sources and sinks. Once reachability is confirmed, our implementation traverses from the identified source to uncover potential taint flow paths. Users may configure the number of paths (\textit{k}) to be explored; we empirically set $\textit{k = 3}$ as a balanced choice, optimizing between thorough analysis coverage and practical time efficiency.

% \textbf{Expert Panel.} Our Expert Panel implementation utilizes two generative LLMs, DeepSeek V3 and OpenAI's GPT-4o-mini, complemented by a reasoning model, OpenAI's o3-mini. DeepSeek V3 and GPT-4o-mini were selected due to their balance among speed, cost-efficiency, and accuracy in generating initial analysis results. Meanwhile, o3-mini was chosen for its superior performance in reasoning tasks, providing enhanced stability and reducing hallucination risks associated with generative models alone. This combination allows our Expert Panel to deliver both efficiency and precision in source-sink identification. 

% \textbf{Extensibility.} While implemented for Python-C, {\tech} can be readily extended to a different language combination $LC$ 
% by (1) identifying cross-language functions between $LC$ hence constructing the CICFG of a system in $LC$ (e.g., leveraging Joern again if both languages in $LC$ are supported by it), (2) identifying the language features that need to be specially handled (e.g., those that Joern does not handle), and (3) developing the feature handlers accordingly. 
% The same LLMs may be reused given code understanding capabilities for a variety of languages. 

This section details the implementation of the {\tech} framework, emphasizing its modular architecture conducive to extensions, and discusses its current technical and implementation-specific limitations.

\subsection{Implementation}
{\tech} is implemented with a modular architecture designed for future enhancements and adaptability, though it currently possesses certain technical and implementation-specific limitations. The framework's design distinctly separates concerns, facilitating extensibility. 
% Core analysis phases like CICFG augmentation and feature-oriented data-flow reasoning are orchestrated to work with abstract representations and defined interfaces. 
This allows for:

\textbf{Broader Language Support.} New programming language pairs can be incorporated by developing parsers to generate the initial control-flow structures and by creating new language-specific “feature handlers" (e.g., Python-C features). The underlying analysis logic remains largely independent of specific language frontends.

\textbf{Interchangeable LLM Components.} The “Expert Panel"  and other LLM interactions are accessed through an interface that can be adapted to different foundation models, allowing for upgrades or changes in LLM providers or types.

\textbf{Alternative Static Analysis Infrastructure.} While Joern is currently used for initial intraprocedural CFG generation, {\tech}’s subsequent CICFG construction and augmentation logic are self-contained. This permits the potential integration of alternative static analysis tools for the initial graph generation phase, provided they can supply a compatible input format.

\subsection{Limitations}
%Despite its capabilities, {\tech} has the following limitations:
\textbf{Reliance on LLM Efficacy.} The accuracy of identifying challenging language features  and reasoning about data flows  is dependent on the capabilities of the integrated LLMs. While mitigation strategies like the expert panel are in place, LLM-based analysis can be susceptible to inaccuracies or “hallucinations," and the interpretability of LLM decisions can be challenging.

\textbf{Dependence on Source/Sink Accuracy.} The overall analysis is sensitive to the quality of the initial source and sink definitions, whether provided by users or identified via LLM-based methods. Inaccuracies here can impact the relevance and completeness of detected taint flows.

%\textbf{Current Language Pair Focus.} The current {\tech} implementation is specifically for Python-C systems. Extending it to other language combinations requires considerable effort, including parsing new foreign function interfaces and developing feature handlers for the new languages.

\textbf{Multilingual Construction Focus.} Our implementation of {\tech} currently only supports Python-C, given its top popularity and impact in multi-language domains (mainly due to AI/ML systems built on them). Moreover, we currently focus on FFI as the interfacing mechanism between Python and C. Although FFI represents the dominant mechanism, information flow induced by non-FFI interfacing would not be captured by our tool. 



\section{\textit{xFlowBench}: A Multilingual Microbench}\label{sec:microbench}
% \usepackage{multirow}


% \usepackage{multirow}




Evaluating the precision and recall of a cross-language static analysis like {\tech}, especially its handling of complex or dynamic language features, requires a suitable benchmark suite. Since existing benchmarks often lack coverage for specific cross-language interactions or challenging features relevant to static analysis, we created xFlowBench, a micro-benchmark suite tailored for evaluating static analysis across Python-C boundaries.



xFlowBench comprises 42 micro-benchmarks specifically designed to test the handling of challenging language features in both Python and C that can affect information flow analysis. As detailed in Table ~\ref{tab:mb}, each benchmark focuses on one or more of these features, presenting scenarios where traditional static analysis might struggle. This suite allows for a systematic assessment of {\tech}'s ability to correctly identify and handle these complex constructs during its cross-language information flow analysis.

\input{Tables/microbench}

==> Sections/05_RQ1.tex <==
% \subsection{RQ1: How prevalent are targeted Python/C features in real-world C-Python projects?}
\subsection{RQ1: Feature Prevalence}
% To comprehensively evaluate {\tech}, we selected a diverse dataset of 14 real-world, open-source multilingual projects. 
% These projects, which primarily use a Python-C architecture, were chosen to represent a wide range of application domains and scales, from small utilities to large-scale data processing and cryptography libraries. 
% This diversity ensures that our evaluation assesses {\tech}'s performance across various coding styles, complexities, and system sizes. 
% A detailed list of these subject projects, along with their respective lines of code and the proportional distribution of Python and C code, is presented in Table~\ref{tab:benchmarks}.

To understand the landscape in which {\tech} operates, we first investigated the prevalence of several targeted challenging Python and C language features within our dataset of 14 real-world, multilingual projects
, as seen in Table~\ref{tab:benchmarks}. 
The presence of these features was determined by utilizing {\tech}’s intrinsic feature detection capabilities, as detailed in Section~\ref{phase 2.2}. These capabilities employ specialized handlers to identify language constructs within the codebase of the subject projects, ensuring our prevalence study is grounded in the same understanding of features that {\tech} uses for its vulnerability analysis. The results of this feature prevalence analysis are in the Table~\ref{tab:prevalence}.

Our analysis reveals that many of these targeted features are indeed utilized in practice, underscoring the need for analysis tools that can effectively handle them. Notably, a significant number of projects incorporate at least one, and often multiple, of these features, indicating that complex language constructs are not mere edge cases but are actively employed in real-world multilingual software development.

Among the Python features analyzed, First-Class Functions were observed with high frequency, present in 10 out of the 14 projects. Decorators were also utilized in three projects (\texttt{\small japronto}, \texttt{\small pycurl}, \texttt{\small simplejson}), indicating their adoption for modifying or extending behavior. In contrast, specific dynamic features like Reflection (found in \texttt{\small simplejson}) and Dynamic Imports (found in \texttt{\small pyo}) were less common in this particular dataset, each appearing in only one project. Lambda Functions, as per our analysis focusing on the features presented in the results table, were not detected in any analyzed project.

For the C features, Conditional Compilation directives were exceptionally prevalent, identified in 11 of the 14 projects, highlighting their widespread use for managing platform-specific code or build configurations. The Setjmp/Longjmp mechanism for non-local gotos was also common, appearing in 9 projects. Function Pointers, a known source of analysis complexity, were detected in 4 projects (\texttt{\small aubio}, \texttt{\small japronto}, \texttt{\small libsmbios}, \texttt{\small pyo}), while Goto statements were found in 3 projects. The C features External Functions, Inline Assembly, and Macros were not detected in any of the projects within this specific prevalence analysis.

These findings confirm that challenging language features, which can obscure information flow and introduce vulnerabilities, are present across a range of real-world Python/C projects, which reinforces the importance of developing sophisticated static analysis techniques, such as those in {\tech}, capable of accurately interpreting these constructs in a cross-language setting.

% \begin{table}[]
% \caption{Targeted features prevalent in real-world projects.}
% \label{prevalence}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{|c|ccc|cccc|}
% \hline
% \multirow{2}{*}{\textbf{Project}} & \multicolumn{3}{c|}{\textbf{Python Features}}                                                                         & \multicolumn{4}{c|}{\textbf{C Features}}                                                                                                                       \\ \cline{2-8} 
%                                   & \multicolumn{1}{c|}{\textbf{Decorators}} & \multicolumn{1}{c|}{\textbf{First-Classs Functions}} & \textbf{Reflection} & \multicolumn{1}{c|}{\textbf{Function Pointers}} & \multicolumn{1}{c|}{\textbf{Conditional Compilation}} & \multicolumn{1}{c|}{\textbf{Macros}} & \textbf{Goto} \\ \hline
% {\Aubio}                             & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                                &                     & \multicolumn{1}{c|}{\checkmark}                 & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{\checkmark}      & \checkmark    \\ \hline
% {\Bottleneck}                       & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{\checkmark}      & \checkmark    \\ \hline
% {\Bounter}                          & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                & \checkmark    \\ \hline
% {\Cvxopt}                           & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                & \checkmark    \\ \hline
% {\Japronto}                          & \multicolumn{1}{c|}{\checkmark}          & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{\checkmark}                 & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{\checkmark}      & \checkmark    \\ \hline
% {\Libsmbios}                         & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{\checkmark}                 & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                & \checkmark    \\ \hline
% {\Pycurl}                           & \multicolumn{1}{c|}{\checkmark}          & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                & \checkmark    \\ \hline
% {\Pygit}                           & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                & \checkmark    \\ \hline
% {\Pytables}                          & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                & \checkmark    \\ \hline
% {\Pyo}                               & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                                &                     & \multicolumn{1}{c|}{\checkmark}                 & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{\checkmark}      &               \\ \hline
% {\Simplejson}                        & \multicolumn{1}{c|}{\checkmark}          & \multicolumn{1}{c|}{\checkmark}                      & \checkmark          & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                &               \\ \hline
% {\Tink}                              & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{\checkmark}                      &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                &               \\ \hline
% {\Ultrajson}                         & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{}                                &                     & \multicolumn{1}{c|}{}                           & \multicolumn{1}{c|}{\checkmark}                       & \multicolumn{1}{c|}{}                &               \\ \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[htbp]
\centering
\caption{Prevalence of targeted features in our subjects}
\label{tab:prevalence}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}l*{3}{c}*{4}{c}@{}}
\toprule
\multirow{2}{*}{\textbf{Project}} & 
\multicolumn{3}{c}{\textbf{Python Features}} & 
\multicolumn{4}{c}{\textbf{C Features}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8}
& \textbf{Decorators} & \textbf{First-Class Functions} & \textbf{Reflection} & 
\textbf{Function Pointers} & \textbf{Conditional Compilation} & \textbf{Macros} & \textbf{Goto} \\
\midrule
{\Aubio}          &         &         &         & \checkmark & \checkmark & \checkmark & \checkmark \\
\midrule
{\Bottleneck}     &         & \checkmark &         &         & \checkmark & \checkmark & \checkmark \\
\midrule
{\Bounter}        &         & \checkmark &         &         & \checkmark &         & \checkmark \\
\midrule
{\Cvxopt}         &         & \checkmark &         &         & \checkmark &         & \checkmark \\
\midrule
{\Japronto}       & \checkmark & \checkmark &         & \checkmark & \checkmark & \checkmark & \checkmark \\
\midrule
{\Libsmbios}      &         & \checkmark &         & \checkmark & \checkmark &         & \checkmark \\
\midrule
{\Pycurl}         & \checkmark & \checkmark &         &         & \checkmark &         & \checkmark \\
\midrule
{\Pygit}          &         & \checkmark &         &         &         &         & \checkmark \\
\midrule
{\Pytables}       &         & \checkmark &         &         & \checkmark &         & \checkmark \\
\midrule
{\Pyo}            &         &         &         & \checkmark & \checkmark & \checkmark &         \\
\midrule
{\Simplejson}     & \checkmark & \checkmark & \checkmark &         & \checkmark &         &         \\
\midrule
{\Tink}           &         & \checkmark &         &         &         &         &         \\
\midrule
{\Ultrajson}      &         &         &         &         & \checkmark &         &         \\
\midrule
\textbf{Total} & \textbf{21\%} & \textbf{71\%} & \textbf{7\%} & \textbf{29\%} & \textbf{79\%} & \textbf{29\%} & \textbf{64\%} \\
\bottomrule
\end{tabular}
}
\end{table}

==> Sections/05_RQ2.tex <==


% \subsection{RQ2: How effective is {\tech} for static cross-language information flow analysis against SOTA baselines?}
\subsection{RQ2: Effectiveness of {\tech}}

% We evaluated MultiQL on all target projects in our study. During the database merging phase, MultiQL encountered a failure in one project \texttt{pygit2}~\footnote{\url{https://github.com/libgit2/pygit2}}, which we excluded from further analysis. For the remaining projects, we performed dataflow analysis by first translating project-specific sources and sinks into the QL query format, then executing these queries against the merged databases.

% To characterize cross-language dataflows, we used the following verification strategies: for source-sink pairs residing in different languages, any connecting path was inherently classified as a cross-language dataflow; and for intra-language pairs, we required validation that the path traversed at least one foreign language component. However, due to MultiQL's limitation in path-sensitivity, we can not conduct such node-level path verification. To overcome this constraint, we applied an alternative verification methodology: we decomposed paths into (a) reachability between the source and foreign function calls, and (b) reachability between foreign function returns and sinks. To achieve this, we manually collected the names of all the exported functions defined through C \code{PyMethodDef} structures, as MultiQL's dataflow tracking is currently limited to this API. Using this information, we constructed queries that treat calls to these foreign functions as sinks in phase (a) and treat returns from these functions as sources in phase (b). This decomposed verification approach provides a sound approximation of cross-language flow validation while operating within the tool's technical constraints. The dataflow results are shown in the below table.

% In this section, we compared {\tech} against representative state-of-the-art baselines spanning static analysis (MultiQL), dynamic analysis (PolyCruise, PolyFuzz), and deep learning (xLoc) on a common set of real-world Python-C projects known to contain cross-language vulnerabilities previously identified by some of these tools. We run all the baselines and {\tech} on the Real-world benchmarks as shown in Table~\ref{tab:benchmarks}.

% Our evaluation revealed significant differences in the effectiveness of the baseline tools on these benchmarks. Both MultiQL and xLoc failed to detect any of the cross-language vulnerabilities within the target projects. For MultiQL, this aligns with known limitations mentioned in its original study, particularly regarding challenges in tracking data flows involving Python object fields across language boundaries. For xLoc, the result suggests potential challenges in generalizing its learned patterns to these specific vulnerabilities or perhaps the need for more extensive or specific training data encompassing these bug types.

% The dynamic analysis tools, PolyCruise and PolyFuzz, were successful in rediscovering the vulnerabilities they had originally reported in their respective studies when applied to these benchmarks. However, they did not identify any additional vulnerabilities beyond their initial findings. This outcome is consistent with the nature of dynamic tools, whose findings are inherently tied to the specific program executions explored, limited by the coverage achieved through their original test inputs (for PolyCruise) or fuzzing campaigns (for PolyFuzz).

% In stark contrast to the baselines, {\tech} demonstrated superior bug-finding capabilities. It successfully identified all the cross-language vulnerabilities previously reported by both PolyCruise and PolyFuzz within the evaluated projects. More significantly, {\tech} uncovered \textbf{4 previously unknown} cross-language vulnerabilities in these projects that were missed by all baseline tools, including the dynamic ones that previously analyzed these same projects. The results clearly position {\tech} as a more effective technique for discovering cross-language vulnerabilities compared to existing static, dynamic, and learning-based approaches, at least within the scope of our evaluated benchmarks. {\tech}'s ability to replicate the findings of dynamic tools like PolyCruise and PolyFuzz, while operating purely statically, highlights its strength in analyzing information flow without needing specific runtime executions. This overcomes the coverage limitations inherent in dynamic analysis.



% \usepackage{tabularray}


% The discovery of 4 new vulnerabilities underscores the potential of {\tech}'s unique approach. Its static nature allows for exploration of paths potentially not covered by dynamic testing. Furthermore, the synergy between traditional static analysis and LLM-based reasoning likely enables {\tech} to handle complex cross-language interactions and implicit flows more effectively than MultiQL's declarative static analysis or xLoc's learned patterns. The LLM component can potentially bridge semantic gaps and reason about dynamic features that challenge purely static methods, while the static analysis component provides the structural grounding that LLMs might lack, leading to a more comprehensive analysis. The inability of MultiQL and xLoc to find any bugs, and the limitation of PolyCruise and PolyFuzz to only their previously discovered bugs, further emphasizes the difficulty of cross-language vulnerability detection and suggests that {\tech}'s hybrid, static approach offers a significant advantage in both recall (finding known bugs) and novelty (finding new bugs).


% \usepackage{tabularray}
% \begin{table}
% \caption{Precision of {\tech} on Sources/Sinks identification}
% \centering
% \begin{tblr}{
%   cells = {c},
%   cell{1}{1} = {r=2}{},
%   cell{1}{2} = {c=2}{},
%   vlines,
%   hline{1,3-16} = {-}{},
%   hline{2} = {2-3}{},
% }
% Project        & Precision &      \\
%                & Source    & Sink \\
% aubio          & 0.72      & 0.70 \\
% bottleneck     & 0.74      & 1.00 \\
% bounter        & 0.80      & 1.00 \\
% cvxopt         & 0.81      & 1.00 \\
% japronto       & 0.88      & 1.00 \\
% libsmbios      & 0.78      & 0.94 \\
% msgpack-python & 0.80      & 1.00 \\
% pycurl         & 0.85      & 0.91 \\
% pygit2         & 0.82      & 0.83 \\
% pytables       & 0.90      & 0.97 \\
% simplejson     & 0.75      & 1.00 \\
% tink           & 0.73      & 1.00 \\
% ultrajson      & 0.86      & 1.00 
% \end{tblr}
% \end{table}



\begin{table}[t]
\caption{Source/Sink precision and count by project}
\label{tab:source_sink_precision}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll|*{14}{c}|c}
\toprule
& & \rotatebox{90}{\Aubio} & \rotatebox{90}{\Bottleneck} & \rotatebox{90}{\Bounter} & \rotatebox{90}{\Cvxopt} & \rotatebox{90}{\Japronto} & \rotatebox{90}{\Libsmbios} & \rotatebox{90}{\Msgpack} & \rotatebox{90}{\Pycurl} & \rotatebox{90}{\Pygit} & \rotatebox{90}{\Pytables} & \rotatebox{90}{\Pyo} & \rotatebox{90}{\Simplejson} & \rotatebox{90}{\Tink} & \rotatebox{90}{\Ultrajson} & \textbf{Avg} \\
\midrule
\multirow{2}{*}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{Precision}} & 72\% & 74\% & 80\% & 81\% & 88\% & 78\% & 80\% & 85\% & 82\% & 78\% & 90\% & 75\% & 73\% & 86\% & \textbf{80\%} \\
& \multicolumn{1}{c|}{\textbf{Count}} & 351 & 82 & 24 & 375 & 250 & 210 & 51 & 222 & 190 & 909 & 666 & 46 & 595 & 44 & \textbf{305} \\
\midrule
\multirow{2}{*}{\textbf{Sink}} & \multicolumn{1}{c|}{\textbf{Precision}} & 70\% & 100\% & 100\% & 100\% & 100\% & 94\% & 100\% & 91\% & 83\% & 100\% & 97\% & 100\% & 100\% & 100\% & \textbf{95\%} \\
& \multicolumn{1}{c|}{\textbf{Count}} & 51 & 12 & 3 & 14 & 14 & 33 & 4 & 17 & 13 & 144 & 65 & 3 & 45 & 12 & \textbf{32} \\
\bottomrule
\end{tabular}%
}
\end{table}

% We evaluate {\tech}'s effectiveness from three perspectives:

\textbf{Expert Panel Accuracy.} The expert panel is the core component responsible for interpreting complex language features that traditional static analyzers fail to model. To evaluate its performance, we assessed its ability to correctly identify implicit control and data flows. The panel achieved a precision of 0.979, a recall of 0.873, and an F1-score of 0.918 based on xFlowBench. These results demonstrate the expert panel's high reliability. 

\textbf{Source and Sink Identification.} We evaluated {\tech}'s LLM-driven ability to automatically identify security-sensitive sources and sinks on 14 real-world projects. As shown in Table~\ref{tab:source_sink_precision}, {\tech} demonstrates high precision in this task. The superior performance on sinks is likely because sink functions (e.g., memory allocation) are often more standardized and security-critical, thus easier for the LLM to recognize. In contrast, data sources can be more varied and application-specific, leading to slightly lower, yet still effective, precision.

Notably, the performance varies across projects, with source precision being very high for some (e.g., 88\% for \texttt{\small japronto}) but lower for others (e.g., 16\% for \texttt{\small tink}). This variance suggests that project-specific coding conventions and complexity, especially in specialized libraries like the cryptographic tink, can influence the accuracy of LLM-based detection.

\textbf{Data Flow Path Detection.} We compared {\tech} against state-of-the-art static and learning-based tools on ability to identify valid, exploitable data flow paths from a source to a sink. As shown in Table~\ref{tab:detection_performance}, {\tech} successfully identified 272 true positive cross-language data flow paths across the evaluated projects, achieving an overall precision of 81.2\%. It even achieved perfect 100\% precision on five projects, including \texttt{\small bounter} and \texttt{\small cvxopt}.

Most significantly, the baseline tools MultiQL (static) and xLoc (learning-based) failed to detect a single vulnerability path (\#TPs = 0 in all cases). This is not merely a quantitative advantage for {\tech}; it's a fundamental difference in capability. It highlights that existing tools are often unable to trace information flow across language boundaries when obscured by the complex features that {\tech} is specifically designed to handle. This proves the necessity of {\tech}'s neuro-symbolic approach for discovering these otherwise invisible vulnerabilities.


% \begin{table}
% \centering
% \caption{}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tblr}{
%   width = \linewidth,
%   colspec = {Q[273]Q[60]Q[96]Q[171]Q[169]Q[146]},
%   cells = {c},
%   cell{1}{1} = {r=2}{},
%   cell{1}{2} = {r=2}{},
%   cell{1}{3} = {r=2}{},
%   cell{1}{4} = {r=2}{},
%   cell{1}{5} = {c=2}{0.315\linewidth},
%   vlines,
%   hline{1,3-17} = {-}{},
%   hline{2} = {5-6}{},
% }
% \textbf{Project} & \textbf{TP} & \textbf{Total} & \textbf{precision} & \textbf{Crossing} &                  \\
%                  &             &                &                    & \textbf{PolyFlow} & \textbf{MultiQL} \\
% aubio            & 27          & 27             & 100                & 0                 & 0                \\
% bottleneck       & 22          & 26             & 84.6               & 3                 & 0                \\
% bounter          & 28          & 28             & 100                & 26                & 0                \\
% cvxopt           & 0           & 0              & -                  & 0                 & 0                \\
% japronto         & 21          & 24             & 87.5               & 5                 & 0                \\
% libsmbios        & 31          & 51             & 60.7               & 18                & 0                \\
% msgpack-python   & 3           & 3              & 100                & 0                 & 0                \\
% pycurl           & 3           & 4              & 75                 & 2                 & 0                \\
% pygit2           & 35          & 41             & 85.3               & 3                 & 0                \\
% pyo              & 0           & 0              & -                  & 0                 & 0                \\
% pytables         & 0           & 0              & -                  & 0                 & 0                \\
% simplejson       & 24          & 24             & 100                & 2                 & 0                \\
% tink             & 65          & 93             & 69.8               & 8                 & 0                \\
% ultrajson        & 12          & 13             & 92.3               & 4                 & 0                
% \end{tblr}
% }
% \end{table}

\begin{table}[t]
\caption{Effectiveness of {\tech} versus baselines}
\label{tab:detection_performance}
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{l|rrr|rrc|c}
\hline
\multirow{2}{*}{\textbf{Project}} & \multicolumn{3}{c|}{{\tech}} & \multicolumn{3}{c|}{{MultiQL}} & \multirow{2}{*}{{xLoc}} \\
\cline{2-4} \cline{5-7}
 & \textbf{\#Paths} & \textbf{\#TPs} & \textbf{Prec} & \textbf{\#Paths} & \textbf{\#TPs} & \textbf{Prec} & \\
\hline
\Aubio & 27 & 27 & 100\% & 0 & 0 & - & - \\
\Bottleneck & 26 & 22 & 85\% & 0 & 0 & - & - \\
\Bounter & 28 & 28 & 100\% & 0 & 0 & - & - \\
\Cvxopt & 1 & 1 & 100\% & 0 & 0 & - & - \\
\Japronto & 24 & 21 & 88\% & 0 & 0 & - & - \\
\Libsmbios & 51 & 31 & 61\% & 0 & 0 & - & - \\
\Msgpack & 3 & 3 & 100\% & 0 & 0 & - & - \\
\Pycurl & 4 & 3 & 75\% & 0 & 0 & - & - \\
\Pygit & 41 & 35 & 85\% & 0 & 0 & - & - \\
\Pyo & 0 & 0 & - & 0 & 0 & - & - \\
\Pytables & 0 & 0 & - & 0 & 0 & - & - \\
\Simplejson & 24 & 24 & 100\% & 0 & 0 & - & - \\
\Tink & 93 & 65 & 70\% & 0 & 0 & - & - \\
\Ultrajson & 13 & 12 & 92\% & 0 & 0 & - & - \\
\hline
\textbf{Total} & \textbf{335} & \textbf{272} 
& \textbf{81.2\%} 
%& \textbf{88\%} 
& \textbf{0} & \textbf{0} & - & - \\
\hline
\end{tabular}%
}
\end{table}

==> Sections/05_RQ3.tex <==
% \subsection{RQ3: Does each of its components contribute significantly to {\tech}'s performance?}
\subsection{RQ3: Ablation Studies}


To understand the individual contributions of the core components within {\tech}, we conduct an ablation study. We evaluate the impact of the \textbf{Augmented Control Flow (ACF)} analysis, which enriches the program's graph representation to reveal hidden execution paths; the \textbf{Feature-Oriented Data Flow (FDF)} reasoning, which tracks data propagation with a focus on implicit flows; and the \textbf{Expert Panel (EP)}, which integrates LLMs for advanced reasoning and refinement. We created three ablated versions of {\tech} by selectively disabling each component, as detailed in Table~\ref{tab:ablated-new}. By comparing the effectiveness of these versions against the full {\tech} system (which found 272 true positives at 81.2\% precision) in detecting cross-language vulnerabilities, we can quantify the importance of each component.

\begin{table}
    \caption{Description of ablated versions}
    \label{tab:ablated-new}
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{l|c|c|c}
    \toprule
         & Augmented Control Flow & Feature-Oriented Data Flow & Expert Panel \\
    \midrule
    (1) w/o FDF & \ding{51} & \ding{55} &  \ding{51}\\
    \midrule
    (2) w/o ACF   & \ding{55} & \ding{51} & \ding{51} \\
    \midrule
    (3) w/o EP & \ding{51} & \ding{51} & \ding{55} \\
    \bottomrule
    \end{tabular}
    }
\end{table}

% \begin{itemize}[leftmargin=*,topsep=2pt]
%     \item \textbf{Augmented Control Flow (ACF)}: This component extends traditional control-flow analysis by incorporating additional language feature—to provide a richer, more detailed representation of a program's execution paths. This enhanced control flow graph helps reveal hidden or indirect execution routes.
%     \item \textbf{Feature-Oriented Data Flow (FDF)}: This part focuses on tracking how data propagates through the program with an emphasis on key language features that can lead to implicit data flow.
%     \item \textbf{Expert Panel (EP)}: This module integrates LLMs into the analysis process. The Expert Panel reviews and validates the automated findings, offers nuanced insights based on real-world experience, and refines the analysis result. 
% \end{itemize}

\begin{table}[t]
\caption{Results of ablation studies}
\label{tab:ablation_analysis}
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{l|rrr|rrr|rrr}
\hline
\multirow{2}{*}{\textbf{Project}} & \multicolumn{3}{c|}{\textbf{Ablation 1}} & \multicolumn{3}{c|}{\textbf{Ablation 2}} & \multicolumn{3}{c}{\textbf{Ablation 3}} \\
\cline{2-4} \cline{5-7} \cline{8-10}
 & \textbf{\#Paths} & \textbf{\#TPs} & \textbf{Prec} & \textbf{\#Paths} & \textbf{\#TPs} & \textbf{Prec} & \textbf{\#Paths} & \textbf{\#TPs} & \textbf{Prec} \\
\hline
\Aubio & 37 & 27 & 73\% & 21 & 21 & 100\% & 21 & 21 & 100\% \\
\Bottleneck & 62 & 22 & 35\% & 17 & 15 & 88\% & 19 & 16 & 84\% \\
\Bounter & 66 & 28 & 42\% & 20 & 20 & 100\% & 26 & 20 & 77\% \\
\Cvxopt & 3 & 1 & 33\% & 0 & 0 & - & 0 & 0 & - \\
\Japronto & 48 & 21 & 44\% & 1 & 1 & 100\% & 13 & 13 & 100\% \\
\Libsmbios & 102 & 31 & 30\% & 47 & 26 & 55\% & 48 & 26 & 54\% \\
\Msgpack & 11 & 3 & 27\% & 3 & 3 & 100\% & 3 & 3 & 100\% \\
\Pycurl & 49 & 3 & 6\% & 4 & 3 & 75\% & 4 & 3 & 75\% \\
\Pygit & 83 & 35 & 42\% & 34 & 30 & 88\% & 39 & 34 & 87\% \\
\Pyo & 57 & 0 & 0\% & 0 & 0 & - & 0 & 0 & - \\
\Pytables & 49 & 0 & 0\% & 0 & 0 & - & 0 & 0 & - \\
\Simplejson & 15 & 24 & 160\% & 22 & 22 & 100\% & 22 & 22 & 100\% \\
\Tink & 163 & 65 & 40\% & 81 & 58 & 72\% & 87 & 59 & 68\% \\
\Ultrajson & 41 & 12 & 29\% & 10 & 10 & 100\% & 12 & 11 & 92\% \\
\hline
\textbf{Total} & \textbf{786} & \textbf{272} & \textbf{34.6\%} & \textbf{260} & \textbf{209} & \textbf{80.4\%} & \textbf{294} & \textbf{228} & \textbf{77.6\%} \\
\hline
\end{tabular}%
}
\end{table}

The results in Table~\ref{tab:ablation_analysis} reveal the distinct and synergistic roles of each component. Disabling the \textbf{FDF} analysis (Ablation 1) dramatically degrades precision. While this version successfully identifies all 272 true positive paths, it does so at the cost of being flooded by false positives, causing the overall precision to plummet to 34.6\% from an explosion in reported paths. This demonstrates that FDF is not essential for reachability but is crucial for pruning infeasible paths by verifying actual data propagation, thereby eliminating a significant number of false alarms.

Conversely, removing the \textbf{ACF} analysis (Ablation 2) severely impacts recall. The number of true positives found drops by nearly 25\%, as many valid cross-language execution paths are never discovered. Without ACF's ability to resolve dynamic and implicit control flows (e.g., via function pointers or decorators), the foundational graph representation is incomplete, rendering entire classes of vulnerabilities invisible to the subsequent data-flow analysis. The precision, however, remains high (80.4\%) for the paths it can analyze, as the FDF component is still effective on the limited graph.

Finally, operating without the \textbf{EP} (Ablation 3) degrades both precision and recall. This highlights the EP's dual role. It enhances recall by correctly interpreting complex language features that the symbolic engine alone cannot resolve and improves precision by providing nuanced, context-aware reasoning to validate or refute potential taint flows. 

In summary, the experimental results highlight that each component is vital. ACF provides the necessary foundational path coverage, FDF delivers the precision needed to make the results usable, and the EP provides the deep reasoning required to handle modern language complexities. Together, these components form a synergistic framework that is significantly more effective than any of its parts in isolation.

==> Sections/05_RQ4.tex <==


% \subsection{RQ4: How efficient is {\tech} on real-world systems?}
\subsection{RQ4: Efficiency of {\tech}}\label{RQ4}


% To comprehensively evaluate the runtime efficiency of {\tech}, we conducted experiments on 14 real-world benchmarks ranging from small utility libraries like bounter, ultrajson, and simplejson to large-scale systems such as PyTables, tink, and pyo. Our evaluation focused on three key metrics: Lines of Code (in thousands), Execution Time (in hours), and Peak Memory Usage (in MB). For each project, we collected data on its code size and measured the corresponding execution time and memory consumption during {\tech}’s operation.

% As shown in Figure~\ref{fig:efficiency}, the results indicate that while {\tech}’s execution time generally increases with program size, the trend is not entirely linear. In smaller projects, the runtime overhead remains relatively low, with execution times staying under 5 hours, which confirms {\tech}’s high efficiency in environments with limited code and features. However, once the system size exceeds 30K lines of code, the overhead begins to rise significantly. For example, the largest benchmark, pyo (with approximately 60K lines of code), has an execution time approaching 55 hours, whereas systems like cvxopt and tink exhibit overheads ranging from 30 to 45 hours. This increase is likely due to the deeper execution stacks and richer language features present in larger systems, which introduce more computational burden during tracking.

% In contrast, memory usage shows a relatively flat trend relative to the size of the code. For most systems under 30K LOC, the peak memory consumption remains consistently under 200 MB. Even as project sizes grow, memory usage scales only moderately—tink peaks at around 370 MB, and pyo reaches 750 MB. These levels are within acceptable limits on modern computing platforms, including those with constrained resources.

% Overall, the evaluation demonstrates that {\tech} maintains high efficiency for small to medium systems, while its increased resource demands in larger frameworks remain within reasonable bounds. This suggests that {\tech} is adaptable and effective across a wide spectrum of system sizes, making it a promising solution for various application scenarios.

To comprehensively evaluate the runtime efficiency of {\tech}, we conducted experiments on 14 real-world benchmarks. Our evaluation focused on key performance metrics: total analysis time, LLM token consumption, and peak memory usage, contextualized by the lines of code (LOC) of each project. Figure~\ref{fig:efficiency} summarizes the overall performance, while Table~\ref{tab:performance_analysis} provides a breakdown of resource consumption across {\tech}'s two main analysis phases.


\begin{table}[t]
\caption{{\tech} cost breakdown}
\label{tab:performance_analysis}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|cccc|c}
\toprule
\multirow{3}{*}{\textbf{Subject}} & \multicolumn{3}{c|}{\textbf{Phase 1}}  & \multicolumn{4}{c|}{\textbf{Phase 2}} & \multicolumn{1}{c}{\textbf{}} \\
\cmidrule{2-4} \cmidrule{5-7} \cmidrule{8-8}
& \textbf{Step 1} & \textbf{Step 2} & \textbf{Step 2} & \textbf{Step 1} & \textbf{Step 2} & \textbf{Step 2} & \textbf{Avg Time} & \textbf{Memory} \\
& \textbf{Time (h)} & \textbf{Time (h)} & \textbf{Tokens (M)} & \textbf{Time (h)} & \textbf{Time (h)} & \textbf{Tokens (M)} & \textbf{per Query (s)} & \textbf{Peak (MB)} \\
\midrule
{\Aubio} & 0.36 & 3.63 & 2.80 & 4.60 & 4.48 & 0.12 & 2.50 & 274 \\
{\Bottleneck} & 0.21 & 1.82 & 0.98 & 2.56 & 4.39 & 0.15 & 3.18 & 209 \\
{\Bounter} & 0.58 & 0.67 & 0.49 & 0.44 & 2.61 & 0.15 & 1.62 & 167 \\
{\Cvxopt} & 0.36 & 4.13 & 4.61 & 4.15 & 7.36 & 0.90 & 5.70 & 338 \\
{\Japronto} & 0.35 & 2.58 & 1.35 & 1.48 & 4.83 & 0.12 & 2.66 & 213 \\
{\Libsmbios} & 0.06 & 1.13 & 0.84 & 1.32 & 4.18 & 0.24 & 1.85 & 183 \\
{\Msgpack} & 0.08 & 0.62 & 0.41 & 6.13 & 5.58 & 0.11 & 1.85 & 183 \\
{\Pycurl} & 0.11 & 3.37 & 1.94 & 0.50 & 0.63 & 0.33 & 1.81 & 230 \\{\Pygit} & 0.08 & 2.42 & 2.40 & 1.11 & 4.72 & 0.28 & 1.84 & 224 \\
{\Pyo} & 0.13 & 11.26 & 15.00 & 8.10 & 9.45 & 2.10 & 4.23 & 2009 \\
{\Pytables} & 1.23 & 7.19 & 8.32 & 3.63 & 4.37 & 2.20 & 2.20 & 606 \\
{\Simplejson} & 0.14 & 0.99 & 0.69 & 6.88 & 5.47 & 0.14 & 1.87 & 185 \\
{\Tink} & 0.41 & 4.78 & 3.63 & 6.17 & 8.24 & 0.62 & 4.86 & 315 \\
{\Ultrajson} & 0.78 & 0.31 & 0.32 & 7.87 & 5.36 & 0.09 & 1.68 & 187 \\
\midrule
\textbf{Average} & \textbf{0.35} & \textbf{3.21} & \textbf{3.13} & \textbf{3.93} & \textbf{5.13} & \textbf{0.54} & \textbf{2.70} & \textbf{380} \\
\bottomrule
\end{tabular}%
}
\end{table}

The results indicate that while {\tech}'s execution time generally scales with project size, the relationship is not strictly linear, with runtime performance also being highly sensitive to code complexity. For example, smaller projects like \texttt{\small ultrajson} and \texttt{simplejson} exhibit longer analysis times than some larger projects. This variance is attributable to our \textit{expert panel} design, which modulates computational cost based on analytical difficulty. Two efficient non-reasoning LLMs can quickly reach a consensus. However, for more complex or ambiguous code constructs, these models may disagree, triggering the invocation of a more powerful and computationally reasoning model to act as an arbiter and resolve the conflict. 
% The longer runtimes for ultrajson and \texttt{\small simplejson} suggest their codebases contain a higher density of such complex constructs, leading to more frequent arbitration and thus increased overall analysis time. 
In general, LLM token consumption, grows with project size and complexity, with \texttt{\small pyo} consuming the most tokens at 17.1 million. This is expected, as larger and more complex projects naturally contain more functions and control-flow paths requiring LLM-based reasoning.


\begin{figure}[tp]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/efficiency.pdf}
\end{center}
\caption{Performance and cost of {\tech} across real-world projects.}
\vspace{0pt}
\label{fig:efficiency}
\end{figure}

A detailed breakdown of the runtime, presented in Table~\ref{tab:performance_analysis}, reveals that the most resource-intensive steps are those involving LLM-based reasoning. Specifically, Phase 1, Step 2 (CICFG augmentation) and Phase 2, Step 2 (Instructed Taint Refinement) consume the majority of both time and tokens. This is because these steps delegate the analysis of complex language features (e.g., function pointers, dynamic imports) that stymie traditional static analysis to the expert panel. The initial, non-LLM steps, such as CICFG construction and taint approximation, are comparatively fast. 

In contrast to execution time, peak memory usage scales more moderately with code size. For most systems under 250k LOC, memory consumption remains well under 1 GB, with an average peak of 380 MB across all projects. Even large projects like \texttt{\small PyTables} (219.8k LOC) and \texttt{\small tink} (257.7k LOC) peaked at 606 MB and 315 MB, respectively. The \texttt{\small pyo} project was an outlier, reaching a peak of approximately 2 GB, likely due to a high density of complex cross-language interactions requiring more state to be held in memory. These footprints are well within the capacity of modern workstations, demonstrating that {\tech}'s memory requirements are practical for real-world use.

% Overall, our evaluation demonstrates that {\tech} achieves a reasonable balance between analytical depth and resource efficiency. While the analysis of large, complex systems is computationally intensive, the costs are primarily driven by the necessary and targeted application of LLM-based reasoning to overcome the fundamental limitations of traditional static analysis. The framework's architecture effectively contains these costs, particularly memory usage, making it a viable and scalable solution for discovering complex vulnerabilities in real-world, multi-language software.


==> Sections/05_RQ5.tex <==


% \subsection{RQ5: Can {\tech} find cross-language vulnerabilities?}\label{RQ4}
\subsection{RQ5: Real-world Bug Discovery}
\newcommand{\tinycircnum}[1]{%
\tikz[baseline=(char.base)]{
    \node[
      shape=circle,
      fill=black,
      inner sep=0pt,
      minimum size=0.7em,
      text height=0.5em,  % Controls vertical centering
      text depth=0.1em,  % Controls baseline offset
      align=center
    ] (char) {\sffamily\bfseries\color{white}\scriptsize #1};
  }%
}
% \begin{table}[t]
% \caption{Comparison of Detection Tools by Project}
% \label{tab:vul_label}
% \centering

% \begin{tabular}{l|cccc}
% \hline
% \textbf{Subject} & \textbf{PolyFlow} & \textbf{MultiQL} & \textbf{xLoc} \\
% \hline
% \Aubio & 1 & 0 & 0 \\
% \Bounter & 3 & 0 & 0 \\
% \Japronto & 2 & 0 & 0 \\
% \Pygit & 1 & 0 & 0 \\
% \Cvxopt & 1 & 0 & 0 \\
% \hline
% \textbf{Total} & \textbf{8} & \textbf{0} & \textbf{0} \\
% \hline
% \end{tabular}

% \end{table}

\begin{wraptable}{l}{0.45\linewidth}
    \caption{Comparison of detection tools by project}
    \label{tab:vul_label}
    \centering
    % 表格的tabular部分保持不变
    \scalebox{0.71}{
        \begin{tabular}{l|cccc}
        \hline
        \textbf{Subject} & \textbf{{\tech}} & \textbf{MultiQL} & \textbf{xLoc} \\
        \hline
        \Aubio & 1 & 0 & 0 \\
        \Bounter & 2 & 0 & 0 \\
        \Ultrajson & 1 & 0 & 0 \\
        \Japronto & 2 & 0 & 0 \\
        \Pygit & 1 & 0 & 0 \\
        \Cvxopt & 1 & 0 & 0 \\
        \hline
        \textbf{Total} & \textbf{8} & \textbf{0} & \textbf{0} \\
        \hline
        \end{tabular}
    }
\end{wraptable}

This Table~\ref{tab:vul_label} summarizes the number of buffer overflows detected per benchmark, along with the total count. So, we select one previously unknown bug discovered by {\tech} to conduct a detailed case study. \texttt{Bounter}
% ~\footnote{\url{https://github.com/piskvorky/bounter}} 
is a Python library accelerated with C extensions, designed for high-speed, memory-bounded frequency counting in massive datasets often encountered in NLP and Machine Learning.  The vulnerability identified by {\tech} exists in the C implementation of the Count-Min Sketch (CMS) initialization routine, specifically the \texttt{CMS\_VARIANT(\_init)} function in \texttt{cbounter/cms\_common.c}, as illustrated in Figure~\ref{fig:bounter}. This function sets up the CMS data structure based on width and depth parameters provided by the user during object instantiation in Python code (\tinycircnum{1})

As shown in Figure~\ref{fig:bounter}, the user-provided width and depth parameters flow from Python into the C initialization function and are parsed using \texttt{PyArg\_ParseTupleAndKeywords} (\tinycircnum{2}). The code subsequently sanitizes the depth parameter by enforcing a strict range check $[1, 32]$ (\tinycircnum{3}), ensuring it does not exceed a small, fixed upper bound. However, the width parameter lacks equivalent sanitization. It is processed to calculate \texttt{self->width} by rounding the input down to the nearest power of two (\tinycircnum{4}), but no check prevents this value from becoming excessively large based on the input.

The function then proceeds to allocate memory for each row of the \texttt{\small CMS} table within a loop (\tinycircnum{5}). Inside this loop, the calloc function is invoked (\tinycircnum{6}): \texttt{\small self->table[i] = (CMS\_CELL\_TYPE *) calloc(self->width, sizeof(CMS\_CELL\_TYPE));}. From a static analysis perspective focusing on input validation, the lack of strict sanitization for the width parameter is critical. A very large user input for width can lead to a large \texttt{self->width} value, causing the calloc at line 31 to request a potentially huge amount of memory. This significantly increases the risk of \texttt{\small calloc} failing and returning NULL. Crucially, the return value from \texttt{\small calloc} is assigned directly to \texttt{\small self->table[i]} without any check for NULL. Should calloc fail due to large size requested (stemming from the insufficiently sanitized width), \texttt{\small self->table[i]} becomes NULL. While this assignment itself does not crash the program, it introduces a null pointer into the CMS structure, setting the stage for a null-pointer dereference vulnerability when subsequent operations (e.g., increment, get) attempt to access this specific table row \texttt{\small self->table[i]} expecting valid memory. Thus, the vulnerability originates from the unsanitized width input leading to a potential \texttt{\small calloc} failure whose result is used unsafely.

{\tech} is adept at identifying this type of cross-language vulnerability due to its core design principles. Firstly, its ability to construct a Cross-language Interprocedural Control Flow Graph (CICFG) accurately models the transition from the Python caller to the C initialization function \texttt{\small CMS\_VARIANT(\_init)}, capturing the initial flow of the user-provided width parameter across the language boundary. Secondly, {\tech}'s two-phase analysis, particularly the Feature-Oriented Data Flow Reasoning phase, performs taint analysis that tracks this width parameter. While width undergoes some transformation, {\tech}'s analysis, aided by its LLM-based expert panel during taint refinement, can recognize that width lacks the strict upper-bound sanitization applied to depth. This lack of sanitization allows the taint to propagate to the size argument of the \texttt{\small calloc} call within the loop. Finally, {\tech}'s analysis identifies the subsequent unsafe handling: the result of \texttt{\small calloc} is assigned to \texttt{\small self->table[i]} without a null check, creating the potential for a later null-pointer dereference. The framework's explicit handling of cross-language interactions and its multi-stage analysis combining static techniques with LLM reasoning enables the detection of such vulnerabilities originating from parameter handling across language interfaces.

On the other hand, existing static, dynamic, and learning-based approaches likely failed to detect this specific vulnerability due to several factors. Static tools like MultiQL often rely on predefined query patterns and may struggle to precisely track data flow across Python-C API boundaries or reason about the semantic implications of insufficient input sanitization leading to allocation failures, particularly if specific rules for this pattern are absent. Dynamic analysis tools, such as PolyCruise or fuzzers like PolyFuzz, depend on runtime execution and would only trigger this bug under specific, hard-to-replicate conditions of memory exhaustion combined with a large input width. Achieving such conditions reliably during testing is challenging, and limited test coverage often hinders the discovery of such edge-case vulnerabilities. Learning-based tools like xLoc might not have been trained on data containing similar subtle memory management flaws stemming from cross-language parameter handling and missing null checks after allocation, limiting their ability to generalize and detect this specific pattern. {\tech}'s combination of cross-language control/data flow graph construction and LLM-assisted reasoning allows it to overcome these limitations by explicitly modeling the cross-language flow and reasoning about the potential consequences of the partially sanitized input.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures//Case Study/bounter-case.pdf}
    \caption{A vulnerability case found in \texttt{bounter} }
    \label{fig:bounter}
\end{figure}






% \setminted{
%   highlightcolor=yellow
% }

% \begin{listing}[!ht]
% \scriptsize
% \begin{minted}[linenos]{python}
% if log_counting == 8:
%     self.cms = cmsc.CMS_Log8(width=self.width, depth=self.depth)
% \end{minted}
% \end{listing}
% \vspace{-20pt}
% \begin{listing}[!ht]
% \scriptsize
% \begin{minted}[linenos]{c}
% static int
% CMS_VARIANT(_init)(CMS_TYPE *self, PyObject *args, PyObject *kwds)
% {
%     static char *kwlist[] = {"width", "depth", NULL};

%     uint32_t w;
%     if (!PyArg_ParseTupleAndKeywords(args, kwds, "II", kwlist,
% 				      &w, &self->depth)) {
%         return -1;
%     }

%     if (self->depth  < 1 || self->depth > 32) {
%         char * msg = "Depth must be in the range 1-16";
%         PyErr_SetString(PyExc_ValueError, msg);
%     }

%     short int hash_length = -1;
%     while (0 != w)
%         hash_length++, w >>= 1;
%     if (hash_length < 0)
%         hash_length = 0;
%     self->width = 1 << hash_length;
%     self->hash_mask = self->width - 1;

%     HyperLogLog_init(&self->hll, 16);

%     self->table = (CMS_CELL_TYPE **) malloc(self->depth * sizeof(CMS_CELL_TYPE *));
%     int i;
%     for (i = 0; i < self->depth; i++)
%     {
%         self->table[i] = (CMS_CELL_TYPE *) calloc(self->width, sizeof(CMS_CELL_TYPE));
%     }
%     return 0;
% }
% \end{minted}
% \caption{Hello World in C}
% \label{listing:2}
% \end{listing}



==> Sections/05_RQ6.tex <==
\subsection{RQ6: How effectively \tech can detect single-language language bugs in Python and C?}

==> Sections/05_evaluation.tex <==
\section{Evaluation} \label{sec:eval}


To understand the effectiveness of {\tech}, we evaluate it on benchmarks and real-world C-Python projects. Specifically, our evaluation aims to answer the following research questions:

\begin{itemize}
    \item[\textbf{RQ1}] How prevalent are targeted Python/C features in real-world C-Python projects?
    \item[\textbf{RQ2}]  How effective is {\tech} for static cross-language information flow analysis against SOTA baselines? 
    \item[\textbf{RQ3}]  Does each of its components contribute significantly to {\tech}'s performance? %Ablation studies.
    \item[\textbf{RQ4}]  How efficient is {\tech} on real-world systems? %What is the runtime overhead of {\tech}.
    \item[\textbf{RQ5}]  Can {\tech} find cross-language vulnerabilities? %Case studies.
    %\item[\textbf{RQ5}]  How effectively {\tech} can detect single-language language bugs in Python and C?
\end{itemize}

\textbf{Experimental Setup}.
In addition to xFlowBench (Table~\ref{tab:mb}), we also evaluated POLYFLOW against 14 real-world multilingual programs written in Python and C as their primary languages. Table~\ref{tab:benchmarks} summarizes these programs as our subjects, including the total code size in thousands of lines of code (2nd column) and the percentage of code written in each respective language (3rd and 4th columns).

We conduct our experiments on a %high-performance 
workstation equipped with an AMD Ryzen Threadripper 3970X CPU, which operates at 3.7GHz and has 32 physical cores, an Nvidia GeForce RTX 3090 GPU, and 256GB of RAM.
For static code analysis tasks, we utilize Joern version 4.0.216. In experiments involving the expert panel, we set the temperature parameter to 0 for LLMs.
% , ensuring deterministic behavior. 
This configuration guarantees consistent output generation from identical inputs, thus enhancing reproducibility.
% All other environment details, libraries, and specific dependencies remain consistent across all experiments, ensuring controlled and reproducible conditions.

% We evaluate {\tech} against xx real-world multilingual systems written in Python and C as primary languages.

\begin{table}[]
    \centering
    \caption{Real-world multilingual subjects}
    \begin{tabular}{lrrr}
        \toprule
        Benchmark & LOC (k) & Python code \% & C code \% \\
        \midrule
        {\Bounter}        & 3.5   & 50.9\% & 48.2\% \\
        {\Ultrajson}      & 5.1   & 34.3\% & 64.8\% \\ 
        {\Simplejson}     & 6.2   & 59.8\% & 37.6\% \\
        {\Libsmbios}      & 8.3   & 30.4\% & 64.2\% \\
        {\Japronto}       & 9.4   & 48.2\% & 50.4\% \\
        {\Pycurl}         & 14.6  & 54.8\% & 40.7\% \\
        {\Msgpack}        & 15.1  & 48.7\% & 50.1\% \\
        {\Bottleneck}     & 16.9  & 49.5\% & 48.6\% \\
        {\Pygit}          & 17.0  & 44.6\% & 57.4\% \\
        {\Aubio}          & 42.9  & 25.4\% & 73.3\% \\ 
        {\Cvxopt}         & 56.0  & 39.0\% & 60.8\% \\
        {\Pytables}       & 219.8 & 46.6\% & 52.1\% \\
        {\Tink}           & 257.7 & 7.2\%  & 33.5\% \\ 
        {\Pyo}            & 259.1 & 48.8\% & 50.8\% \\
        \bottomrule
    \end{tabular}
    \label{tab:benchmarks}
\end{table}

\textbf{Baselines}.
\textit{Static Methods;} We chose MultiQL~\cite{youn2023declarative} as our static analysis baseline because it represents the most recent, state-of-the-art approach in declarative, cross-language static analysis, making it the most direct and relevant comparison for {\tech}'s methodology. MultiQL is a prototype extension of CodeQL, a declarative static analysis framework developed by GitHub, for multilingual program analysis.  As a query-based analysis tool, MultiQL first transforms C and Python source code into databases of facts separately. These databases are subsequently merged by establishing interlanguage dataflow edges, connecting arguments in foreign function calls to their corresponding parameters in cross-language target functions. Once the merged database is generated, MultiQL performs reachability analysis, accepting user-defined sources and sinks as query inputs and computing the existence of dataflow between them as outputs. 


% \subsubsection{Dynamic Methods}
% PolyCruise~\cite{wen22usenixsecurity} is a dynamic information flow analysis (DIFA) technique for multi-language programs. It combines language-specific static analysis to compute symbolic dependencies with language-agnostic online dynamic analysis, overcoming language heterogeneity. We compare {\tech} against PolyCruise on the source/sink pairs PolyCruise used.

% PolyFuzz~\cite{wen23usenixsecurity} is a greybox fuzzer that holistically fuzzes multi-language systems. It uses cross-language coverage feedback and models semantic relationships between program inputs and branch predicates across languages. We compare {\tech} against PolyFuzz by comparing the ultimately found bugs.



\textit{Deep Learning Method;} To evaluate {\tech} against a competing, state-of-the-art methodology, we chose xLoc~\cite{yang2024learning}, which represents a pure deep learning-based approach to the same problem. This comparison allows us to assess the benefits of our neuro-symbolic framework against end-to-end learning solutions. xLoc is a deep learning-based technique for detecting and localizing multilingual bugs using only source code. It employs a customized Transformer model, pre-trained to understand multilingual control-flow structures and fine-tuned using cross-language API vicinity information to specifically target multilingual bugs. The implementation focuses on Python-C software. We compare {\tech} against xLoc on the ultimately found bugs.

\textbf{Metrics and Procedure}.
For RQ1 (targeted feature prevalence), we measure how targeted C and Python features are distributed in real-world C-Python projects we studied. 


For RQ2 (effectiveness measurement), we measure the precision of sources and sinks {\tech} identified and the taint flow paths found correspondingly.

%total number of unique vulnerabilities discovered by {\tech} compared to baseline tools (MultiQL, PolyCruise, PolyFuzz, and xLoc), reporting precision where applicable.

For RQ3 (ablation study), we created several variants of {\tech} by selectively disabling key components. We compare these variants against the complete {\tech} to quantify the contribution of each component.

For RQ4 (performance evaluation), we measured runtime performance and resource consumption. Specifically, we tracked total analysis time (broken down by phase) and peak memory usage.

%and scalability factors including lines of code analyzed per minute and the relationship between codebase size and analysis time.

For RQ5 (real-world bug discovery), we conducted detailed qualitative analysis of selected bugs discovered by {\tech}. Each case study documents the vulnerability type, how it manifests across language boundaries, why existing tools failed to detect it, and the path through which {\tech} successfully identified it.


\input{Sections/05_RQ1}
\input{Sections/05_RQ2}
\input{Sections/05_RQ3}
\input{Sections/05_RQ4}
\input{Sections/05_RQ5}
% \input{Sections/05_RQ5}

==> Sections/06_discussion.tex <==
\section{Discussion}



\subsection{Why {\tech} works}
% A key reason for {\tech}'s success is the explicit and deep handling of challenging language features that are often sources of stealthy vulnerabilities. Instead of treating these features as black boxes, {\tech} uses specialized handlers in a fixed-point iterative process to resolve their complex control flows, enriching the CICFG until it is a stable and more complete representation of the program. This methodical approach allows it to succeed where other static tools like MultiQL fail, particularly in tracing data flows through complex patterns like Python object fields passed across language interfaces. Furthermore, its two-phase, refinement-based strategy—performing a fast, lightweight taint approximation before deploying a more expensive, LLM-driven path analysis—ensures that its deep reasoning is applied efficiently and scalably.

% Compared to dynamic analysis baselines like PolyCruise and PolyFuzz, {\tech}’s purely static nature grants it a fundamental advantage in coverage. It is not constrained by the quality or completeness of test inputs or fuzzing campaigns, allowing it to explore all syntactically possible execution paths. This comprehensive exploration capability is why {\tech} successfully identified previously unknown vulnerabilities in projects that these dynamic tools had already analyzed.

% Finally, {\tech}’s success is not merely due to using LLMs, but to its robust integration strategy. The framework actively mitigates known LLM weaknesses like hallucination and inaccuracy through its "Expert Panel" design, which employs multiple LLMs in a negotiation and arbitration process for cross-validation. By combining the structural rigor of static analysis with the semantic power of carefully managed LLM agents, {\tech} achieves a more comprehensive and effective analysis of cross-language information flows than prior state-of-the-art approaches.

The success of {\tech} is founded on three synergistic design principles that address the core difficulties of cross-language static analysis.

First, {\tech} constructs a comprehensive CICFG. Traditional static analyzers often fail to connect information flows across language boundaries due to complex features that obscure control flow. For instance, in our motivating example~\ref{fig:vuln-example}, a Python tool may not recognize a \texttt{\small @app.route} decorator as a data source, while a C tool halts at an unresolved function pointer. This makes it impossible to link the tainted Python input to the C-based format-string vulnerability. {\tech} resolves these through a fixed-point iterative process, enriching the CICFG with the complete, end-to-end control-flow path. This robust graph provides a solid foundation for subsequent data-flow analysis.

Second, {\tech} utilizes a novel agentic framework that delegates tasks to Large Language Models. Rather than passing entire codebases to LLMs---an approach that is infeasible and prone to error---{\tech} uses its static analyzer as a “controller." This controller invokes an LLM “expert panel" only for specific, challenging features where traditional analysis fails. This targeted delegation leverages the semantic reasoning of LLMs while mitigating their weaknesses, such as hallucination, through a multi-LLM negotiation and fact-checking process.

Finally, {\tech} employs an efficient and scalable two-phase, refinement-based data-flow reasoning strategy. It first performs a fast, lightweight taint approximation using control-flow reachability to quickly identify a small set of candidate paths. It then deploys a more expensive, LLM-driven “Instructed Taint Refinement" only on these pre-filtered paths. This two-phase approach ensures that deep, semantic reasoning is applied efficiently, focusing computational resources only where necessary and making the analysis practical for complex, real-world systems.

\subsection{Where {\tech} Falls Short and Why}
Despite its effectiveness, {\tech}'s design incorporates trade-offs and dependencies that introduce shortcomings. The framework's capabilities are fundamentally tied to the quality of its underlying components—both the initial static analysis infrastructure and the LLMs. Its reliance on Joern for initial control-flow graph generation means it inherits any limitations or parsing inaccuracies from that tool. More centrally, while LLMs provide the semantic reasoning needed to bridge language gaps, they are also a primary source of limitations. The analysis is subject to the inherent probabilistic nature and potential inaccuracies of LLMs, which necessitates complex mitigation strategies like the Expert Panel. 
% This dependency also introduces practical concerns regarding computational cost and the reproducibility of results with different or updated models.

Furthermore, {\tech}'s analytical depth comes at the cost of performance. The same deep, iterative feature handling  and multi-staged, LLM-assisted taint refinement  that allow it to uncover subtle, cross-language vulnerabilities also make it computationally intensive. This can lead to significant analysis runtimes, particularly on very large-scale systems, which may not be suitable for all development workflows. This trade-off between analytical rigor and speed is a deliberate design choice but a practical limitation.

Finally, challenges exist in its real-world application and extension. Like many advanced static analysis tools, its findings may require manual effort to confirm true exploitability, as the tool identifies potential information flows rather than guaranteed vulnerabilities. While the framework is designed to be modular, extending it to new language pairs is a non-trivial engineering task. It requires developing new, specialized handlers and defining the intricate rules of interaction for the new language combination, a process that demands significant domain expertise.

\subsection{Limitations of Existing Techniques}
Static analysis frameworks like CodeQL, and by extension its multilingual prototype MultiQL, struggle with the semantic gaps inherent in cross-language interactions. In our experiments, MultiQL failed to detect any cross-language vulnerabilities in our benchmark projects. Our investigation revealed this is largely because MultiQL fails to track data flows for the fields of Python objects across the language boundary. This limitation manifests in common invocation patterns. For example, in the “aubio" project, a C function is bound to a Python object method; MultiQL detects the object reference but fails to resolve the subsequent field access on the method call, thus missing the data flow edge entirely. This inability to trace data through object-bound or module-bound function calls renders it ineffective for many common designs in Python-C software.

Dynamic analysis tools, such as PolyCruise~\cite{wen22usenixsecurity} and PolyFuzz~\cite{wen23usenixsecurity}, are fundamentally constrained by the execution paths they explore. While they successfully rediscovered the vulnerabilities they were originally designed to find, they did not identify any of the new vulnerabilities discovered by {\tech}. Their effectiveness is inherently tied to the coverage achieved by their specific test cases or fuzzing campaigns. A concrete example of this insufficiency is the bounter vulnerability (Section~\ref{RQ4}), which is triggered by a large input value causing a memory allocation failure. Dynamic tools are unlikely to find such a bug unless their test inputs are specifically crafted to induce memory exhaustion, a condition that is difficult to achieve reliably during testing and is often missed.

Finally, learning-based techniques like xLoc, which rely on patterns learned from existing code, also failed to find any vulnerabilities in the target projects. The primary limitation of such approaches is their difficulty in generalizing to novel or complex bug patterns that were not well-represented in their training data. 
For the bounter vulnerability, a learning-based model would need to have been trained on very specific examples of cross-language parameter handling that lead to unchecked memory allocation failures to detect the flaw; without such prior examples, it is unable to identify the pattern. 
% {\tech} was designed to overcome these specific limitations by combining the comprehensive path coverage of static analysis with the semantic reasoning required to navigate complex cross-language interactions.

==> Sections/07_related-cai.tex <==
% root: paper-ccs.tex
\section{Related Work}\label{sec:related}
%\vspace{3pt}\noindent
\textbf{LLM-assisted/agent-based program analysis.}
Given their capabilities for code understanding and generating, LLMs have been used to assist with various program analysis tasks, ranging from comprehending source/obfuscated code~\cite{fang2024large} to detecting/classifying software vulnerabilities~\cite{linlarge25ndss}. 
{LLift}~\cite{li2024enhancing} complements symbolic execution with LLMs for identifying use-before-initialization bugs in the Linux kernel, utilizing the LLMs to extract and solve path constraints that trigger the bugs. 
To recover names and types for local variables and user-defined data structures from stripped binaries, {ReSym}~\cite{xie2024resym} fine-tunes two LLMs and combines them with Prolog-based reasoning, mimicking a manual reverse engineering process. 
Recently, {IRIS} leverages LLMs to assist CodeQL with static taint analysis for Java projects, using LLMs to refine CodeQL's taint specification and then to triage the taint paths reported by CodeQL via contextual analysis. 
AutoCodeRover~\cite{zhang2024autocoderover} builds an agent by combining LLMs with code search to automatically solve GitHub issues, while 
SWE-Agent~\cite{yang2024swe} and OpenHands~\cite{wang2024openhands} are agents serving a broader set of coding tasks such as code editing. 

In comparison, {\tech} addresses multilingual code while involving LLMs directly in the core program analysis steps (control-flow augmentation and data-flow propagation) and without fine-tuning. Our agentic approach is also different in that it adds autonomy to LLMs via program analysis, rather than merely letting LLMs assist with the latter. 


\vspace{3pt}\noindent
\textbf{Static taint/information flow analysis.}
Language-level information flow analysis, such as JFlow~\cite{myers1999jflow} for Java, realizes static flow checking by extending a given language, while application-level 
approaches like Pixy~\cite{jovanovic2006pixy} for PhP detect taint-style vulnerabilities via data-flow analysis. 
Static taint analysis has also been enabled to detect sensitive user inputs in SUPOR~\cite{huang2015supor} and privacy leaks in UIPicker~\cite{nan2015uipicker}, both 
for Android apps and leveraging FlowDroid~\cite{arzt2014flowdroid}---a static data flow analyzer for those apps. 
Information flow control has also been achieved at the level of the hardware description language to verify hardware security mechanisms~\cite{ferraiuolo2017verification}. 
%
In contrast, we focus on static information flow analysis \textit{across different languages}, versus these approaches addressing flows within language boundaries. 

\vspace{3pt}\noindent
\textbf{Cross-language code analysis.}
By adopting CodeQL to multi-language projects, MultiQL~\cite{youn2023declarative} achieves proof-of-concept static cross-language bug detection by extending CodeQL's 
databases to include interoperation rules based on cross-language APIs. The reliance on CodeQL makes MultiQL inherit its fundamental limitations, such as applicability to only vulnerabilities whose code patterns are known and can be well-defined, as well as low precision and recall due to the lack of in-depth data/control flow analysis and ignorance of challenging language features. 
AXA~\cite{roth2024axa} obtains cross-language static analysis results by orchestrating the interleaved execution of single-language analyses, propagating results between
the two analyzers hence integrating their results. 
Similarly, JNIFER~\cite{zhang2025interactive} interactively resolves native code to accomplish cross-language pointer analysis, while 
CSS~\cite{kan2024cross} refines the native code specification by incorporating caller sensitivity, both for Java-C code. 
A number of other static analysis approaches for multilingual programs exist, relying on handcrafted summaries/rules an/or heavy engineering, as summarized in~\cite{roth2024axa}. 
However, like JNIFER and CSS, AXA relies on the availability and capabilities of a sophisticated analysis infrastructure of each language. 

{\tech} is developed to overcome these limitations of existing approaches, explicitly handling various language features by leveraging the merits of LLMs for code analysis.  

==> Sections/07_related.tex <==
\section{Related work}

==> Sections/08_conclusion-cai.tex <==
% root: paper-ccs25.tex
\section{Conclusion}\label{sec:conclusion}
With cross-language vulnerabilities burgeoning and continuing to compromise the security of multi-language systems, 
it is imperative to discover those defects before they are exploited. 
Yet existing defensive techniques suffer from various critical limitations that impede their practical adoption. 
We thus explore a neuro-symbolic approach to statically reasoning about information flow across language boundaries, hence 
developing {\tech}, a static cross-language information flow analysis framework. 
By combining the strengths of traditional static analysis and LLMs while mitigating their respective weaknesses, 
{\tech} overcomes semantics disparities and challenging language features within and across heterogeneous languages. 
%explicitly dealing with key technical challenges to this analysis
Compared to state-of-the-art solutions of various kinds against diverse real-world multi-language systems, 
{\tech} demonstrated its merits in terms of cost-effectiveness and cross-language vulnerability discovery. 

==> Sections/08_conclusion.tex <==

\section{Conclusion}
The conclusion goes here.

==> Tables/cc_comparison.tex <==
\begin{table}[t]
\caption{Cost-effectiveness vs.\ Claude Code %on the 29 multilingual subjects.
}
\label{tab:cc_cost}
\centering
\small
\begin{tabular}{lrrr}
\toprule
                                  & \textbf{{\tech}} & \textbf{Claude Code} & \textbf{Ratio (CC/{\tech})} \\
\midrule
Total LLM cost (\$)               & 96.38            & 452.50               & 4.7$\times$  \\
Avg.\ cost per project (\$)       & 3.32             & 15.60                & 4.7$\times$  \\
Cross-lang.\ vulnerabilities found & 18               & 5                    & 0.28$\times$ \\
\textbf{Cost per bug found (\$)}  & \textbf{5.35}    & \textbf{90.50}       & \textbf{16.9$\times$} \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\end{table}


==> Tables/lan_feature.tex <==
\begin{table}[htbp]
\centering
\caption{Summary of challenging language features and their support status in Joern and \tech, where $\protect\yes$ indicates full support, $\protect\rhalf$ denotes partial support with missing control flow edges, $\protect\lhalf$ represents missing nodes, and $\protect\no$ indicates complete lack of support.}


% 
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{clcc}
\hline
\multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{Challenging Features}} & \multirow{2}{*}{\textbf{Joern}} & \multirow{2}{*}{\textbf{\tech}} \\
 &  &  &  \\ \hline
\multirow{8}{*}{C} & Function Pointers & \rhalf & \yes \\ 
 & Conditional Compilation & \no & \yes \\ 
 & External Functions & \no & \yes \\ 
 & Inline Assembly & \rhalf & \yes \\ 
 & Macros Expanding to Function Calls & \rhalf & \yes \\ 
 & Goto Statements & \rhalf & \yes \\ 
 & Setjmp/Longjmp & \rhalf & \yes \\ 
 & Recursive Functions & \yes & \yes \\ \hline
\multirow{6}{*}{Python} & Decorators & \rhalf & \yes \\ 
 & First-Class Functions & \rhalf & \yes \\ 
 & Lambda Functions & \no & \yes \\ 
 & Generators and Coroutines & \yes & \yes \\ 
 & Reflection & \rhalf & \yes \\ 
 & Dynamic Imports & \no & \yes \\ \hline
\end{tabular}
}
\label{tab:motivation-study}
\end{table}

==> Tables/lan_feature_new.tex <==
\begin{table}[htbp]
\centering
\caption{Summary of challenging language features and their support status in Joern and \tech, where $\protect\yes$ indicates support and $\protect\no$ indicates lack of support.}


% 
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{clcc}
\hline
\multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{Challenging Features}} & \multirow{2}{*}{\textbf{Joern}} & \multirow{2}{*}{\textbf{\tech}} \\
 &  &  &  \\ \hline
\multirow{8}{*}{C} & Function Pointers & \no & \yes \\ 
 & Conditional Compilation & \no & \yes \\ 
 & External Functions & \no & \yes \\ 
 & Inline Assembly & \no & \yes \\ 
 & Macros Expanding to Function Calls & \no & \yes \\ 
 & Goto Statements & \no & \yes \\ 
 & Setjmp/Longjmp & \no & \yes \\ 
 & Recursive Functions & \yes & \yes \\ \hline
\multirow{6}{*}{Python} & Decorators & \no & \yes \\ 
 & First-Class Functions & \no & \yes \\ 
 & Lambda Functions & \no & \yes \\ 
 & Generators and Coroutines & \yes & \yes \\ 
 & Reflection & \no & \yes \\ 
 & Dynamic Imports & \no & \yes \\ \hline
\end{tabular}
}
\label{tab:motivation-study}
\end{table}

==> Tables/lan_feature_old.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{Challenging features~}} & \multirow{2}{*}{\parbox{1.8cm}{\centering \textbf{Joern}\\\textbf{handling}}} & \multicolumn{2}{c|}{\textbf{Impact on static analysis}} & \multicolumn{2}{c|}{\textbf{PolyFlow design}} & \multirow{2}{*}{\parbox{1.8cm}{\centering \textbf{PolyFlow}\\\textbf{handling}}} \\ \cline{4-7} 
 &  &  & \parbox{2.2cm}{\centering \textbf{Code entities}\\\textbf{(CICFG nodes)}} & \parbox{2.2cm}{\centering \textbf{Flow facts}\\\textbf{(CICFG edges)}} & \parbox{2.2cm}{\centering \textbf{Static analysis}\\\textbf{enhancement}} & \parbox{2.2cm}{\centering \textbf{LLM-driven}\\\textbf{enhancements}} &  \\ \hline
\multirow{6}{*}{C} 
  & Function Pointers                  & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Conditional Compilation            & \no  & \yes & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & External Functions                 & \no  & \yes & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Inline Assembly                    & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Macros Expanding to Function Calls & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Goto Statements                    & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Setjmp/Longjmp                     & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Recursive Functions                & \yes & -   & -    & -   & -   & \yes \\ \hline
\multirow{6}{*}{Python} 
  & Decorators                & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & First-Class Functions     & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Lambda Functions          & \no  & \yes & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Generators and Coroutines & \yes & -   & -    & -   & -   & \yes \\ \cline{2-8}
  & Reflection                & \no  & -   & \yes  & -   & \yes & \yes \\ \cline{2-8}
  & Dynamic Imports           & \no  & \yes & \yes  & -   & \yes & \yes \\ \hline
\end{tabular}%

==> Tables/microbench.tex <==

\begin{table}[htbp]
\caption{Summary of xFlowBench}
\centering
% \footnotesize
\resizebox{1\columnwidth}{!}{
\begin{tabular}{clccccc}
\hline
\multirow{2}{*}{\textbf{Lang.}} & \multirow{2}{*}{\textbf{Feature}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\#micro-\\ benchs\end{tabular}}} & \multicolumn{2}{c}{\textbf{\#data points}} & \multirow{2}{*}{\textbf{\#FNs}} & \multirow{2}{*}{\textbf{\#FPs}} \\ \cline{4-5}
 &  &  & \textbf{\#edges} & \textbf{\#nodes} &  &    \\ \hline \hline
\multirow{5}{*}{\rotatebox{90}{\textbf{Python}}} 
 & Decorators & 2 & 12 & 0 & 0 & 0  \\
 & First-Class Functions & 2 & 4 & 0 & 0 & 0  \\
 & Lambda Functions & 4 & 5 & 4 & 1 & 0  \\
 & Dynamic Typing & 2 & 4 & 0 & 0 & 0 \\
 & Reflection & 4 & 4 & 0 & 2 & 0  \\
 & Dynamic Imports & 4 & 1 & 1 & 0 & 0 \\ \hline
\multirow{7}{*}{\rotatebox{90}{\textbf{C}}} 
 & Function Pointers & 2 & 10 & 0 & 0 & 0  \\
 & Conditional Compilation & 2 & 1 & 1 & 0 & 0 \\
 & External Functions & 4 & 2 & 1 & 2 & 0  \\
 & Inline Assembly & 4 & 4 & 0 & 2 & 0  \\
 & Macro Functional Calls & 4 & 2 & 0 & 1 & 0 \\
 & Goto Statements & 4 & 4 & 0 & 0 & 0  \\
 & Setjmp/Longjmp & 4 & 4 & 0 & 0 & 0  \\ \hline
\multicolumn{2}{c}{\textbf{Total}} & 42 & 57 & 7 & 8 & 0  \\ \hline
\end{tabular}
}
\label{tab:mb}
\end{table}


==> Tables/microbench_old.tex <==

\begin{table*}[htbp]
\caption{Summary of the xFlowBench micro-benchmark suite}
\centering
% \footnotesize
\resizebox{1\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\textbf{lang/langc}} & \multirow{2}{*}{\textbf{Feature}} & \multirow{2}{*}{\textbf{\#micro-benchmarks}} & \multicolumn{2}{c|}{\textbf{\#data points}} & \multirow{2}{*}{\textbf{\#Total}} & \multirow{2}{*}{\textbf{\#FN}} & \multirow{2}{*}{\textbf{\#FP}} & \multirow{2}{*}{\textbf{\#TP}} & \multirow{2}{*}{\textbf{\#vul\_path}} & \multirow{2}{*}{\textbf{\#FN}} & \multirow{2}{*}{\textbf{\#FP}} & \multirow{2}{*}{\textbf{\#TP}} \\ 
\cline{4-5}
 &  &  & \textbf{\#edges} & \textbf{\#nodes} &  &  &  &  &  &  &  &  \\ 
\hline
\multirow{5}{*}{\textbf{Python}} & Decorators & 2 & 12 & 0 & \multirow{5}{*}{35} & 0 & 0 & 12 & \multirow{12}{*}{16} & \multirow{12}{*}{1} & \multirow{12}{*}{0} & \multirow{12}{*}{12} \\ 
\cline{2-5}\cline{7-9}
 & First-Class Functions & 2 & 8 & 0 &  & 0 & 0 & 8 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Lambda Functions & 4 & 5 & 4 &  & 1 & 0 & 4 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Reflection & 4 & 4 & 0 &  & 2 & 0 & 2 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Dynamic Imports & 4 & 1 & 1 &  & 0 & 0 & 2 &  &  &  &  \\ 
\cline{1-9}
\multirow{7}{*}{\textbf{C}} & Function Pointers & 2 & 10 & 0 & \multirow{7}{*}{29} & 0 & 0 & 10 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Conditional Compilation & 2 & 1 & 1 &  & 0 & 0 & 2 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & External Functions & 4 & 2 & 1 &  & 2 & 0 & 1 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Inline Assembly & 4 & 4 & 0 &  & 2 & 0 & 2 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Macros & 4 & 2 & 0 &  & 1 & 0 & 1 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Goto & 4 & 4 & 0 &  & 0 & 0 & 4 &  &  &  &  \\ 
\cline{2-5}\cline{7-9}
 & Setjmp/Longjmp & 4 & 4 & 0 &  & 0 & 0 & 4 &  &  &  &  \\
\hline
\end{tabular}
}
\label{tab:mb}
\end{table*}
